An Introduction to Quantum Machine Learning for Engineers

In the current noisy intermediate-scale quantum (NISQ) era, quantum machine learning is emerging as a dominant paradigm to program gate-based quantum computers. In quantum machine learning, the gates of a quantum circuit are parametrized, and the parameters are tuned via classical optimization based on data and on measurements of the outputs of the circuit. Parametrized quantum circuits (PQCs) can efficiently address combinatorial optimization problems, implement probabilistic generative models, and carry out inference (classification and regression). This monograph provides a self-contained introduction to quantum machine learning for an audience of engineers with a background in probability and linear algebra. It first describes the necessary background, concepts, and tools necessary to describe quantum operations and measurements. Then, it covers parametrized quantum circuits, the variational quantum eigensolver, as well as unsupervised and supervised quantum machine learning formulations.

==> Chapter5/Chapter5.tex <==
\chapter{Generalizing Quantum Measurements (Part II)}

\section{Introduction}

In this chapter, we generalize quantum measurements in an arbitrary basis, which were introduced in Chapter 3, in two successive steps. In the first step, we introduce projective measurements as a form of ``incomplete'' measurements, as opposed to ``complete'' measurements in arbitrary orthonormal bases. Projective measurements will allow us to define the important concept of quantum observables. As an application of projective measurements, we will briefly introduce the problem of quantum error correction. Then, in the second step, we will further generalize projective measurements to  positive operator-valued measurements (POVMs), which provide the most general form of quantum measurements. As an application of POVMs, we will discuss the problem of unambiguous state detection.
		
	
	\section{Projective Measurements}\label{sec:ch5:projmeas}
	
	In this section, we introduce projective measurements.
	
	\subsection{Complete vs. Incomplete Measurements}
		 von Neumann measurements of $n$ qubits in an arbitrary orthonormal basis $\{|v_{x}\rangle\}_{x=0}^{2^{n}-1}$
		are \textbf{complete} in the sense that the post-measurement state is known to be a specific coherent state. In fact, given the measurement's output
			 $x\in \{0,1,...,2^{n}-1\}$, the post-measurement state is   given by vector $|v_{x}\rangle$.  Note that the post-measurement is known even when, as is usually the case, the measured state is not.
		
		 Projective measurements generalize conventional von Neumann measurements by allowing for \textbf{incomplete} measurements, whereby 			 the post-measurement state is only known to lie in a subspace specified
			by the output of the measurement. As we will see, projective measurements are strongly related to partial
		measurements studied in Chapter 3 (see Sec. \ref{sec:ch3:partial}) in which only a subset of qubits is measured.

	
		 To introduce projective measurements, let us first review complete measurements in an arbitrary orthonormal
		basis $\{|v_{0}\rangle,...,|v_{N-1}\rangle\}$ of $N=2^{n}$ vectors,
		each of dimension $N\times1$. As discussed in Sec. \ref{sec:ch3:densityform}, 
		 for a quantum (density) state $\rho$ of the system of $n$ qubits, von Neumann measurements
		prescribe that the probability of observing $x\in\{0,1,...,N-1\}$
		is
		\begin{align}
			\Pr[\textrm{measurement output equals }x] & =\langle v_{x}|\rho|v_{x}\rangle \nonumber\\ &=\textrm{tr}(|v_{x}\rangle\langle v_{x}|\rho)=\textrm{tr}(v_{x}\rho),
		\end{align}
		where we have defined the \textbf{projection matrices} 
		\begin{equation}
		v_{x}=|v_{x}\rangle\langle v_{x}|
		\end{equation}
		for $x\in\{0,1,...,N-1\}$.
		 Projection matrices are positive semi-definite matrices with eigenvalues
		equal to 0 or 1.  Furthermore, the post-measurement state, expressed as a density matrix,
		is 
		\begin{equation}\label{eq:ch5:postm}
		|v_{x}\rangle\langle v_{x}|=\frac{v_{x}\rho v_{x}}{\langle v_{x}|\rho|v_{x}\rangle}.
		\end{equation}
		 Equality (\ref{eq:ch5:postm}) can be proved by noting that we can always write the density matrix $\rho$ as 
		\begin{equation}
		\rho=\sum_{x=0}^{N-1}\sum_{x'=0}^{N-1}\lambda_{x,x'}|v_{x}\rangle\langle v_{x'}|,
		\end{equation}
		with $\lambda_{x,x'}=\langle v_{x}|\rho|v_{x'}\rangle$.
	

	
		 von Neumann measurements are hence defined by \textbf{rank-1 projection matrices}
		$v_{x}=|v_{x}\rangle\langle v_{x}|$, which satisfy the \textbf{resolution
		of the identity condition} 
		\begin{equation}\label{eq:ch5:resid}
		\sum_{x=0}^{N-1}v_{x}=I.
		\end{equation}
		 To see that the equality (\ref{eq:ch5:resid}) holds, it is sufficient to note that we
		have the equality 
		\begin{equation}
		\left(\sum_{x=0}^{N-1}v_{x}\right)|\psi\rangle=|\psi\rangle
		\end{equation}
		for any input state, since we can always express any input state
		as the superposition $|\psi\rangle=\sum_{x=0}^{N-1}\alpha_{x}|v_{x}\rangle$
		and we have 
		\begin{equation}
		v_{x}|v_{x'}\rangle=|v_{x}\rangle\langle v_{x}|v_{x'}\rangle,
		\end{equation}
		with $\langle v_{x}|v_{x'}\rangle=0$ for $x\neq x'$ and $\langle v_{x}|v_{x}\rangle=1$.
	

	\subsection{Defining Projective Measurements}\label{sec:ch5:defproj}
	
		Generalizing the description given in the previous subsection of standard complete measurements, projective measurements are defined by a set $N'\leq N$
		of projection matrices $\{\Pi_{y}\}_{y=0}^{N'-1}$, with rank possibly
		larger than 1 (when $N'<N$), such that the resolution-of-identity
		condition 
		\begin{equation}\label{eq:ch5:residg}
		\sum_{y=0}^{N'-1}\Pi_{y}=I
		\end{equation}
		is satisfied.
		Geometrically, condition (\ref{eq:ch5:residg}) indicates that linear combinations
		of vectors from the subspaces spanned by the $N'$ predictors cover the
		entire Hilbert space. More formally, the sum of the subspaces spanned
		by the projectors coincides with the Hilbert space.
		 We will see later how to satisfy this condition in practice by partitioning the vectors of 
		an orthonormal basis of the Hilbert space.
	

	
		 A projective measurement defined by projection matrices $\{\Pi_{y}\}_{y=0}^{N'-1}$ satisfying the resolution-of-identity condition (\ref{eq:ch5:residg}) is defined as follows.\begin{itemize}
		 	\item \textbf{Born's rule}: The probability of observing $y\in\{0,1,...,N'-1\}$ is
		\begin{align}\label{eq:ch5:Born}
			\Pr[\textrm{measurement output equals }y]=\textrm{tr}(\Pi_{y}\rho),
		\end{align}which, for a pure state  $\rho=|\psi\rangle\langle\psi|$ simplifies as \begin{align}\label{eq:ch5:Bornpure}
		\Pr[\textrm{measurement output equals  }y]=\textrm{tr}(\Pi_{y}\rho)=\langle\psi|\Pi_{y}|\psi\rangle;
	\end{align}
	\item \textbf{``Incomplete collapse'' of the state}:	The post-measurement state is
		\begin{equation}\label{eq:ch5:postmeas}
		\frac{\Pi_{y}\rho\Pi_{y}}{\textrm{tr}(\Pi_{y}\rho)}, 
		\end{equation}which, for a pure state  $\rho=|\psi\rangle\langle\psi|$ simplifies as\begin{equation}\label{eq:ch5:postmeaspure}
		\frac{\Pi_{y}|\psi\rangle}{\sqrt{\langle\psi|\Pi_{y}|\psi\rangle}}.
	\end{equation}
\end{itemize}Note that with rank-1 projection matrices, these rules reduce to the standard, complete, von Neumann
		measurement reviewed in the previous subsection. 
		
	
		To elaborate on the post-measurement state (\ref{eq:ch5:postmeas})-(\ref{eq:ch5:postmeaspure}), we now discuss how to  construct a projective measurement. The projection matrices $\{\Pi_{y}\}_{y=0}^{N'-1}$ defining a projective
		measurement can be always obtained from some orthonormal basis $\{|v_{0}\rangle,...,|v_{N-1}\rangle\}$
		by partitioning these vectors into $N'$ subsets and defining $\Pi_{y}$ as the projector onto the subspace spanned by the $y$th subset of basis vectors. More formally, let us partition the index set $\{0,1,...,N-1\}$ into $N'$ disjoint subsets  $\mathcal{X}_{y}\subseteq \{0,1,...,N-1\}$ with $y\in\{0,1,...,N'-1\}$, such that their union equals the overall set $\{0,1,...,N-1\}$.  Each matrix $\Pi_{y}$ is the projector into the
		subspace spanned by the $y$th subset of vectors, i.e., 
		\begin{equation}
		\Pi_{y}=\sum_{x\in\mathcal{X}_{y}}|v_{x}\rangle\langle v_{x}|.
		\end{equation}
	
	
Returning to the post-measurement state (\ref{eq:ch5:postmeaspure}), we can now make the following observations. First, a complete measurement in basis $\{|v_{0}\rangle,...,|v_{N-1}\rangle\}$
	leaves an input state $|\psi\rangle$ unchanged if it is one of the vectors $|v_{x}\rangle$
	in the basis, i.e., if $|v_{x}\rangle=|\psi\rangle$ for some $x\in\{0,...,N-1\}$. In contrast,  a projective measurement leaves a state $|\psi\rangle$ unchanged if
	it is \emph{any} vector  in the subspace spanned by one of the projectors
	$\Pi_{y}$, i.e., if it can be written as a linear combination $|\psi\rangle=\sum_{x\in\mathcal{X}_{y}} \alpha_x |v_x\rangle$ for some $y\in\{0,...,N'-1\}$. Second, as we will see in the next subsection with an example, based on the given an arbitrary pure state $|\psi\rangle$, upon observing a measurement $y\in\{0,...,N'-1\}$, the post-measurement state (\ref{eq:ch5:postmeaspure}) is generally only known to lie in the subspace $\Pi_y$.
		

\subsection{An Example: Parity Measurements}\label{sec:ch5:paritymeas}
	
		 To illustrate the operation of a projective measurement, let us consider  $n=2$ qubits (i.e., $N=4$) and fix the computational
		basis $\{|00\rangle$ ,$|01\rangle$, $|10\rangle$, $|11\rangle\}.$ A projective measurement with $N'=2$ possible outcomes can be defined by  partitioning these vectors into \textbf{even-parity states} $\{|00\rangle,|11\rangle \}$, for which the number of ones in the defining cbit string is an even number; 
		and \textbf{odd-parity states} $\{|01\rangle,|10\rangle \}$ in which the number of ones is odd. Note that this corresponds to the subsets  $\mathcal{X}_{0}=\{00,11\}$ and $\mathcal{X}_{1}=\{01,10\}$. Accordingly,  the \textbf{parity projective measurement} is defined by the rank-2 projectors
		\begin{equation}
		\Pi_{0}=|00\rangle\langle00|+|11\rangle\langle11|
		\end{equation} and 
		\begin{equation}
		\Pi_{1}=|01\rangle\langle01|+|10\rangle\langle10|.
		\end{equation}
	
Let us not study the effect of the parity projective measurements on two qubits in an arbitrary pure state
			\begin{equation}\label{eq:ch5:genstate}
			|\psi\rangle=\alpha_{00}|00\rangle+\alpha_{01}|01\rangle+\alpha_{10}|10\rangle+\alpha_{11}|11\rangle.
			\end{equation} By the Born rule (\ref{eq:ch5:Bornpure}), 
			the output of the measurement is $y=0$ with probability
			\begin{align}\label{eq:ch5:parityp1}
				\langle\psi|\Pi_{0}|\psi\rangle=|\alpha_{00}|^{2}+|\alpha_{11}|^{2},
			\end{align} and $y=1$ with probability 	
		\begin{align}\label{eq:ch5:parityp2}
		\langle\psi|\Pi_{1}|\psi\rangle=|\alpha_{01}|^{2}+|\alpha_{10}|^{2}.
	\end{align}
		Furthermore,	the post-measurement state (\ref{eq:ch5:postmeaspure}) is 
			\begin{equation}\label{eq:ch5:postex}
			\frac{\Pi_{0}|\psi\rangle}{\sqrt{\langle\psi|\Pi_{0}|\psi\rangle}}=\frac{1}{\sqrt{|\alpha_{00}|^{2}+|\alpha_{11}|^{2}}}(\alpha_{00}|00\rangle+\alpha_{11}|11\rangle)
			\end{equation} when the measurement output is $y=0$; while it is \begin{equation}
			\frac{\Pi_{1}|\psi\rangle}{\sqrt{\langle\psi|\Pi_{1}|\psi\rangle}}=\frac{1}{\sqrt{|\alpha_{01}|^{2}+|\alpha_{10}|^{2}}}(\alpha_{01}|01\rangle+\alpha_{10}|10\rangle)
		\end{equation} when the measurement output is $y=1$.
	

	
		Let us consider the case in which the original state (\ref{eq:ch5:genstate}) is unknown, i.e., we do not know the amplitudes $\alpha_{00},$ $\alpha_{01}$,  $\alpha_{10}$, and  $\alpha_{11}$. If the measurement is $y=0$, the post-measurement state (\ref{eq:ch5:postex})  is in the subspace spanned
			by $\Pi_{0}$, i.e., by the even-parity vectors $|00\rangle$ and $|11\rangle$. Apart from this information,
			nothing else can be inferred from the output of the measurement. This makes the measurement ``incomplete''. 
		  Note the difference with complete von Neumann measurements
			in the computational basis, in which the post-measurement state is
			the basis vector $|x_{0},x_{1}\rangle$ corresponding to the measurement's
			output $x_{0},x_{1}$.
	
Consider now the situation in which the measured  state $|\psi\rangle$ is in the subspace spanned by $\Pi_0$, and hence it can be written as  $|\psi\rangle=\alpha_{0}|00\rangle+\alpha_{1}|11\rangle.$ Since this state is the superposition of even-parity computational basis vectors, it is also said to have an even parity. When applied such an even-parity state, the
	parity measurement produces output $y=0$ with probability 1, and
	the post-measurement state equals the measured state. 
	Similarly, if the state $|\psi\rangle$ has an odd parity, i.e., it is given as $|\psi\rangle=\alpha_{0}|01\rangle+\alpha_{1}|10\rangle,$ lying in the subspace spanned by projector $\Pi_1$, the
	parity measurement produces output $y=1$ with probability 1, and
	the post-measurement state equals the measured state.
		
	
	\section{Observables}\label{sec:ch5:obs}

	
		 An observable $O$ assigns a numerical (real) value $o_{y}$ to each
		output $y$ of a projective measurement $\{\Pi_{y}\}_{y=0}^{N'-1}$. 
		 Therefore, by the Born rule (\ref{eq:ch5:Born}), measuring the observable $O$
	 returns the numerical value $o_{y}$ with probability $\textrm{tr}(\Pi_{y}\rho)$,
		when the input quantum state is $\rho$. We may express this as \begin{equation}\label{eq:ch5:probobs}  \Pr[\textrm{measurement of $O$ equals  }y]=\textrm{tr}(\Pi_{y}\rho)=\langle\psi|\Pi_{y}|\psi\rangle.
		\end{equation}
		
		An important role in many quantum algorithms is played by the \textbf{expected value, or the expectation, of an observable}. By (\ref{eq:ch5:probobs}), given an input quantum state
		$\rho$, the expectation of observable $O$, denoted as $\langle O\rangle_{\rho}$, can be computed as 
		\begin{equation}\label{eq:ch5:expobs}
		\langle O\rangle_{\rho}=\sum_{y=0}^{N'-1}o_{y}\textrm{tr}(\Pi_{y}\rho)=\textrm{tr}(O\rho),
		\end{equation}
		where we have defined the matrix
		\begin{equation}\label{eq:ch5:expobsmat}
		O=\sum_{y=0}^{N'-1}o_{y}\Pi_{y}.
		\end{equation} Matrix $O$ is Hermitian (since the projection matrices are also Hermitian);
		but not necessarily positive semi-definite, since the values $o_{y}$
		can be negative.  Specializing (\ref{eq:ch5:expobs}), for a pure input quantum state $|\psi\rangle$, the expectation of  observable $O$, denoted as $O\rangle_{|\psi\rangle}$, can be written
		as 
		\begin{equation}\label{eq:ch5:expobspure}
			\langle O\rangle_{|\psi\rangle}=\textrm{tr}(O|\psi\rangle\langle\psi|)=\langle\psi|O|\psi\rangle.
		\end{equation}
		
By the discussion above, we conclude that an observable $O$ can be described in terms of a Hermitian matrix $O$, justifying the use of the same notation for both concepts.  This is in the sense that knowing matrix $O$ allows us to compute the probability (\ref{eq:ch5:probobs}) of all possible outputs $\{o_y\}_{y=0}^{N'-1}$ of the observable, as well as the expectation of the observable via (\ref{eq:ch5:expobs}) or (\ref{eq:ch5:expobspure}). 
		
 In practice, by the no cloning theorem,	estimating the expectation $\langle O\rangle_{\rho}$ of an observable requires running the procedure that produces state $\rho$ multiple times. This way, one can carry out multiple projective measurements, one on each produced copy of state $\rho$,  in order 
		to obtain an empirical
		average of the observed values $o_y$.
		
		We have just seen that, given an observable $O$ in terms of a projective measurement $\Pi_y$ and associated numerical values $o_y$ for $y\in\{0,1,...,N'-1\}$, we can associate to it the Hermitian matrix (\ref{eq:ch5:expobsmat}). The latter fully describes the observable. We now consider the opposite direction of this association. To this end, fix an observable defined by a Hermitian matrix $O$. How can we assign to it projective
		measurement and corresponding numerical values $\{\Pi_y,o_y\}$?
		
		Since matrix $O$ is Hermitian, we can write an observable on $n$ qubits via the eigendecomposition
		as
		\begin{equation}\label{eq:ch5:obseig}
		O=\sum_{x=0}^{N-1}\lambda_{x}|v_{x}\rangle\langle v_{x}|,
		\end{equation}
		where the eigenvectors $|v_{0}\rangle,...,|v_{N-1}\rangle$ form an
		orthonormal basis and the associated eigenvalues $\lambda_{0},\lambda_{1},...,\lambda_{N-1}$
		are real. The eigenvectors  $|v_{0}\rangle,...,|v_{N-1}\rangle$  define the \textbf{eigenbasis} of observable $O$. Let us now write as $o_{y}$ with $y\in\{0,1,...,N'-1\}$, the $N'$ distinct values
		of the eigenvalues. Note that we have $N' \leq N$. The projective measurement associated with observable $O$ is then defined by the projectors \begin{equation}\label{eq:ch5:decproj}\Pi_{y}=\sum_{x:\textrm{ }\lambda_{x}=o_{y}}|v_{x}\rangle\langle v_{x}|
		\end{equation} for $y\in\{0,1,...,N'-1\}$. That is, each matrix $\Pi_y$ projects into the subspace spanned by all eigenvectors with eigenvalues equal to $o_y$. In fact, with this choice, the observable (\ref{eq:ch5:obseig}) can be written as in (\ref{eq:ch5:expobsmat}).
	
We finally observe that, for projectors of rank larger than one, the decomposition (\ref{eq:ch5:decproj}) is not unique. This is in the sense that any other set of orthonormal basis vectors for the subspace associated with the projector $\Pi_y$ could be used in lieu of the vectors $\{|v_x\rangle\}$. An example will be given in Sec. \ref{sec:ch5:multiqobs}. 


	\subsection{Examples of Single-Qubit Observables}
	In this subsection, we study a few examples of observables. 	For a single qubit $(n=1)$, consider first the \textbf{$Z$ observable}. Note that this is a valid observable, because the Pauli matrix $Z$ is Hermitian. Furthermore, the eigendecomposition (\ref{eq:ch5:obseig}) specializes as 
		\begin{equation}\label{eq:ch5:Zeig}
		Z=|0\rangle\langle0|-|1\rangle\langle1|.
		\end{equation}
		 Therefore, by the discussion in the previous subsection, measuring the $Z$ observable corresponds to a standard von Neumann measurement in the
		computational basis, in which the measurement output 0 is associated
		eigenvalue $o_0=+1$ and the measurement output 1 is associated eigenvalue
		$o_1=-1$. Note, in fact, that the computational basis is the eigenbasis of the $Z$ observable.
		
		Accordingly, standard single-qubit measurements are also referred to as \textbf{``measuring
		the $Z$ observable''}. 
		 For any pure state $|\psi\rangle=\alpha_{0}|0\rangle+\alpha_{1}|1\rangle$, by (\ref{eq:ch5:expobspure}), 
		we have the expectation
		\begin{equation}
		\langle Z\rangle_{|\psi\rangle}=\langle\psi|Z|\psi\rangle=(+1)|\langle0|\psi\rangle|^{2}+(-1)|\langle1|\psi\rangle|^{2}=|\alpha_{0}|^{2}-|\alpha_{1}|^{2}.
		\end{equation}
	

	
		 Consider now the \textbf{$X$ observable}. 
		 This is also a valid observable because the Pauli matrix $X$ is Hermitian, and it can be expressed
		with its eigendecomposition as
		\begin{equation}
		X=|+\rangle\langle+|-|-\rangle\langle-|.
		\end{equation}
		 Accordingly, this corresponds to a measurement in the $\{|+\rangle,|-\rangle\}$
		basis -- the eigenbasis of observable $X$ -- in which the measurement output 0 is associated eigenvalue
		$o_0=+1$ and the measurement output 1 is associated eigenvalue $o_1=-1$.
		Single-qubit measurements in the diagonal basis are also referred
		to as \textbf{``measuring the $X$ observable''}.
		 Finally, for any pure state $|\psi\rangle=\alpha_{0}|0\rangle+\alpha_{1}|1\rangle$,
		we have the expectation
		\begin{align}
			\langle X\rangle_{|\psi\rangle} & =\langle\psi|X|\psi\rangle=(+1)|\langle+|\psi\rangle|^{2}+(-1)|\langle-|\psi\rangle|^{2}\nonumber\\
			& =\frac{|\alpha_{0}+\alpha_{1}|^{2}}{2}-\frac{|\alpha_{0}-\alpha_{1}|^{2}}{2}.
		\end{align}
	
	\subsection{Multi-Qubit Observables}\label{sec:ch5:multiqobs}

		Let us now consider observables on any number $n$ of qubits. Following Sec. \ref{sec:ch2:Paulibasis}, any observable on $n$ qubits, i.e., any Hermitian matrix of dimension
		$N\times N$ with $N=2^{n}$, can be expressed
		as a linear combination with real coefficients of Pauli strings. To recall, let us write as $P_s$ with $s\in\{0,1,2,3\}$ a Pauli matrix, with \begin{equation}
			P_{0}=I,\textrm{ \ensuremath{P_{1}=X,\textrm{ \ensuremath{P_{2}=Y,\textrm{ and \ensuremath{P_{3}=Z}}}}}}.
		\end{equation} Let $s^{n}=[s_1,...,s_n]$ be a vector of integers $s_k\in\{0,1,2,3\}$ with $k=1,...,n$.  A string of $n$ Pauli matrices $P_{s^{n}}$ is given by the Kronecker product of $n$ Pauli matrices \begin{equation}\label{eq:ch5:Paulistring}P_{s^{n}}=P_{s_1} \otimes P_{s_2}  \otimes \cdots \otimes P_{s_n},
		\end{equation} where each matrix $P_{s_k}$ is one of the Pauli matrices $\{I,X,Y,Z\}$. An observable can be expressed as\begin{equation}\label{eq:ch5:obsPauli} O=\sum_{s^{n}\in\{0,1,2,3\}^{n}} a_{s^{n}} P_{s^{n}} 
	\end{equation} for some real coefficients $\{a_{s^{n}}\}$.

The decomposition (\ref{eq:ch5:obsPauli}) demonstrates that observables defined as strings of Pauli matrices play an important role. In fact, by (\ref{eq:ch5:obsPauli}), the expectation $\langle O\rangle_{\rho} $ of any observable $O$ can be expressed as the weighted sum, with weights $\{a_{s^{n}}\}$, of the expectations $\langle P_{s^{n}}\rangle_{\rho} $ of the $4^n$ Pauli observables: \begin{equation}\label{eq:ch5:expPauli}\langle O \rangle_{\rho}=\sum_{s^{n}\in\{0,1,2,3\}^{n}} a_{s^{n}} \langle{P_{s^{n}}}\rangle_{\rho}.
\end{equation}	 We  refer to an observable of the form (\ref{eq:ch5:Paulistring}) -- i.e., to an observable expressed as the Kronecker product of single-qubit observables -- as a separable observable.  As long as one is only interested in the numerical value of the observable, the measurement of a separable observable can be implemented via separate measurements across the $n$ qubits. However, if one is also interested in the post-measurement state, one should implement the associated projective measurement, which may require joint measurements. This is illustrated next with an example. 
	

	
		 Consider $n=2,$ and the observable $O=Z\otimes Z$. 
		By using the eigendecomposition (\ref{eq:ch5:Zeig}), this observable can be written as
		\begin{align}\label{eq:ch5:eigZ2}
			O & =(|0\rangle\langle0|-|1\rangle\langle1|)\otimes(|0\rangle\langle0|-|1\rangle\langle1|)\nonumber\\
			& =(\underbrace{|00\rangle\langle00|+|11\rangle\langle11|}_{\Pi_{0}})-(\underbrace{|01\rangle\langle01|+|10\rangle\langle10|}_{\Pi_{1}}).
		\end{align}
		 The expression (\ref{eq:ch5:eigZ2}) reveals the eigendecomposition of the observable $O$, which is characterized by two eigenvalues -- $+1$ and $-1$ -- with associated subspaces of dimension 2. Specifically, the eigenvector $+1$ is associated with the subspace spanned by the even-parity computational basis vectors, i.e., by projector $\Pi_0$; while the eigenvector $-1$ is associated with the subspace spanned by the odd-parity computational basis vectors, i.e., by projector $\Pi_1$. From the discussion in Sec. \ref{sec:ch5:obs}, it follows that  a measurement of the observable $O=Z\otimes Z$ corresponds
		to the parity projective measurement in which eigenvalue $+1$ is
		assigned to an even parity output, and eigenvalue $-1$ to an odd-parity
		output.
		
		 Therefore, from Sec. \ref{sec:ch5:paritymeas}, for an arbitrary pure state (\ref{eq:ch5:genstate}), 
		a measure of the observable $O=Z\otimes Z$ returns $+1$ with probability
		$|\alpha_{00}|^{2}+|\alpha_{11}|^{2}$ and $-1$ with probability
		$|\alpha_{01}|^{2}+|\alpha_{10}|^{2}$. As a result, measuring $Z\otimes Z$ is not the same as measuring the  $Z$ observable separately on the two qubits. In fact, this situation
		would correspond to a complete measurement (producing two cbits),
		and not to a parity projective measurement (producing one cbit). 
		
		That said, if one is only interested in the numerical output, and
		not also in the post-measurement state, it is possible to measure
		the $Z$ observable separately for the two qubits and multiply the
		outputs. In fact, measuring the $Z$ observables separately at the two qubits yields the cbits 
		$(1,1)$ with probability $|\alpha_{00}|^{2}$; $(-1,-1)$ with probability
		$|\alpha_{11}|^{2}$; $(1,-1)$ with probability $|\alpha_{01}|^{2}$;
		and $(-1,1)$ with probability $|\alpha_{10}|^{2}$.
		 Therefore, the product of the two observations equals $1$ with probability
		$|\alpha_{00}|^{2}+|\alpha_{11}|^{2}$ and $-1$ with probability
		$|\alpha_{01}|^{2}+|\alpha_{10}|^{2}$.
		
		We finally observe that the projectors defining the parity projective measurement can be expressed also in terms of other orthonormal bases. A useful example is the Bell basis (\ref{eq:ch2:Bell}). It can be, in fact, directly checked that the projectors in (\ref{eq:ch5:eigZ2}) can be expressed as	\begin{equation}
			\Pi_{0}=|\Phi^{+}\rangle\langle\Phi^{+}|+|\Phi^{-}\rangle\langle \Phi^{-}|
		\end{equation} and 
		\begin{equation}
			\Pi_{1}=|\Psi^{+}\rangle\langle\Psi^{+}|+|\Psi^{-}\rangle\langle \Psi^{-}|.
		\end{equation}
	
	\subsection{Compatible Observables}\label{sec:ch5:compatible}
	

		
			 Suppose that we are interested in measuring multiple observables --
			say $O_{1}$ and $O_{2}$ -- at the same time.
			We are specifically interested only in measuring the numerical outputs from the observables,
			i.e., the corresponding eigenvalues (and not the post-measurement states).  Can we do this with
			a single measurement?
			
			In this section, we have seen that an observable, say $O_{1}$, can be
			measured by carrying out a measurement of the given quantum state
			$|\psi\rangle$ in the eigenbasis of the
			observable. 
			 Once such a measurement is made, the post-measurement state is given
			by the eigenvector corresponding to the measured eigenvalue of $O_{1}$.
			 Therefore, once a measurement of an observable $O_{1}$ is made, one
			can generally no longer measure a second observable $O_{2}$ for the original
			quantum state $|\psi\rangle$. There is an exception to this rule -- namely, the 
			 case in which observable $O_{2}$ shares a common eigenbasis
			with $O_{1}$. (Note that the eigenbases are not unique when multiple
			eigenvectors correspond to the same eigenvalue.)
			 When this happens, we say that observables $O_{1}$ and $O_{2}$ are
			compatible.

		
			 To summarize, two observables $O_{1}$ and $O_{2}$ can be measured
			simultaneously with a single measurement -- and are hence \textbf{compatible} --if they share a common eigenbasis.
			 In fact, in this case, it is sufficient to carry out a single measurement
			in the given common eigenbasis. 
			 Mathematically, let 
			\begin{equation}
			O_{1}=\sum_{x=0}^{N-1}\lambda_{1,x}|v_{x}\rangle\langle v_{x}|\textrm{ and \ensuremath{O_{2}}=\ensuremath{\sum_{x=0}^{N-1}\lambda_{2,x}}|\ensuremath{v_{x}\rangle\langle v_{x}}|}
			\end{equation}
			two compatible observables. Note that they share the same eigenbasis
			$\{|v_{x}\rangle\}_{x=0}^{N-1}$ and they have generally different
			eigenvalues. 
			 Measuring both observables simultaneously is possible by carrying
			out a measurement in the eigenbasis $\{|v_{x}\rangle\}_{x=0}^{N-1}$.
			When obtaining the output $x$, the numerical output for observable
			$O_{1}$ is the eigenvalue $\lambda_{1,x}$ and for observable $O_{2}$
			we have the numerical output $\lambda_{2,x}.$ 
		
		
			 Let us consider some example. To start, consider two qubits and the observables \textrm{$O_{1}=Z\otimes I$}
			and $O_{2}=Z\otimes Z$, with the latter being the parity measurement.
			These two observables are compatible, and can be both measured via
			a standard measurement in the computational basis. As another example, any single-qubit observables applied to different qubits -- e.g., $O_1=X\otimes I$ and $O_1=I\otimes Z$ -- are compatible. 
			 In contrast, the observables $O_{1}=Z$ and $O_{2}=X$ on a single
			qubit are not compatible since they do not share an eigenbasis.
			 It follows that they cannot be measured simultaneously: One needs
			to prepare the state to be measured twice and implement two separate
			measurements for the two observables.
	
		
			It can be proved that two observables $O_{1}$ and $O_{2}$ are compatible if and only if
			they \textbf{commute}, that is, if and only if we have the equality
			\begin{equation}
			O_{1}O_{2}=O_{2}O_{1}.
			\end{equation}
			 This condition can provide an efficient way to check whether two observables
			are compatible. 
			
			 For instance, one can check that the observables \textrm{$Z\otimes I$}
			and $Z\otimes Z$ commute, since we have the equality
			\begin{equation}
			(Z\otimes I)(Z\otimes Z)=I\otimes Z=(Z\otimes Z)(Z\otimes I);
		\end{equation}
			while the two observables $Z$ and $X$ do not commute, since we have
			\begin{equation}
			XZ=iY=-ZX.
		\end{equation}
			 The latter condition describes operators that \textbf{anti-commute}, that is,
			that satisfy the equality $O_{1}O_{2}=-O_{2}O_{1}$.
			
			 The existence of incompatible observables is at the core of Heisenberg
			uncertainty principle, which indicates that for a given input quantum
			state $|\psi\rangle$, the product of the standard deviations of the
			observations of two measurements is lower bounded by a quantity that
			depends on the degree to which the two observables satisfy the condition
			above. 
	
	
	

%
\section{Projective Measurements as Partial Measurements}\label{sec:ch5:balanced}
	
		 As we have seen in Sec. \ref{sec:ch3:implany}, any complete measurement in an arbitrary basis $\{|v_{0}\rangle,...,|v_{N-1}\rangle\}$
		can be implemented as illustrated in Fig. \ref{fig:ch3:implany} by means of standard measurements in the computational basis. This is done by adding pre- and post-processing unitary transformations
		$U_{v_{x}\rightarrow x}=\sum_{x=0}^{N-1}|x\rangle\langle v_{x}|$ and $U_{v_{x}\rightarrow x}^{\dagger}=U_{x\rightarrow v_{x}}$ 
		that convert the given basis into the computational basis $\{|x\rangle\}_{x=0}^{N-1}$ and back, respectively.
		 Recall that measurements in the computational basis corresponds to projective
		measurements $\{\Pi_{x}=|x\rangle\langle x|\}_{x=0}^{N-1}$. As we discuss in this section, a similar approach can be used to implement more general projective
		measurements for an important special case. 
		
		 Specifically, given $n$ qubits,  we will focus on projective measurements that satisfy the following two conditions: \begin{itemize}
			\item the number of measurement outcomes, and hence the number of projectors, is $N'=2^{n'}$ for some integer for $n'\leq n$; 
			\item and all projectors $\Pi_y$, with $y\in\{0,1,...,2^{n'}-1\}$, have the same rank $N/N=2^{n-n'}$ with $N=2^n$.
		\end{itemize} We may refer to such projective measurements as ``balanced'', since the subspaces corresponding to the projectors defining it have the same dimension. Note that these conditions are satisfied by the parity measurement introduced in Sec. \ref{sec:ch5:paritymeas}.
		
		\subsection{Partial Measurements in the Computational Basis}\label{sec:ch5:balancedsimple}
		
		We start with a special case of the ``balanced'' projective measurements of interest in this section. To describe it, let us consider a system of
		$n$ qubits divided into two subsets of $n-n'$ and $n'$ qubits,
		with corresponding Hilbert spaces spanned by the computational bases
		$\{|x\rangle\}_{x=0}^{N/N'-1}$ and $\{|y\rangle\}_{y=0}^{N'-1}$
		with $N=2^{n}$ and $N'=2^{n'}$. 
		 We are interested in projective measurements defined by projection
		matrices
		\begin{equation}\label{eq:ch5:projsp}
		\Pi_{y}=\sum_{x=0}^{N/N'-1}|x,y\rangle\langle x,y|
		\end{equation}
		for $y\in\{0,1,...,N'-1\}$.
		 Accordingly, each subset $\mathcal{X}_{y}$ contains the indices of all basis vectors
		of the form $|x,y\rangle$ with a fixed $n'$-cbit string $y$. 
		
		The projective measurement defined by matrices (\ref{eq:ch5:projsp}) is indeed a ``balanced'' measurement, since we have $N'=2^{n'}$ possible measurement outputs and all projectors (\ref{eq:ch5:projsp}) have rank $N-N$. 
		 How can we implement a projective measurement of this type?
	


	
		 To make progress, recall the identity $|x,y\rangle \langle z,w|=|x\rangle\langle z| \otimes |y\rangle \langle w|$, we rewrite the projector (\ref{eq:ch5:projsp}) as 
		\begin{align}\label{eq:ch5:projsp1}
			\Pi_{y} & =\sum_{x=0}^{N/N'-1}|x,y\rangle\langle x,y|\nonumber\\
			& =\left(\sum_{x=0}^{N/N'-1}|x\rangle\langle x|\right)\otimes|y\rangle\langle y|\nonumber\\
			& =I\otimes|y\rangle\langle y|,
		\end{align}where the identity matrix is of dimension $N/N' \times N/N'$. 
		 The expression (\ref{eq:ch5:projsp1}) suggests that the projective measurement defined by predictors $	\{\Pi_{y}\}_{y=0}^{N'-1}$ can be implemented by making a partial measurement, as described in Sec. \ref{sec:ch3:partial}, that only applies to the second set of $n'$ qubits. This observation follows from the presence of the $N/N'\times N/N'$ identity matrix $I$, which indicates that states of the first $n-n'$ qubits are left unchanged by the projection; and by the presence of the $N' \times N'$ rank 1-projector $|y\rangle\langle y|=y$, which corresponds to a standard (von Neumann) measurement  applied  the second set of $n'$  qubits. 
		 
		 To prove the equivalence between ``balanced'' projective measurements defined by matrices (\ref{eq:ch5:projsp1}) and the partial measurement of the last $n'$ qubits, we need to show that the measurement probabilities  (\ref{eq:ch5:Bornpure}) and the post-measurement state (\ref{eq:ch5:postmeaspure}) coincide with the generalized Born rule (\ref{eq:ch3:genBorn}) and post-measurement state (\ref{eq:ch3:genBorn1}) (when applied to the last $n'$ qubits instead of the first qubit as in (\ref{eq:ch3:genBorn})-(\ref{eq:ch3:collgen})). 
		 
		 
		To this end, by the generalized Born rule (\ref{eq:ch3:genBorn}), the probability of observing $y \in \{0,1,...,2^{n'}-1\}$ for the partial measurement is given by \begin{align}
			(I\otimes\langle y|)|\psi\rangle\langle\psi|(I\otimes|y\rangle) & =\langle\psi|(I\otimes|y\rangle)(I\otimes\langle y|)|\psi\rangle \nonumber\\
			& =\mathrm{\langle\psi}|(I\otimes|y\rangle\langle y|)|\psi\rangle,
		\end{align}which coincides with (\ref{eq:ch5:Bornpure}). Similarly, by (\ref{eq:ch3:genBorn1}), when measurement $y$ is obtained, the post-measurement state of the overall system after the partial measurement of the second set of qubits is given as\begin{equation}
	\frac{(I\otimes\langle y|)|\psi\rangle}{\sqrt{\langle\psi|(I\otimes|y\rangle\langle y|)|\psi\rangle}}\otimes|y\rangle=\frac{(I\otimes|y\rangle\langle y|)|\psi\rangle}{\sqrt{\langle\psi|(I\otimes|y\rangle\langle y|)|\psi\rangle}}, 
	\end{equation}which coincides with (\ref{eq:ch5:postmeaspure}).

%		 consider a
%		general pure state
%		\begin{equation}
%			|\psi\rangle=\sum_{x=0}^{N/N'-1}\sum_{y=0}^{N'-1}\alpha_{x,y}|x,y\rangle
%		\end{equation} for the $n$ qubits. By the generalized Born rule (\ref{eq:ch3:genBorn}) defining partial measurements, measuring the second set of qubits 
%		yields the output $y\in\{0,1,...,N'-1\}$ 	with probability  $\langle\psi|\Pi_{y}|\psi\rangle=|\sum_{x=0}^{N/N'-1}\alpha_{x,y}|^{2}$, and the corresponding post-measurement state is
%		\begin{equation}
%			\left(\frac{1}{|\sum_{x=0}^{N/N'-1}\alpha_{x,y}|^{2}}\sum_{x=0}^{N/N'-1}\alpha_{x,y}|x,y\rangle\right)\otimes|y\rangle=\frac{\Pi_{y}|\psi\rangle}{\sqrt{\langle\psi|\Pi_{y}|\psi\rangle}}.
%		\end{equation}This recovers the Born rule (\ref{eq:ch5:Bornpure}) and the post-measurement state (\ref{eq:ch5:postmeaspure}) of projective measurements, concluding the proof of the claimed equivalence.
	 
		
		
We have hence concluded that projective measurements $	\{\Pi_{y}\}_{y=0}^{N'-1}$ of the form (\ref{eq:ch5:projsp}) are equivalent to measurements of the second set of $n'$ qubits in the computational basis $\{|y\rangle\}_{y=0}^{N'-1}$. This is illustrated in Fig.  \ref{fig:ch5:partproj}.

\begin{figure}
\begin{center}
				\begin{quantikz}
					\lstick[wires=2]{$\ket{\psi}$}& \qwbundle{n-n'} & \qw & \qw \rstick[wires=2]{$\frac{\Pi_{y}|\psi\rangle}{\sqrt{\langle\psi|\Pi_{y}|\psi\rangle}}$}\\
					& \qwbundle{n'} & \meter{$y$} & \qw  
				\end{quantikz}
		\end{center}\vspace{-0.4cm} \caption{ ``Balanced'' projective measurements $	\{\Pi_{y}\}_{y=0}^{N'-1}$ of the form (\ref{eq:ch5:projsp}) are equivalent to partial measurements involving only the second set of $n'$ qubits in the computational basis $\{|y\rangle\}_{y=0}^{N'-1}$.\label{fig:ch5:partproj}}
	\end{figure}

	\subsection{Projective Measurements as Partial Measurements}\label{sec:ch5:balancedcomp}
		 Let us study the more general case of ``balanced'' measurements as defined at the beginning of this section.  From Sec. \ref{sec:ch5:defproj}, any such projective measurement can be expressed in terms of an
		orthonormal basis $\{|v_{x'}\rangle\}_{x'=0}^{N-1}$, which is partitioned
		into $N'=2^{n'}$ subsets, each with $N/N'=2^{n-n'}$
		elements. In this subsection, we show that such measurements can be carried out by measuring only $n'$ qubits as in the architecture illustrated in Fig. \ref{fig:ch5:partproj}. The only caveat is that suitable pre- and post-measurement unitaries need to be put in place that carry out a specific change-of-basis transformation, generalizing the system in Fig. \ref{fig:ch3:implany}. The overall circuit, detailed in the rest of this subsection, is illustrated in Fig. \ref{fig:ch5:partialproj}. 
		
	The key underlying idea is to implement a change-of-basis unitary transformation $U_{v_{x'}\rightarrow x,y}$ performing the mapping \begin{equation}
		|v_{x'}\rangle \rightarrow |x,y\rangle
	\end{equation}
		between a vector $|v_{x'}\rangle$ belonging to the eigenspace of the $y$th projector ( $y\in\{0,1,...,N'-1\}$), i.e., with $x'\in\mathcal{X}_{y}$, 
		and the computational-basis vector $|x,y\rangle$, where $x\in\{0,1,...,N/N'-1\}$ is different for distinct vectors $|v_{x'}\rangle$. Accordingly, after the transformation  $U_{v_{x'}\rightarrow x,y}$ \begin{itemize}
		\item the state $|y\rangle$ of second set of $n'$ cbits indicates the index of the projector $\Pi_y$; and 
		\item the state $|x\rangle$ of the first set of $n-n'$ bits identifies a specific eigenstate within an  eigenbasis of the projector $\Pi_y$.
		\end{itemize}
		 Note that, for $N'=N$, this unitary  is equivalent to the change-of-basis transformation used in Fig. \ref{sec:ch3:implany}
		for complete measurements.
	


	\begin{figure}
\begin{center}
			\begin{quantikz}
				\lstick[wires=2]{$\ket{\psi}$}& \qwbundle{n-n'} & \qw & \gate[wires=2]{U_{v_{x'}\rightarrow x,y}}& \qw & \gate[wires=2]{U^{\dagger}_{v_{x'}\rightarrow x,y}}& \qw  \rstick[wires=2]{$\frac{\Pi_{y}|\psi\rangle}{\sqrt{\langle\psi|\Pi_{y}|\psi\rangle}}$}\\
				& \qwbundle{n'} &\qw & & \meter{$y$} & \qw & \qw 
			\end{quantikz}
	\end{center}\vspace{-0.4cm}\caption{Architecture implementing a general ``balanced'' projective measurement via a partial measurement of a subset of qubits. \label{fig:ch5:partialproj}}
	\end{figure}

	\subsection{Parity Measurements as Partial Measurements}\label{sec:ch5:partialprojpar}
		In this subsection, we specialize the architecture in Fig. \ref{fig:ch5:partialproj} to the parity measurement  with projection matrices $\{\Pi_{0},\Pi_{1}\}$ in  (\ref{eq:ch5:projsp}) on $n=2$ qubits. Note that we have $n'=1$ and that both projectors have rank equal to 2. Therefore, this is a ``balanced'' projective measurement as defined in this section.
		 
		 For the parity measurement, the transformation $U_{v_{x'}\rightarrow x,y}$ described in the previous subsection should map states
		$|00\rangle$ and $|11\rangle$ to $|00\rangle$ and $|10\rangle$,
		respectively; and states $|01\rangle$ and $|10\rangle$ to $|01\rangle$
		and $|11\rangle$, respectively. In fact, after this transformation, the state of the second qubit describes the index $y$ of the projector associated with the input eigenstate; while the state of the first qubit distinguishes the two input eigenstates within the eigenbasis of the same projector.   This transformation can be directly seen to be simply a CNOT gate.
		
		 Therefore, a parity measurement can be implemented by specializing the architecture in Fig. \ref{fig:ch5:partialproj} as in Fig. \ref{fig:ch5:partialprojpar}. In this circuit, 
		the second qubit first computes the parity of an input state in the computational basis before it is measured. 
	\begin{figure}
\begin{center}
			\begin{quantikz}
				\lstick[wires=2]{$\ket{\psi}$} & \qw & \ctrl{1}& \qw & \ctrl{1}& \qw  \rstick[wires=2]{$\frac{\Pi_{y}|\psi\rangle}{\sqrt{\langle\psi|\Pi_{y}|\psi\rangle}}$}\\
				& \qw & \gate{X}& \meter{$y$} & \gate{X} & \qw 
			\end{quantikz}
	\end{center}\vspace{-0.4cm}\caption{A quantum circuit implementing a parity measurement on two qubits. \label{fig:ch5:partialprojpar}}
	\end{figure}

	
		 To verify that the circuit in Fig. \ref{fig:ch5:partialprojpar} indeed produces the desired outcome, consider an arbitrary pure state
		\begin{equation}
		|\psi\rangle=\alpha_{00}|00\rangle+\alpha_{01}|01\rangle+\alpha_{10}|10\rangle+\alpha_{11}|11\rangle.
		\end{equation}
		 After the first CNOT  in Fig. \ref{fig:ch5:partialprojpar}, we have
		\begin{equation}
		C_{01}|\psi\rangle=\alpha_{00}|00\rangle+\alpha_{01}|01\rangle+\alpha_{10}|11\rangle+\alpha_{11}|10\rangle.
		\end{equation} Note that for each vector in the computational basis, i.e., every input vector of the form $|x,y\rangle$ with $x,y\in\{0,1\}$, the second qubit now reports the parity of the corresponding input. 
		By the generalized Born rule, measuring the second qubit produces the post-measurement state
		\begin{equation}
		\frac{1}{\sqrt{|\alpha_{00}|^{2}+|\alpha_{11}|^{2}}}(\alpha_{00}|00\rangle+\alpha_{11}|10\rangle)
		\end{equation}
		with probability $|\alpha_{00}|^{2}+|\alpha_{11}|^{2}$.
		 After the second CNOT, we finally get the desired post-measurement state (\ref{eq:ch5:postmeaspure}) as
		\begin{equation}
		\frac{\Pi_{0}|\psi\rangle}{\sqrt{\langle\psi|\Pi_{0}|\psi\rangle}}=\frac{1}{\sqrt{|\alpha_{00}|^{2}+|\alpha_{11}|^{2}}}(\alpha_{00}|00\rangle+\alpha_{11}|11\rangle).
		\end{equation}

	

%
\section{An Application of Projective Measurements: Quantum Error Correction}\label{sec:ch5:qec}
	
		 As an application of projective measurements, in this section, we briefly introduce the
		problem of quantum error correction. To this end, suppose that we have a ``channel'' that may ``flip'' a qubit, i.e.,
		that may, or may not, apply an $X$ operator to a qubit. 
		 A channel may represent, for instance, a communication link or noisy
		hardware. We would like to design an error correction scheme that is able to recover the original state of a qubit irrespective of whether a``bit flip'' was applied to the channel. Classically, the problem could be solved via redundancy: By copying and transmitting the information of interest multiple times through the channel, one can ensure some level of protection against channel errors. However, by the no cloning theorem, we cannot duplicate an unknown quantum
		state in order to increase robustness to noise.
		 
		 Notwithstanding the outlined limitation imposed by no cloning, is some form of error correction possible? We will see in this section that the answer to this question is affirmative, and that quantum error correction hinges on the implementation of projective measurements. It is emphasized that quantum error correction is a vast area of research, and that this section is only meant to illustrate some basic ideas pertaining the connection with projective measurements.
	
	\subsection{Bit-Flip Channel}
		 In order to illustrate the idea of quantum error correction,
		we consider a channel that may flip at most one out of three qubits. By this we mean that if we have three qubits in a
			general state 
			\begin{equation}
			|\psi_{in}\rangle=\sum_{x,y,z=0}^{1}\alpha_{x,y,z}|x,y,z\rangle
			\end{equation}
			at the input of the channel, the state $|\psi_{out}\rangle$
			at the output of the channel may be
			\begin{align}
			|\psi_{out}\rangle &=	 |\psi_{in}\rangle, \textrm{ or}\\
				|\psi_{out}\rangle &=\textrm{ \ensuremath{(X\otimes I\otimes I)|\psi_{in}\rangle=}}\sum_{x,y,z=0}^{1}\alpha_{x,y,z}|\bar{x},y,z\rangle, \textrm{ or}\\
				|\psi_{out}\rangle &= (I\otimes X\otimes I)|\psi_{in}\rangle=\sum_{x,y,z=0}^{1}\alpha_{x,y,z}|x,\bar{y},z\rangle, \textrm{ or}\\
				|\psi_{out}\rangle &= (I\otimes I\otimes X)|\psi_{in}\rangle=\sum_{x,y,z=0}^{1}\alpha_{x,y,z}\ensuremath{|x,y,\bar{z}\rangle},
			\end{align}
			where $\bar{x}=1\oplus x$, $\bar{y}=1\oplus y$, and $\bar{z}=z\oplus1$. The first state output $|\psi_{out}$ corresponds to the case in which no bit flip is applied; the second to the case in which the first qubit is flipped; and so on. Note that a bit flip corresponds to a Pauli string with a single $X$ operator in the position corresponding to the qubit affected by the flip.
	

		\subsection{Quantum Coding}
		 Let us assume that we have a qubit with an unknown state $|\psi\rangle=\alpha_{0}|0\rangle+\alpha_{1}|1\rangle$, which we would like to protect against the bit-flip channel described in the previous subsection. 
		 Specifically, we would like to encode this qubit in such a way that errors due to
		the channel can be corrected.
		 While duplication (cloning) is not possible, we can use the ``classical
		cloning'', or basis-copying, circuit introduced in Sec. \ref{sec:ch4:BC}.	The corresponding encoding circuit is shown in Fig. \ref{fig:ch5:enc}. Importantly, the resulting encoded state\begin{equation}
			\alpha_{0}|000\rangle+\alpha_{1}|111\rangle
		\end{equation}is different from a simple replica of the quantum state $|\psi\rangle$, which, by the no cloning theorem, cannot be realized for any input state $|\psi\rangle$. 
	
	\begin{figure}
\begin{center}
			\begin{quantikz}
				\lstick[wires=1]{$|\psi\rangle=\alpha_{0} \ket{0} + \alpha_{1} \ket{1}$} &[2mm] \qw & \ctrl{1} & \ctrl{2} & \qw & \qw  \rstick[wires=3]{$\alpha_{0} \ket{000} + \alpha_{1} \ket{111} \neq \ket{\psi}^{\otimes 3}$}\\
				\lstick{$\ket{0}$} & \qw & \gate{X} & \qw & \qw & \qw  \\
				\lstick{$\ket{0}$} & \qw & \qw & \gate{X} & \qw & \qw  
			\end{quantikz}
	\end{center}\vspace{-0.4cm}\caption{Quantum encoding for a quantum error correction scheme designed to correct at most one bit flip.\label{fig:ch5:enc}}
	\end{figure}


		 With this encoding circuit, the channel at hand can output one of the following
		states $|\psi_{out}\rangle$
		\begin{align*}
		|\psi_{out}\rangle &=	\alpha_{0}|000\rangle+\alpha_{1}|111\rangle & \textrm{ if there is no error}\\
		|\psi_{out}\rangle &=	\alpha_{0}|100\rangle+\alpha_{1}|011\rangle & \textrm{ if the first qubit is flipped}\\
		|\psi_{out}\rangle &=	\alpha_{0}|010\rangle+\alpha_{1}|101\rangle & \textrm{ if the second qubit is flipped}\\
		|\psi_{out}\rangle &=\alpha_{0}|001\rangle+\alpha_{1}|110\rangle & \textrm{ if the last qubit is flipped.}
		\end{align*}
	
\subsection{Quantum Decoding via a Projective Measurement}\label{sec:ch5:qecdec}
		 Based on the discussion in the previous subsection, if there is no error, the state lies in the two-dimensional
		space spanned by vectors $|000\rangle$ and $|111\rangle$. The projector into this subspace is given as 
		\begin{equation}\label{eq:ch5:qecdec1}
		\Pi_{00}=|000\rangle\langle000|+|111\rangle\langle111|.
		\end{equation}
		 If the first qubit is flipped, the state lies instead in the two-dimensional
		space spanned by vectors $|100\rangle$ and $|011\rangle$, whose corresponding projector is
		\begin{equation}
		\Pi_{10}=|100\rangle\langle100|+|011\rangle\langle011|.
		\end{equation} Similarly, if the second qubit is flipped, the state lies in the two-dimensional
		space spanned by vectors $|010\rangle$ and $|101\rangle$ with projector 
		\begin{equation}
		\Pi_{11}=|010\rangle\langle010|+|101\rangle\langle101|; 
		\end{equation}
		 and, if the third qubit is flipped, the state lies in the two-dimensional
		space spanned by vectors $|001\rangle$ and $|110\rangle$ with projector 
		\begin{equation}\label{eq:ch5:qecdec2}
		\Pi_{01}=|001\rangle\langle001|+|110\rangle\langle110|.
		\end{equation}
		 The reason for the specific choice of the  numbering of the projectors will be made clear later.
	

	
		 Based on the observations in the previous paragraph, applying the projective measurement $\{\Pi_{00},\Pi_{01},\Pi_{10},\Pi_{11}\}$ to the output of the quantum channel $|\psi_{out}\rangle$ allows us to correct one bit flip error by applying a NOT gate, i.e., a Pauli $X$ operator, to the
		first, second, or third qubit depending on the output of the measurement. Specifically, if the output of the measurement is $y=00$, no operation should be applied; if it is  $y=10$, a NOT gate should be applied to the first qubit; and so on. Crucially, the success of this operation in correcting a bit flip hinges on the use of a projective measurement. In fact, with a complete measurement, the state
		of the qubits at the output of the channel would collapse, destroying the original superposition
		state $|\psi\rangle=\alpha_{0}|0\rangle+\alpha_{1}|1\rangle.$ In contrast, as we have seen in this section, the projective measurement leaves unchanged quantum states that lie within the subspace corresponding to each projector.
		 
		 In order to apply error correction, one should therefore implement a NOT (Pauli $X$) gate depending on the output of the projective measurement $\{\Pi_{0},\Pi_{01},\Pi_{10},\Pi_{11}\}$. To make this possible, one should have both measurement output and post-measurement state 
		 simultaneously encoded in the state of the quantum system. This way, at the next computation step, the measurement output can be used to determine the operation to be applied to the post-measurement state.  This is typically done by adding so-called \textbf{ancilla} qubits, whose state encodes the output $y$ of the measurement. This will be discussed in the next section.
		 
		 

	\subsection{Key Principles of Quantum Error Correction}
		 Before discussing the implementation of the error-correcting circuit through the introduction of ancillas,
		it is useful to reiterate and generalize the principle underlying
		quantum error correction.
		 Quantum error correction aims at protecting the unknown state of $k$
		qubits -- $k=1$ in the example above -- by encoding such state
		into the state of $n$ qubits -- $n=3$ in the example. Note that the unknown state lies in a Hilbert space of dimension $2^k$. 
		 As a result of encoding, the state of the encoded qubit occupies a $2^{k}$-dimensional
		subspace in the $2^{n}$ Hilbert space corresponding to the $n$ encoded
		qubits.
		
		Encoding is designed in such a way that any possible distinct error causes the state
		of the encoded qubits to lie in an orthogonal subspace of dimension
		$2^{k}$.  A projective measurement defined by projection matrices in these orthogonal
		subspaces can hence distinguish among the different types of errors, while leaving the state
		within each subspace undisturbed.
		
		If there are $m$ different errors -- $m=3$ in the example -- the design requirement outlined in the previous paragraph calls for a number of encoded qubits, $n$,  satisfying the condition \begin{equation}\label{eq:ch5:Hamming}2^{n}\geq2^{k}(1+m).
		\end{equation} In fact, the Hilbert space of the encoded qubits should include $m+1$ orthogonal subspaces, each of dimension $2^k$, with one subspace corresponding to the absence of errors on the channel and the others accounting for each of the $m$ types of errors.  When further elaborated on by accounting for all possible error types on single qubits, the inequality (\ref{eq:ch5:Hamming}) yields the so called \textbf{quantum Hamming bound}. In the example studied in this section, we have $k=1$, $n=3$, and $m=3$, which satisfies this condition with equality as  $2^{3}=2^{1}(1+3)=8.$
		 
		 \subsection{Quantum Error Detection}
		
		As a less powerful alternative to quantum error correction, it is also possible to design \textbf{quantum error detection}
		schemes, whereby errors are only detected and not corrected. With error detection, one only determines, possibly with some probability, the presence of an error, without necessarily identifying, and correcting, the specific error. With reference to the discussion in the previous subsection, for quantum error detection, there is no need for the $m$ subspaces corresponding
		to different errors to be orthogonal. In fact, it is sufficient that each type of error cause the post-channel state to lie in the \emph{same} subspace, as long as the latter is orthogonal to that encompassing the encoded state.
		
		 To implement a quantum error detector, one can define an observable that assigns the $+1$ eigenvalue to the ``no-error'' projector $\Pi_0$ describing the subspace spanned by the code, and a $-1$ eigenvalue to the subspace $\Pi_1$ orthogonal to $\Pi_0$. This way, if a measurement of the observable returns $-1$, one can conclude with certainty that an error has occurred, while, if the output is $+1$, the state can be concluded to be unaffected by errors.  We refer to Sec. \ref{sec:ch5:Pauliobs} for a discussion on how to implement binary measurements in the common case in which the projectors $\Pi_0$ and $\Pi_1$ are defined in terms of Pauli strings. In this regard, we also point the reader to the field of \textbf{stabilizer codes}, whereby a code is described by the observables defined by Pauli strings. 
		 
		 %This line of thinking leads to the formalism of \textbf{stabilizer codes}, whereby a code is described by the observables defined by Pauli strings  with the mentioned property in terms of eigenvalues and eigenvectors. For example, for the code considered here the set of such observables, known as the stabilizer, is given as $\{I \otimes I \otimes I, Z \otimes Z \otimes I,$ $I \otimes Z \otimes Z, Z \otimes I \otimes Z\}$.
	

%
\section{Implementing Projective Measurements with Ancillas}
	
	As we have discussed in the previous section, for some applications, including quantum error correction, it is useful to have the output of the measurement and the post-measurement state simultaneously encoded in the state of separate quantum systems. This requires adding to the system a set of \textbf{ancilla} qubits, whose state encodes the measurement's output. We will hence refer to such measurements as ``measurements with ancillas''. In this section, we discuss how to implement measurements with ancillas, starting with the case of complete measurements and then generalizing to projective measurements.
	
	\subsection{Complete Measurements with Ancillas}
		As we demonstrate in this subsection, we can implement a complete von
		Neumann measurement with ancillas in any orthonormal basis $\{|v_{0}\rangle,...,|v_{N-1}\rangle\}$ for a system of $n$ qubits ($N=2^n$) via the circuit shown in Fig. \ref{fig:ch5:ancilla}. The circuit operates on the $n$ qubits being measured -- in an arbitrary state $\psi\rangle_n$ -- as well as on $n$ ancilla qubits initialized in the ground state $|0\rangle_n$. 
		
	The circuit in Fig. \ref{fig:ch5:ancilla} first applies the change-of-basis unitary $U_{v_x \rightarrow x}$ to the $n$ qubits being measured as in Fig. \ref{fig:ch3:implany}. As detailed in Sec. \ref{sec:ch3:implany}, this unitary maps each vector $|v_{x}\rangle$ of the basis defining the measurement to the vector $|x\rangle$ in the computational basis.  Unlike the circuit in Fig. \ref{fig:ch3:implany}, the first set of $n$ qubits are not directly measured. Rather, they are fist ``copied''  to the second set of $n$ qubits, i.e., to the ancilla qubits, and then the ancillas are measured, before the final inverse change-of-basis transformation  $U_{x \rightarrow v_x}$ is applied to the first $n$ qubits. 
	
	More precisely, after the first change-of-basis unitary, we apply a basis-copying transformation (see Sec. \ref{sec:ch4:BC}), i.e.,
	\begin{equation}
		U_{BC}=\sum_{x=0}^{N-1}\sum_{y=0}^{N-1}|x,x\oplus y\rangle\langle x,y|,
	\end{equation}
	where $\{|y\rangle\}_{y=0}^{N-1}$ represents the computational basis
	for the Hilbert space of the ancillas. The unitary $U_{BC}$  has the effect of ``cloning'' the vectors in the computational basis from the first $n$ qubits to the ancillas. 
			

			
			\begin{figure}
			\begin{center}
				\begin{quantikz}
					\lstick{$\ket{\psi}_{n}$} & \qw & \gate{U_{v_{x}\rightarrow x}} & \gate[wires=2]{U_{BC}} & \qw & \qw & \gate{U_{x\rightarrow v_{x}}} & \qw \rstick{$\ket{v_x}$}\\
					\lstick{$\ket{0}_{n}$} & \qw & \qw &  & \qw & \meter{$x$} & \qw & \qw \rstick{$\ket{x}$}
				\end{quantikz}
		\end{center}\vspace{-0.4cm}\caption{Complete measurement in an arbitrary orthonormal basis $\{|v_{0}\rangle,...,|v_{N-1}\rangle\}$ with ancillas. The ancillas qubits are the second set of $n$ qubits initialized to the ground state $|0\rangle_n$. Unlike the circuit in Fig. \ref{fig:ch3:implany}, this architecture produces both the post-measurement state (for the first $n$ qubits) and the output of the measurement, $x\in \{0,1,...,2^{n}-1\}$, with the latter encoded in the state of the $n$ ancilla qubits. \label{fig:ch5:ancilla}}
	\end{figure}
	
	
For an arbitrary pure state $|\psi\rangle=\sum_{x=0}^{N-1}\alpha_{x}|v_{x}\rangle$
			of the $n$ qubits being measured, and hence a global state $\sum_{x=0}^{N-1}\alpha_{x}|x,0\rangle$
			after the change-of-basis transformation $U_{v_{x}\rightarrow x}$, the basis-copying
			unitary operator yields the state
			\begin{equation}
			U_{BC}(U_{v_{x}\rightarrow x}\otimes I)\sum_{x=0}^{N-1}\alpha_{x}|v_{x},0\rangle=\sum_{x=0}^{N-1}\alpha_{x}|x,x\rangle.
			\end{equation} Therefore, by the generalized Born rule, measuring the ancillas yields
			the separable post-measurement state $|x,x\rangle$ with probability
			$|\alpha_{x}|^{2}.$ Finally, this produces the separable state $|v_{x},x\rangle$ after
			the inverse change-of-basis transformation $U_{x\rightarrow v_{x}}$. This calculation demonstrates that the architecture in Fig. \ref{fig:ch5:ancilla} implements a von Neumann measurement in the basis $\{|v_{0}\rangle,...,|v_{N-1}\rangle\}$. 
		Note that this is a selective measurement in the sense that
			it retains the value $x$ of the measurement.
	

\subsection{Projective Measurements with Ancillas}
	
We now generalize the architecture in Fig. \ref{fig:ch5:ancilla} to the ``balanced'' projective measurements introduced in Sec. \ref{sec:ch5:balanced}. To see how, we consider here the class of ``balanced'' projective measurements studied in Sec. \ref{sec:ch5:balancedsimple}, which are characterized by the projection matrices (\ref{eq:ch5:projsp1}).  This is without loss of generality since, as seen in Sec. \ref{sec:ch5:balancedcomp}, by adding suitable pre- and post-measurement transformations, one can implement a general ``balanced'' measurement from a measurement defined by matrices (\ref{eq:ch5:projsp1}). We will provide an example of this procedure at the end of this subsection.

As discussed in Sec. \ref{sec:ch5:balancedsimple}, this projective measurement amounts to the partial measurement of the second set of $n'$ qubits out of the total $n$ qubits being measured. Therefore, the measurement can be implemented via a generalization of the architecture introduced in the previous subsection whereby only the second set of $n'$ qubits are ``copied'' -- in the computational basis -- to the ancillas. 

Specifically, as illustrated in Fig. \ref{fig:ch5:ancilla1}, the measurement involves the introduction of $n'$ ancilla qubits, which are used to encode the output index $y \in \{0,1,...,2^{n'}-1\}$.  The basis-copying unitary $\tilde{U}_{BC}$
``copies'' only the second set of qubits as controlling qubits onto the ancillas. This amounds to a unitary transformation that maps each vector $|x\rangle \otimes |y\rangle \otimes |0\rangle=|x,y,0\rangle$ -- with $x\in\{0,1,...,2^{n-n'}-1\}$, $y\in\{0,1,...,2^{n'}-1\}$, and $|0\rangle$ being the initial ground state of the $n'$ ancillas -- into the state $|x,y,y\rangle$. 
	
		
		\begin{figure}
		\begin{center}
				\begin{quantikz}
					\lstick{$\ket{\psi}_{n}$} &[2mm] \qw & \gate[wires=2]{\tilde{U}_{BC}} & \qw & \qw & \qw  \rstick{$\frac{\Pi_{y}|\psi\rangle}{\sqrt{\langle\psi|\Pi_{y}|\psi\rangle}}$}\\
					\lstick{$\ket{0}_{n'}$} & \qw &  & \qw & \meter{$y$} & \qw  \rstick{$\ket{y}$}
				\end{quantikz}
		\end{center}\vspace{-0.4cm}\caption{A ``balanced'' projective measurement defined by projectors $\{\Pi_y\}_{y=0}^{2^{n'}-1}$ in (\ref{eq:ch5:projsp1}) with ancillas. As for Fig. \ref{fig:ch5:ancilla}, the architecture produces both the post-measurement state (for the first $n$ qubits) and the output of the measurement, $y\in\{0,1,...,2^{n'}-1\}$, with the latter encoded in the state of the $n'$ ancillas qubits.  \label{fig:ch5:ancilla1}}
	\end{figure}


	
		As an example, consider again the parity measurement $\{\Pi_{0},\Pi_{1}\}$ introduced in Sec. \ref{sec:ch5:paritymeas}. Since
		there are only two values for the measurement ($n'=1$), it is sufficient
		add a single ancilla qubit. As discussed in Sec. \ref{sec:ch5:partialprojpar}, in order to implement this measurement via measurements in the computational basis,  one can pre- and post-process the state to be measured with the change-of-basis unitaries illustrated in Fig. \ref{fig:ch5:partialprojpar}. These amount to a simple CNOT gate. Therefore, as detailed in Fig. \ref{fig:ch5:parityanc}, the first step is to apply a CNOT gate to the two qubits being measured, which are initially in state $|\psi\rangle$. Then, as in the architecture in Fig. \ref{fig:ch5:ancilla1}, one applies a basis-copying circuit from the second qubit to the ancilla, followed by a measurement of the ancilla. The basis-copying circuit also amounts to a CNOT gate.  Finally, the initial change-of-basis unitary is inverted with a last CNOT gate. It can be directly checked that the circuit in Fig. \ref{fig:ch5:parityanc} indeed produces the output $y$ and corresponding post-measurement state with the probability (\ref{eq:ch5:parityp1})-(\ref{eq:ch5:parityp2}). 
		\begin{figure}
	\begin{center}
			\begin{quantikz}
				\lstick[wires=2]{$\ket{\psi}$} &[2mm] \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1}& \qw \rstick[wires=2]{$\frac{\Pi_{y}|\psi\rangle}{\sqrt{\langle\psi|\Pi_{y}|\psi\rangle}}$} \\
				&[2mm] \qw & \gate{X} & \ctrl{1} & \qw & \qw &\gate{X}&\qw\\
				\lstick{$\ket{0}$} & \qw & \qw & \gate{X} & \qw & \meter{$y$} &\qw& \qw \rstick{$\ket{y}$}
			\end{quantikz}
	\end{center}\vspace{-0.4cm}\caption{An ancilla-based implementation of the parity measurement introduced in Sec. \ref{sec:ch5:paritymeas}. The circuit in the figure specializes the general architecture in Fig. \ref{fig:ch5:ancilla1}, which applies to any ``balanced'' projective measurement as introduced in Sec. \ref{sec:ch5:balanced}. \label{fig:ch5:parityanc}}
\end{figure}

	
		The architecture in Fig. \ref{fig:ch5:ancilla1} provides a solution to implement any ``balanced'' projective measurement -- and hence also any complete measurement in any basis -- with ancillas. That said, it may not necessarily provide the most efficient circuit. For example, for the parity measurement discussed in the last paragraph, the circuit in Fig. \ref{fig:ch5:parityanc}  can be directly seen to be equivalent to that in Fig. \ref{fig:ch5:paritys}, while requiring only two CNOT gates. The operation of the circuit in Fig. \ref{fig:ch5:paritys} has the interesting interpretation that the ancilla qubit computes the parity -- separately on each 
		computational basis state -- of the two qubits being measured. This is done via the two CNOT gates. In fact, if the two qubits being measured are in state $|x,y\rangle$, with $x,y\in\{0,1\}$, the state of the ancilla qubit after the two CNOT gates is $|x\oplus y\rangle$.
	\begin{figure}
\begin{center}
			\begin{quantikz}
				\lstick[wires=2]{$\ket{\psi}$} &[2mm] \qw & \ctrl{2} & \qw & \qw & \qw \rstick[wires=2]{$\frac{\Pi_{y}|\psi\rangle}{\sqrt{\langle\psi|\Pi_{y}|\psi\rangle}}$} \\
				&[2mm] \qw & \qw & \ctrl{1} & \qw & \qw \\
				\lstick{$\ket{0}$} & \qw & \gate{X} & \gate{X} & \meter{$y$} & \qw  \rstick{$\ket{y}$}
			\end{quantikz}
	\end{center}\vspace{-0.4cm}\caption{An equivalent implementation of the parity measurement with ancilla. Unlike the equivalent circuit in Fig. \ref{fig:ch5:parityanc}, here the ancilla qubit -- initialized in the ground state -- computes the parity of the two qubits being measured, separately for each computational basis state, via the two CNOTs. \label{fig:ch5:paritys}}
\end{figure}
%
\subsection{Application to Quantum Error Correction}
	
Let us now return to the problem of designing a decoding circuit for the quantum error correction code introduced in Sec. \ref{sec:ch5:qec}. As we have seen in Sec. \ref{sec:ch5:qecdec},  the decoder carries out the projective measurement $\{\Pi_{00},\Pi_{01},\Pi_{10},\Pi_{11}\}$ with projection matrices in (\ref{eq:ch5:qecdec1})-(\ref{eq:ch5:qecdec2}). According to the discussion in this section, this measurement can be implemented by introducing two ancilla qubits ($n'=2$), since there are four possible outcomes. The resulting circuit is illustrated in Fig. \ref{fig:ch5:qdec}, and is detailed next.

Generalizing the circuit in Fig. \ref{fig:ch5:paritys}, the decoder takes as input the post-channel state, and computes the parity -- in the computational basis -- of the first and second pair of qubits in the post-channel state. Specifically, the first ancilla qubit measures the parity of the first pair, and the second ancilla qubit of the second pair. The outputs $y_0, y_1\in \{0,1\}^{2}$ of the measurement of the ancillas (in the computational basis) are then used to determine whether an $X$ gate should be applied to the any of the three input qubits. 

It can be demonstrated in a manner similar to Fig. \ref{fig:ch5:paritys} that the measurement circuit in Fig. \ref{fig:ch5:qdec} implements the projective measurement $\{\Pi_{00},\Pi_{01},\Pi_{10},\Pi_{11}\}$. Furthermore, the shortcut notation $X^{ab}$ in Fig. \ref{fig:ch5:paritys} indicates that an $X$ gate is applied when $a=b=1$, recovering the decoding rule described in Sec. \ref{sec:ch5:qec}. Accordingly, as long as the channel applies at most one bit flip, the corrected state $\ensuremath{|\psi_{corr}\rangle\alpha_{0}|000\rangle+\alpha_{1}|111\rangle}$ equals the encoded state $|\psi_{in}$.

			
			\begin{figure}
			\begin{center}
				\begin{quantikz}
					\lstick[wires=3]{$\ket{\psi_{out}}$} \qw & \ctrl{3} & \qw & \qw & \qw & \qw & \qw & \gate{X^{y_0\bar{y}_1}} &\qw \rstick[wires=3]{$\ket{\psi_{corr}}$}\\
					\qw & \qw & \ctrl{2} & \ctrl{3} & \qw  & \qw & \qw & \gate{X^{y_0y_1}} &\qw\\
					\qw & \qw & \qw & \qw & \ctrl{2}  & \qw & \qw &\gate{X^{\bar{y}_0y_1}} &\qw\\
					\lstick{$\ket{0}$}\qw & \gate{X} & \gate{X} & \qw & \qw  & \qw & \meter{$y_0$}& \qw & \qw & \qw\\
					\lstick{$\ket{0}$}\qw & \qw & \qw & \gate{X} & \gate{X}  & \qw & \meter{$y_1$}& \qw & \qw & \qw
				\end{quantikz}
		\end{center}\vspace{-0.4cm} \caption{Decoder for the quantum error correction code described in Sec. \ref{sec:ch5:qec}. The decoder uses the output of the measurement encoded in the state of the two ancilla qubits (the last two qubits) in order to determine the operation applied on the encoded qubits (the first three qubits) at the next computation step.\label{fig:ch5:qdec}}
	\end{figure}
	
	In closing this subsection, we note that it is also possible to implement quantum error correction
			without an explicit measurement of the ancillas through the use of
			three-qubit gates, namely Toffoli gates.
		
		
		
		\subsection{Implementing Measurements with Ancillas for Pauli Strings Observables}\label{sec:ch5:Pauliobs}
		 In this subsection, we focus on the implementation of an important class of binary 
				projective measurements $\{\Pi_{0},\Pi_{1}\}$ with ancillas that find applications in quantum error correction and detection. Specifically, we  study measurements
				of observables defined as a string of Pauli operators \begin{equation}\label{eq:ch5:Ps}P=P_{1}\otimes P_{2}\cdots\otimes P_{n}
				\end{equation}where we have $P_k \in \{I,X,Y,Z\}$ with $k=1,2,...,n$.

		 The first observation is that, since Pauli matrices $P_k \in \{X,Y,Z\}$, have eigenvalues $+1$ and $-1$, the Pauli string $P$ also has eigenvalues $+1$ and $-1$. This is because the eigenvalues of the Kronecker product in (\ref{eq:ch5:Ps}) are equal to the product of the eigenvalues of the individual matrices being multiplied. It follows that any observable of the form (\ref{eq:ch5:Ps}) has the eigendecomposition
				\begin{equation}
				P=P_{1}\otimes P_{2}\cdots\otimes P_{n}=\Pi_{0}-\Pi_{1},
				\end{equation}
				where $\Pi_{0}$ is the projector associated with the eigenspace of
				eigenvalue $+1$ and $\Pi_{1}$ is the projector associated with the
				eigenspace of eigenvalue $-1.$ 
			 Furthermore, we can express these projectors directly in terms of the Pauli string (\ref{eq:ch5:Ps})  as  
				\begin{align}\label{eq:ch5:PP}
					\Pi_{0} & =\frac{1}{2}\left(I+P\right)\nonumber\\
					\Pi_{1} & =\frac{1}{2}\left(I-P\right).
				\end{align}
		
The projective measurement corresponding to the measurement of observable (\ref{eq:ch5:Ps}) can be seen to be ``balanced'' in the sense described in Sec. \ref{sec:ch5:balanced}. Therefore, the general architecture in Fig. \ref{fig:ch5:ancilla1} could be used to implement it with $n'=1$ ancilla qubit. Using the circuit in Fig. \ref{fig:ch5:ancilla1} would require, however, to specify the basis-copying circuit $\tilde{U}_{BC}$. The main point of this subsection is that such measurements can be also implemented with the circuit illustrated in Fig. \ref{fig:ch5:Pauliobs}, which directly depends on the Pauli string $P$.

\begin{figure}
\begin{center}
						\begin{quantikz} \lstick{$|\psi\rangle$}	\qw & \qw & \gate{P} &  \qw & \qw & \qw \rstick{$\frac{\Pi_y |\psi\rangle}{\sqrt{\langle \psi |\Pi_y |\psi\rangle}}$}\\	
							\lstick{$|0\rangle$} \qw & \gate{H} &\ctrl{-1} & \gate{H} & \meter{$y$} & \qw	\rstick{$|y\rangle$}	\end{quantikz}
				\end{center}\vspace{-0.4cm} \caption{A quantum circuit that implements the measurement of a Pauli string observable (\ref{eq:ch5:Ps}). \label{fig:ch5:Pauliobs}}
		\end{figure}

		%
	
	In the circuit in Fig. \ref{fig:ch5:Pauliobs}, we add an ancilla qubit in state $|0\rangle$ to the $n$ qubits to be measured. The ancilla goes through a Hadamard gate, and then a controlled-$P$ gate is applied across the $n+1$ qubits. The controlled-$P$ gate is defined as\begin{equation} 
		I\otimes|0\rangle\langle0|+P\otimes|1\rangle\langle1|.
		\end{equation}Accordingly, on the ``branch'' of the computation in which the ancilla is in state $|0\rangle$ no operation is applied to the $n$ qubits; while, on the ``branch'' of the computation in which the ancilla is in state $|1\rangle$ we apply the separable operator defined by the Pauli string $P$ to the $n$ qubits. Another Hadamard gate is then applied to the ancilla, and finally a standard measurement of the ancillas is made. 
	
	To see that the circuit in Fig. \ref{fig:ch5:Pauliobs} implements the desired measurement of the observable $P$, we observe that the	state prior to the measurement is given as 
				\begin{align}
					& \frac{1}{2}\left(I+P\right)|\psi\rangle|0\rangle+\frac{1}{2}\left(I-P\right)|\psi\rangle|1\rangle \nonumber\\
					& =\Pi_{0}|\psi\rangle|0\rangle+\Pi_{1}|\psi\rangle|1\rangle,
				\end{align}where we have used the equalities in (\ref{eq:ch5:PP}). 
		Therefore, by the generalized Born rule, we have that the output state
				is given by 
				\begin{align}
					\frac{\Pi_{x}|\psi\rangle|x\rangle}{\sqrt{\langle\psi|\Pi_{x}|\psi\rangle}} & \textrm{ w.p. \ensuremath{\langle\psi}|\ensuremath{\Pi_{x}}|\ensuremath{\psi\rangle}},
				\end{align}as desired.



%
\section{POVM Measurements}\label{sec:ch5:povm}
	
		 As we have seen in the previous section, general projective measurements can be implemented
		by adding ancillas in ground state, applying an entangling operator,
		namely the basis-copying circuit, and then measuring the ancillas (see Fig. \ref{fig:ch5:ancilla1}). In this section, we address the following question: 
		 What if we applied a more general entangling operator, i.e., an arbitrary
		unitary matrix, to the overall system including the ancillas, and
		then measured the ancillas (in a selective way)? As we will detail, this lead to the most general form of (selective) measurements, namely positive operator-valued measurement (POVM).
	

%
\subsection{Deriving POVM Measurements}
	
		 To derive POVMs, let us consider a system of $n$ qubits with $n'$
		ancillas, with the latter being initially in the ground state $|0\rangle.$
		 If the system of $n$ qubit is in state $|\psi\rangle$, the overall
		system is hence in the separable state $|0,\psi\rangle=|0\rangle\otimes|\psi\rangle.$
		Note that, unlike what we have done in the rest of this chapter, here we append the ancillas in front of the $n$-qubit state in order to simplify the derivations that
		follow.  The setting under study is illustrated in Fig. \ref{fig:ch5:povm}.
		\begin{figure}
		\begin{center}
				\begin{quantikz}  				\lstick{$\ket{0}\bra{0}$} & \gate[wires=2]{U}\qwbundle{} & \qwbundle{} & \qw \\ 				\lstick{$\rho$} & \qwbundle{} &  \meter{$y$} \qwbundle{} & \qw\rstick{$\ket{y}$  w.p. $\textrm{tr}(M_{y}\rho)$} 			\end{quantikz}
		\end{center}\vspace{-0.4cm}\caption{A POVM describes a situation in which the system of interest interact through a unitary $U$ with ancilla qubits, initially in the ground state $|0\rangle$, and then the ancillas are measured (in a selective manner). \label{fig:ch5:povm}}
	\end{figure}

		Applying a unitary matrix $U$ to the overall system we get 
		\begin{equation}
		U|0,\psi\rangle=\left[\begin{array}{cccc}
			U_{00} & U_{01} & \cdots & U_{0,N'-1}\\
			U_{10} & U_{11} & \cdots & U_{1,N'-1}\\
			\vdots & \vdots &  & \vdots\\
			U_{N'-1.0} & U_{N'-1,1} & \cdots & U_{N'-1,N'-1}
		\end{array}\right]\left[\begin{array}{c}
			|\psi\rangle\\
			0\\
			\vdots\\
			0
		\end{array}\right],
		\end{equation}
		where the matrices $U_{km}$ are of size $N\times N$, with $N=2^{n}$, and we set $N'=2^{n'}.$ It follows that the output of the unitary operation is
		\begin{equation}
		U|0,\psi\rangle=\left[\begin{array}{c}
			U_{00}|\psi\rangle\\
			U_{10}|\psi\rangle\\
			\vdots\\
			U_{N'-1,0}|\psi\rangle
		\end{array}\right]=\sum_{y=0}^{N'-1}|y\rangle\otimes U_{y0}|\psi\rangle.
		\end{equation}
		 Furthermore, by the unitarity of matrix $U$, i.e., by the equality
		$U^{\dagger}U=I$, we have the condition 
		\begin{equation}\label{eq:ch5:povm1}
		\sum_{y=0}^{N'-1}U_{y0}^{\dagger}U_{y0}=I.
		\end{equation}


		 Now, if we measure the ancillas in the computational basis, by the
		generalized Born rule, we get 
		\begin{align}
		\Pr[\textrm{measurement output equals  }y]&=\langle\psi|U_{y0}^{\dagger}U_{y0}|\psi\rangle\\&=\textrm{tr}(M_{y}\rho),
		\end{align}
		where we have defined matrix $M_{y}=U_{y0}^{\dagger}U_{y0}$ and the density matrix 
		$\rho=|\psi\rangle\langle\psi|$. 
		 Furthermore, the post-measurement (density) state is 
		\begin{equation}
		\frac{U_{y0}\rho U_{y0}^{\dagger}}{\textrm{tr}(M_{y}\rho)}.
		\end{equation}
	

%
\subsection{Defining a POVM}
	
		 Generalizing the derivation above, a POVM is defined by a set of positive
		semi-definite matrices $M_{y}$ with $y\in\{0,1,...,N'-1\}$, with
		$N'$ generally different from $N$ -- and possibly larger than $N$
		-- such that the following condition -- from (\ref{eq:ch5:povm1}) -- applies
		\begin{equation}
		\sum_{y=0}^{N'-1}M_{y}=I.
		\end{equation}
		 A POVM stipulates that output $y$ is observed with probability 
		\begin{equation}
		\Pr[\textrm{measurement output equals }y]=\textrm{tr}(M_{y}\rho).
		\end{equation}
	

	
		 The state after a measurement is made is not uniquely specified by a
		POVM defined by matrices $\{M_{y}\}_{y=0}^{N'-1}$. 
		 By taking the positive semi-definite square root of $M_{y}$, i.e.,
		\begin{equation}
		M_{y}^{1/2}=\sqrt{M_{x}}=V_{y}\Lambda_{y}^{1/2}V_{y}^{\dagger},
		\end{equation}
		where $M_{y}=V_{y}\Lambda_{y}V_{y}^{\dagger}$ is the eigendecomposition
		of $M_{y}$, one typically sets the post-measurement state to the density matrix
		\begin{equation}
		\frac{M_{y}^{1/2}\rho M_{y}^{1/2}}{\textrm{tr}(M_{y}\rho)}.
		\end{equation}
		 POVMs generalize projective measurements, which are obtained by setting
		$M_{y}=\Pi_{y}$ (note that we have $\Pi_{y}^{1/2}=\Pi_{y})$.
	

\subsection{POVM for Unambigous Quantum State Discrimination}\label{sec:ch5:povmd}
	
		In this subsection, we study the application of POVMs for quantum state detection. To this end, assume that the state of a quantum system, with an arbitrary number
		of qubits, can either be vector $|\psi_{0}\rangle$ or vector $|\psi_{1}\rangle$,
		but we do not know which. 
		 If the vectors $|\psi_{0}\rangle$ and $|\psi_{1}\rangle$ are orthogonal,
		it is possible to distinguish them exactly (with probability 1) by
		using the standard von Neumann measurement defined by the projectors
		\begin{align}
			\Pi_{0} & =|\psi_{0}\rangle\langle\psi_{0}|\nonumber\\
			\Pi_{1} & =|\psi_{1}\rangle\langle\psi_{1}|\nonumber\\
			\Pi & _{2}=I-\Pi_{0}-\Pi_{1}
		\end{align}
		 In fact, if the true vector is $|\psi_{y}\rangle$ the measurement
		returns $y$ with probability $\textrm{tr}(\Pi_{y}|\psi_{y}\rangle\langle\psi_{y}|)=1$
		for $y\in\{0,1\}$.
		 Note that if there is a single qubit, the third projector is not necessary.
		 What if $|\psi_{1}\rangle$ or vector $|\psi_{2}\rangle$ are not
		orthogonal?
	

	
		 In this case, we can design a POVM such that, whenever a decision
		is made, the decision is correct; but it is allowed for the measurement
		to return a ``don't know'' decision.
		 To this end, consider the POVM
		\begin{align}
			M_{0} & =a(I-|\psi_{1}\rangle\langle\psi_{1}|)\nonumber\\
			M_{1} & =a(I-|\psi_{0}\rangle\langle\psi_{0}|)\nonumber\\
			M & _{2}=I-M_{0}-M_{1}
		\end{align}
		where $a=(1+|\langle\psi_{0}|\psi_{1}\rangle|)^{-1}$.
	

%

	
		 If the true state is $|\psi_{0}\rangle$, the measurement returns
		$y=0$ with probability
		\begin{align}
			\textrm{tr}(M_{0}|\psi_{0}\rangle\langle\psi_{0}|) & =a\langle\psi_{0}|(I-|\psi_{1}\rangle\langle\psi_{1}|)|\psi_{0}\rangle\nonumber\\
			& =a\cdot(1-|\langle\psi_{0}|\psi_{1}\rangle|^{2})=1-|\langle\psi_{0}|\psi_{1}\rangle|;
		\end{align}
		it returns $y=1$ with probability 
		\begin{align}
			\textrm{tr}(M_{1}|\psi_{0}\rangle\langle\psi_{0}|) & =a\langle\psi_{0}|(I-|\psi_{0}\rangle\langle\psi_{0}|)|\psi_{0}\rangle\\
			& =a\cdot(1-1)=0;
		\end{align}
		and ``don't know'', i.e., $y=2$, with probability
		\begin{align}
			\textrm{tr}(M_{2}|\psi_{0}\rangle\langle\psi_{0}|) & =|\langle\psi_{0}|\psi_{1}\rangle|.
		\end{align} A similar situation occurs if the true state is $|\psi_{1}\rangle.$
		
		We conclude that, with the designed POVM,  So there is no ambiguous detection, but a ``declaration of ignorance''
		with probability \textrm{$|\langle\psi_{0}|\psi_{1}\rangle|$:} The 
		more aligned the two vectors are, the more likely it is that the detector
		will not be able to make a definite decision.
		 Note that, in order to obtain unambiguous state discrimination, as
		decribed above, it is necessary to use a POVM and projective measurements
		are not sufficient.
		
		\section{Quantum Channels}
		
%		\begin{frame}{Quantum Noise}
%			\begin{itemize}
%				\item In the previous lectures, we have assumed the possibility to prepare
%				quantum states, implement unitary transformations, and carry out measurements
%				exactly as prescribed by theory.
%				\item In practice, all these steps are subject to imperfections and noise.
%				\item In this lesson, we will elaborate on noise that arises from the interaction
%				of the system with the environment.
%				\item As we have seen, open quantum systems, interacting with the environment,
%				are affected by decoherence. 
%				\item This implies that, rather than producing specific pure states, practical
%				quantum gate produce mixed states. 
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Quantum Channels}
%			\begin{itemize}
%				\item To study the effect of quantum noise, we consider the following general
%				situation:
%				\begin{itemize}
%					\item the input state is density $\rho_{in}$
%					\item ancillas are added in the ground state, with the state of the overall
%					system being $|0\rangle\langle0|\otimes\rho_{in}$
%					\item a unitary $U$ is applied to the overall system, producing state $U(|0\rangle\langle0|\otimes\rho_{in})U^{\dagger}$
%					\item a non-selective measurement is applied to a subset of qubits, which
%					is equivalent to measuring them and discarding the output
%				\end{itemize}
%				\item We will refer to this quantum system as a quantum channel.
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Quantum Channels}
%			
%			{\small{}\begin{center}
%					\begin{quantikz} 
%						\lstick{$\ket{0}\bra{0}$}& \gate[wires=2]{U}\qwbundle{} & \meter{} \qwbundle{}& \trash{\text{trash}} \qwbundle{}\\
%						\lstick{$\rho_{in}$} & \qwbundle{} &  \qwbundle{} & \qw 
%					\end{quantikz}
%			\end{center}}{\small\par}
%		\end{frame}
%		%
%		\begin{frame}{Quantum Channels}
%			\begin{itemize}
%				\item The situation is equivalent to that yielding POVMs with the important
%				caveat that the measurement output is not retained. 
%				\item From the analysis of POVM, we recall that the output of the unitary,
%				with $\rho_{in}=|\psi\rangle\langle\psi|$, can be written as 
%				\[
%				U|0,\psi\rangle=\left[\begin{array}{c}
%					U_{00}|\psi\rangle\\
%					U_{10}|\psi\rangle\\
%					\vdots\\
%					U_{N'-1,0}|\psi\rangle
%				\end{array}\right]=\sum_{x=0}^{2^{n'}-1}|x\rangle\otimes K_{x}|\psi\rangle,
%				\]
%				where matrices $K_{x}$ are of size $2^{n}\times2^{n}$, and satisfy
%				the condition
%				\[
%				\sum_{x=0}^{2^{n'}-1}K_{x}^{\dagger}K_{x}=I.
%				\]
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Quantum Channels}
%			\begin{itemize}
%				\item We also recall that the effect of a non-selective measurement can
%				be described via the partial trace operation.
%				\item Tracing out the ancillas yields the state
%				\begin{align*}
%					\rho_{out} & =\textrm{tr}_{A}(U(|0\rangle\langle0|\otimes\rho_{in})U^{\dagger})\\
%					& =\sum_{x=0}^{2^{n'}-1}(\langle x|\otimes I)(U(|0\rangle\langle0|\otimes\rho_{in})U^{\dagger})(|x\rangle\otimes I)\\
%					& =\sum_{x=0}^{2^{n'}-1}K_{x}\rho_{in}K_{x}^{\dagger}.
%				\end{align*}
%				\item This operation defines a quantum channel.
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Quantum Channel}
%			\begin{itemize}
%				\item To summarize, a quantum channel is defined by a set of matrices $\{K_{x}\}_{x=0}^{r-1}$,
%				known as Kraus matrices, of dimension $2^{n}\times2^{n}$, satisfying
%				the property 
%				\[
%				\sum_{x=0}^{r-1}K_{x}^{\dagger}K_{x}=I
%				\]
%				for some integer $r.$
%				\item The output state is given as 
%				\[
%				\rho_{out}=\sum_{x=0}^{r-1}K_{x}\rho_{in}K_{x}^{\dagger}.
%				\]
%				\item We write a quantum channel as 
%				\[
%				\rho_{out}=\mathcal{N}(\rho_{in}).
%				\]
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Quantum Channels}
%			\begin{itemize}
%				\item One can intuitively think of a quantum channel has modifying the input
%				density $\rho_{in}$ to the (normalized version of the unnormalized)
%				density $K_{x}\rho_{in}K_{x}^{\dagger}$ with probability related
%				to the trace of the latter.
%				\item Unless $r=1,$ quantum channels are generally not reversible, as they
%				describe situations in which the system interacts with ancilla systems,
%				e.g., the ``environment'' -- which ``measures'' the system -- and
%				information about the system is lost.
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Quantum Channels}
%			\begin{itemize}
%				\item The Kraus representation of a quantum channel is not unique.
%				\item In fact, Kraus matrices are equivalent up to a unitary transformation.
%				\item Specifically, two Kraus representations are equivalent if we can write
%				\[
%				K_{x}=\sum_{y}[U]_{xy}K_{y}^{'},
%				\]
%				where $U$ is a unitary matrix.
%				\item A Kraus representation with the smallest number of terms in the sum
%				is known as a minimal representation.
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Quantum Channels}
%			\begin{itemize}
%				\item Technically, quantum channels are
%				\begin{itemize}
%					\item linear, 
%					\item completely positive (CP), 
%					\item trace preserving (TP).
%				\end{itemize}
%				\item In short, they are CPTP operators.
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Quantum Channels}
%			\begin{itemize}
%				\item Linearity is evident (see also below for an equivalent representation
%				in terms of matrix-vector multiplication).
%				\item Trace preservation can be checked as:
%				\begin{align*}
%					\mathrm{tr}(\rho_{out}) & =\sum_{x=0}^{r-1}\mathrm{tr}\left(K_{x}\rho_{in}K_{x}^{\dagger}\right)\\
%					& =\sum_{x=0}^{r-1}\mathrm{tr}\left(\rho_{in}K_{x}^{\dagger}K_{x}\right)=\mathrm{tr}\left(\rho_{in}\sum_{x=0}^{r-1}K_{x}^{\dagger}K_{x}\right)=1
%				\end{align*}
%				\item Note that this explains the need for the condition \textrm{$\sum_{x=0}^{r-1}K_{x}^{\dagger}K_{x}=I$.}
%				\item Completely positivity means that, when applied on a subset of a larger
%				system, the transformation yields a valid density for the whole system.
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Quantum Channels}
%			\begin{itemize}
%				\item Quantum channels can be further generalized by allowing the number
%				of qubits being measured to be generally different (larger or smaller)
%				from the number of ancilla qubits.
%				\item If the number of input qubits is $n_{in}$ and the number of output
%				qubits is $n_{out}$, a quantum channel, a quantum channel is defined
%				by a set of matrices $\{K_{x}\}_{x=0}^{r-1}$, known as Kraus matrices,
%				of dimension $2^{n_{out}}\times2^{n_{in}}$, satisfying the completeness
%				relationship
%				\[
%				\sum_{x=0}^{r-1}K_{x}^{\dagger}K_{x}=I_{2^{n_{in}}}.
%				\]
%				\item The output state is given as 
%				\[
%				\rho_{out}=\sum_{x=0}^{r-1}K_{x}\rho_{in}K_{x}^{\dagger},
%				\]
%				\item It can be proved that the number of Kraus operators $r$ can be bounded
%				without loss of generality by $2^{n_{in}+n_{out}}.$
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Examples of Quantum Channels}
%			\begin{itemize}
%				\item Quantum channels include all quantum primitives that do not involve
%				a selective measurement. Some examples follow.
%				\item Quantum state preparation: Create a quantum ensemble $\{p_{x},|v_{x}\rangle\},$
%				i.e., a density matrix $\rho_{out}=\sum_{x}p_{x}|v_{x}\rangle\langle v_{x}|$: 
%				\begin{itemize}
%					\item $K_{x}=\sqrt{p_{x}}|v_{x}\rangle$ ($\sum_{x}p_{x}\langle v_{x}|v_{x}\rangle=1$),
%					yielding the output state \textrm{$\rho_{out}=\sum_{x=0}^{r-1}p_{x}|v_{x}\rangle\langle v_{x}|$}
%				\end{itemize}
%				\item Appending ancillas in a state $\sum_{x}p_{x}|v_{x}\rangle\langle v_{x}|$:
%				$K_{x}=I\otimes\sqrt{p_{x}}|v_{x}\rangle$
%				\item Trace: $K_{x}=\langle x|$
%				\item Partial trace: $K_{x}=I\otimes\langle x|$
%				\item POVM $\{M_{x}\}$ non-selective measurements: $K_{x}=M_{x}^{1/2}$
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Examples of Quantum Channels}
%			\begin{itemize}
%				\item Quantum channels are also used to describe ``noisy'' channels.
%				\item To start consider a classical discrete noisy channel defined by a
%				conditional distribution $p(y|x)$ on finite alphabets for input $x$
%				and output $y$.
%				\item This can be described with the Kraus operators $K_{xy}=\sqrt{p(y|x)}|y\rangle\langle x|$
%				if the classical input and output values are described by the orthogonal
%				states given by the computational basis (check!).
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Examples of Quantum Channels}
%			\begin{itemize}
%				\item As a truly quantum example, Pauli channels are single-qubit channels
%				that have Kraus matrices
%				\[
%				K_{0}=\sqrt{p_{0}}I,\textrm{}K_{1}=\sqrt{p_{1}}X,\textrm{}K_{2}=\sqrt{p_{2}}Y,\textrm{}K_{3}=\sqrt{p_{3}}Z,
%				\]
%				yielding
%				\[
%				\rho_{out}=p_{0}\rho_{in}+p_{1}X\rho_{in}X+p_{2}Y\rho_{in}Y+p_{3}Z\rho_{in}Z
%				\]
%				for $p_{k}\geq0$ with $\sum_{k=0}^{3}p_{k}=1$.
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Examples of Quantum Channels}
%			\begin{itemize}
%				\item Single-qubit channels are practically important since most error models
%				in quantum computing assume independent errors across qubits.
%				\item These examples suggest that we can think of the Kraus operators as
%				the different types of errors that can occur on a qubit, with each
%				error having a different probability.
%				\item In particular, the different types of errors correspond to the application
%				of $X,$$Y,$or $Z$ operators. 
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Examples of Quantum Channels}
%			\begin{itemize}
%				\item Pauli channels specialize to some important subclasses of channels
%				\item Bit flip channel, i.e., $X$ errors:
%				\[
%				\rho_{out}=(1-p)\rho_{in}+pX\rho_{in}X,
%				\]
%				where we can assume without loss of generality $p\leq0.5$ (otherwise,
%				we can apply an $X$ operator to $\rho_{in}$ to obtain the same channel).
%				\item If $\rho_{in}$ describes a classical distribution $(p_{0},p_{1})$,
%				then $\rho_{out}$ is given as
%				\[
%				\rho_{out}=\left[\begin{array}{cc}
%					(1-p)p_{0}+pp_{1} & 0\\
%					0 & (1-p)p_{1}+pp_{0}
%				\end{array}\right],
%				\]
%				which describes the distribution of a classical bit flip channel with
%				input distribution $(p_{0},p_{1})$.
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Examples of Quantum Channels}
%			\begin{itemize}
%				\item Dephasing channel, i.e., $Z$ errors:
%				\[
%				\rho_{out}=(1-p)\rho_{in}+pZ\rho_{in}Z,
%				\]
%				where we can assume without loss of generality $p\leq0.5$ (otherwise,
%				we can apply an $Z$ operator to $\rho_{in}$ to obtain the same channel).
%				\item For a single qubit with density 
%				\[
%				\rho_{in}=\left[\begin{array}{cc}
%					\rho_{00} & \rho_{01}\\
%					\rho_{01}^{*} & \rho_{11}
%				\end{array}\right],
%				\]
%				where $\rho_{00},\rho_{11}\geq0$, $\rho_{00}+\rho_{11}=1$, and $\rho_{00}\rho_{11}\geq|\rho_{01}|^{2},$
%				we have 
%				\[
%				\rho_{out}=\left[\begin{array}{cc}
%					\rho_{00} & (1-2p)\rho_{01}\\
%					(1-2p)\rho_{01}^{*} & \rho_{11}
%				\end{array}\right].
%				\]
%			\end{itemize}
%		\end{frame}
%		%
%		\begin{frame}{Examples of Quantum Channels}
%			\begin{itemize}
%				\item A dephasing channel does not modify classical distributions, but it
%				does affect more general density states.
%				\item In particular, with $p=0.5$, we obtain the completely dephasing channel,
%				in which $\rho_{out}$ has the same diagonal elements of $\rho_{in}$
%				but zero out-of-diagonal elements.
%			\end{itemize}
%		\end{frame}
	
\section{Conclusions}
In this chapter, we have extended the formalism of quantum measurements to projective measurements and to POVMs, with the latter providing the most general form of quantum measurement. Throughout, we have emphasized quantum circuit that can implement such measurements via standard measurements in the computational basis. We have also highlighted two important applications: quantum error correction for projective measurements and quantum detection for POVMs.

\section{Recommended Resources}
Projective measurements and POVMs are well explained in \cite{nielsen10,wilde2013quantum}. Quantum error correction is a vast field, and the books \cite{mermin2007quantum,nielsen10} provide excellent introductions. Quantum communications and networking are covered by \cite{wilde2013quantum,rohde2021quantum}.
%
\section{Problems}
	
	\begin{itemize}
		\item For an observable $O$ and two states $|\psi\rangle=\sum_{x}\sqrt{p_{x}}|x\rangle$
		and $\rho=\sum_{x}p_{x}|x\rangle\langle x|$, show the relationship
		\begin{equation}
			\langle O\rangle_{|\psi\rangle}=\langle O\rangle_{\rho}+\sum_{x,y:x\neq y}\sqrt{p_{x}p_{y}}\langle x|O|y\rangle.\end{equation} Interpret this equality.
		\item Consider a non-selective projective measurement implemented with
		ancillas in which the output of the measurement of the ancillas is
		discarded. Describe the post-measurement state for an arbitrary input
		density matrix $\rho$.
		\item Consider the observables $X\otimes X$, $Y\otimes Y$, and $Z\otimes Z$,
		and show that the numerical outputs of their observations can be obtained
		by using either separable measurements or joint measurements in the
		Bell basis (Hint: We have $Z\otimes Z=(|00\rangle\langle00|+|11\rangle\langle11|)-(|01\rangle\langle01|+|10\rangle\langle10|)=(|\Phi^{+}\rangle\langle\Phi^{+}|+|\Phi^{-}\rangle\langle\Phi^{-}|)-(|\Psi^{+}\rangle\langle\Psi^{+}|+|\Psi^{-}\rangle\langle\Psi^{-}|)$.
		\item  Describe the Helstrom measurement (i.e., the measurement that
		has the minimum error probability when trying to distinguish between
		two states).
		\item Prove that a non-selective measurement on the output of a unitary
		transformation involving ancillas results in a POVM (see, e.g., M.
		Wilde's book).
		\item Describe the measurement-based definition of the quantum entropy.
		\item Derive a necessary condition on the numbers $k$, $n$, and $m$ of information qubits, encoded qubits, and types of errors, that is required for quantum error detection.
		\item Describe a circuit that measures the observable $X \otimes X$ in a system with two qubits. Consider the implementation involving only the two qubits, as well as the implementation that includes ancilla qubits. 
		\item Describe a quantum error correction code, including encoder and decoder, for the channel that may flip the phase of at most one out of three qubits. A phase flip corresponds to the application of a Pauli $Z$ operator. [Hint: Phase flips correspond to bit flips with a suitable change of basis.]
	\end{itemize}
		
		
		
	
	




%{Grover's Search Algorithm}
%	
%		 We wish to find a single value $x^{*}$ in a discrete set $\{0,1,....,2^{n}-1\}$
%		that satisfies some property.
%		 We assume that we have a verifier function $f(x)$ that outputs $1$
%		only when $x=x^{*}$, i.e., $f(x^{*})=1$, while returning $f(x)=0$
%		otherwise.
%		 Consider first a classical strategy, where we probe the verifier function
%		$f(x)$ successively at different values of $x$.
%		 If we randomly pick a value of $x$ uniformly on all the remaining
%		objects, the probability of finding $x^{*}$ after $k$ trials is
%		\begin{equation}
%		\frac{k}{2^{n}}
%		\end{equation}
%		and hence each new query adds $1/2^{n}$ to the probability of success.
%		 To obtain a probability of success $1-\epsilon$, we hence need
%		\begin{equation}
%		k=(1-\epsilon)2^{n}=O(2^{n})
%		\end{equation}
%		queries.
%	
%
%%
%{Grover's Search Algorithm}
%	
%		 Assume now that we have a quantum verifier $U_{f}$ that implements
%		function $f$.
%		 How many times do we have to query the quantum verifier to find $x^{*}$
%		with high probability?{\small{}\begin{center}
%				\begin{quantikz}
%					\lstick{$\ket{x}$} & \qwbundle{n} & \gate[wires=2]{U_f} & \qwbundle{n}  \rstick{$\ket{x}$}\\
%					\lstick{$\ket{0}$} & \qw & & \qw  \rstick{$\ket{0}$ if $x\neq x^{*}$ and $\ket{1}$ if $x=x^{*}$}
%				\end{quantikz}
%		\end{center}}{\small\par}
%	
%
%%
%{Grover's Search Algorithm}
%	
%		 Let us start by choosing as input the separable state in which the
%		first $n$ qubits are in state
%		\begin{equation}
%		\ensuremath{|+\rangle^{\otimes n}=H^{\otimes n}|0\rangle^{\otimes n}=\frac{1}{\sqrt{2^{n}}}\sum_{x=0}^{2^{n}-1}|x\rangle},
%		\end{equation}
%		which consists of a full superposition of all possible vectors in
%		the computational basis; and $|-\rangle$ for the last qubit.{\small{}\begin{center}
%				\begin{quantikz}
%					\lstick{$\ket{+}^{\otimes n}$} & \qwbundle{n} & \gate[wires=2]{U_f} & \qwbundle{n}  \\
%					\lstick{$\ket{-}$} & \qw & & \qw  
%				\end{quantikz}
%		\end{center}}{\small\par}
%	
%
%%
%{Grover's Search Algorithm}
%	
%		 {\small{}By phase kick-back (see previous lecture), one can easily
%			check that, after the application of $U_{f},$ the state of the first
%			$n$ qubits is }
%		\begin{equation}
%		\ensuremath{\frac{1}{\sqrt{2^{n}}}\sum_{x=0,\textrm{ }x\neq x^{*}}^{2^{n}-1}|x\rangle-\frac{1}{\sqrt{2^{n}}}|x^{*}\rangle=\sqrt{\frac{2^{n}-1}{2^{n}}}|\bar{x}\rangle-\frac{1}{\sqrt{2^{n}}}|x^{*}\rangle},
%		\end{equation}
%		where $|\bar{x}\rangle=\frac{1}{\sqrt{2^{n}-1}}\sum_{x=0,\textrm{ }x\neq x^{*}}^{2^{n}-1}|x\rangle.${\small{}\begin{center}
%				\begin{quantikz}
%					\lstick{$\ket{+}^{\otimes n}$} & \qwbundle{n} & \gate[wires=2]{U_f} & \qwbundle{n}  \rstick{$\sqrt{\frac{2^{n}-1}{2^{n}}}|\bar{x}\rangle-\frac{1}{\sqrt{2^{n}}}|x^{*}\rangle$}\\
%					\lstick{$\ket{-}$} & \qw & & \qw  \rstick{$\ket{-}$}
%				\end{quantikz}
%		\end{center}}{\small\par}
%	
%
%%
%{Grover's Search Algorithm}
%	
%		 So measuring the first $n$ qubits in the computational basis would
%		return the correct response with probability $1/2^{n}$, as the classical
%		system.{\small{}\begin{center}
%				\begin{quantikz}
%					\lstick{$\ket{+}^{\otimes n}$} & \qwbundle{n} & \gate[wires=2]{U_f} & \qwbundle{n}  \rstick{$\sqrt{\frac{2^{n}-1}{2^{n}}}|\bar{x}\rangle-\frac{1}{\sqrt{2^{n}}}|x^{*}\rangle$}\\
%					\lstick{$\ket{-}$} & \qw & & \qw  \rstick{$\ket{-}$}
%				\end{quantikz}
%		\end{center}}{\small\par}
%	
%
%%
%{Grover's Search Algorithm}
%	
%		 Consider now the inverse-about-the-mean transform 
%		\begin{equation}
%		U_{IAM}=2|+\rangle^{\otimes n}\langle+|^{\otimes n}-I.
%		\end{equation}
%		 Geometrically, this is a Householder matrix that reflects vectors
%		about the unique hyperplane through the origin that has $|+\rangle$
%		as normal vector and negates the output.
%		 Let us apply it to a general state $|\psi\rangle=\sum_{x=0}^{2^{n}-1}\alpha_{x}|x\rangle$
%		and define as 
%		\begin{equation}
%		\mu=\frac{1}{2^{n}}\sum_{x=0}^{2^{n}-1}\alpha_{x}
%		\end{equation}
%		the mean of the amplitudes.
%	
%
%%
%{Grover's Search Algorithm}
%	
%		 Let us apply it to a general state $|\psi\rangle=\sum_{x=0}^{2^{n}-1}\alpha_{x}|x\rangle$
%		and define as 
%		\begin{equation}
%		\mu=\frac{1}{2^{n}}\sum_{x=0}^{2^{n}-1}\alpha_{x}
%		\end{equation}
%		the mean of the amplitudes.
%		 We obtain
%		\begin{align*}
%			U_{IAM}|\psi\rangle & =2|+\rangle^{\otimes n}\underbrace{\langle+|^{\otimes n}|\psi\rangle}_{\frac{1}{\sqrt{2^{n}}}\sum_{x=0}^{2^{n}-1}\alpha_{x}=\sqrt{2^{n}}\mu}-\sum_{x=0}^{2^{n}-1}\alpha_{x}|x\rangle\\
%			& =2\left[\begin{array}{c}
%				\mu\\
%				\mu\\
%				\vdots\\
%				\mu
%			\end{array}\right]-\left[\begin{array}{c}
%				\alpha_{0}\\
%				\alpha_{1}\\
%				\vdots\\
%				\alpha_{2^{n}-1}
%			\end{array}\right]=\left[\begin{array}{c}
%				2\mu-\alpha_{0}\\
%				2\mu-\alpha_{1}\\
%				\vdots\\
%				2\mu-\alpha_{2^{n}-1}
%			\end{array}\right]
%		\end{align*}
%	
%
%%
%{Grover's Search Algorithm}
%	
%		 Let us add the inverse-about-the-mean transform to the circuit as
%		shown below.
%		 Since 
%		\begin{align*}
%			\mu & =\frac{1}{2^{n}}(2^{n}-1)\frac{1}{\sqrt{2^{n}}}-\frac{1}{2^{n}}\frac{1}{\sqrt{2^{n}}}=\frac{1}{2^{n}\sqrt{2^{n}}}(2^{n}-2)=O\left(\frac{1}{\sqrt{2^{n}}}\right).
%		\end{align*}
%		 The state of the first $n$ qubits become
%		\begin{equation}
%		\left(\sqrt{1-(\alpha^{*})^{2}}\right)|\bar{x}\rangle+\left(\underbrace{2\mu+\frac{1}{\sqrt{2^{n}}}}_{=\alpha^{*}}\right)|x^{*}\rangle
%		\end{equation}
%		{\small{}\begin{center}
%				\begin{quantikz}
%					\lstick{$\ket{+}^{\otimes n}$} & \qwbundle{n} & \gate[wires=2]{U_f} & \qwbundle{n} & \gate[wires=2]{U_{IAM}} & \qwbundle{n}\\
%					\lstick{$\ket{-}$} & \qw & & \qw  && \qw
%				\end{quantikz}
%		\end{center}}{\small\par}
%	
%
%%
%{Grover's Search Algorithm}
%	
%		 {\small{}Accordingly, the amplitude corresponding to the desired state
%			$|x^{*}\rangle$ has increased by }\textrm{$O\left(\frac{1}{\sqrt{2^{n}}}\right).$}
%		 {\small{}This suggests that }\textrm{$O(\sqrt{2^{n}})$}{\small{}
%			queries are sufficient to obtain a given level of accuracy.}{\small\par}
%		 This yields a quadratic improvement over classical systems.
%		 This conclusion can be made formal through a precise analysis.
	


==> Chapter6/Chapter6__KCL1JY99K3_s_conflicted_copy_2022-05-03_.tex <==

\chapter{Quantum Machine Learning}


\section{Introduction}

In this chapter, we introduce the basics of quantum machine learning. We  start by presenting a taxonomy of approaches, and proceed with reviewing the key concept of parametrized quantum circuit (PQC) and ansatz. As a preliminary step, we describe the variational quantum eigensolver (VQE) as a means to address a specific class of combinatorial problems. VQEs share with quantum machine learning techniques the key idea of using classical optimization to minimize the expectation of a quantum observable as the loss function. With this background, we overview probabilistic and deterministic machine learning models obtained from PQCs, with applications to unsupervised generative learning and supervised learning (regression and classification). We conclude with some additional discussion about the choice of the ansatz, as well as with an outlook.

\section{What is Quantum Machine Learning?}

As introduced in Chapter 4, quantum computing algorithms have been traditionally designed by hand
assuming the availability of \textbf{fault-tolerant} quantum computers with a large number of qubits and gates. In practice, current  quantum computers support a few tens of qubits, and projections are that in the near term the number of qubits will not exceed around 1000. Furthermore, quantum state preparation, quantum gates, and quantum measurements in real quantum computers are subject to decoherence and noise (see Sec. \ref{sec:ch3:decoh}). This makes it necessary to implement forms of quantum error correction in order to emulate the operation of the corresponding noiseless operation assumed by the designed quantum algorithms (see Sec. \ref{sec:ch5:qec}). And this requirement, in turn, further increases the number of necessary physical qubits, as each logical qubit must be encoded into a number of physical qubits to implement quantum error correction strategies. 

Against this backdrop, quantum machine learning refers to the alternative paradigm illustrated in Fig. \ref{fig:ch6:qmlintro} of fixing a priori a, possibly generic, parametric architecture for the quantum algorithm and then using classical optimization to optimize the parameters of the algorithm. Specifically, as sketched in Fig. \ref{fig:ch6:qmlintro}, the operation of the quantum algorithm is defined by a unitary operation $U(\theta)$ dependent on a vector of parameters $\theta$. The vector $\theta$ represent free parameters that can be optimized. The quantum computer implementing the unitary $U(\theta)$ is connected to a classical optimizer, which takes as input measurements of the quantum state produced by the quantum computer and produces as output updates to the vector $\theta$. 

The classical optimizer typically observes expected values of observables under the quantum state produced by the quantum computer. This requires evaluating empirical averages of multiple runs of the quantum algorithm in order to determine the updates to the model parameter vector $\theta$. Furthermore, the classical optimizer may have access to data, which it can use to define objective functions to be optimized. Data may also be fed to the quantum computer. We refer to the next section for more discussion on the role of data.

The quantum machine learning architecture of Fig. \ref{fig:ch6:qmlintro} has a number of potential advantages over the standard approach of handcrafting quantum algorithms assuming fault-tolerant quantum computers: \begin{itemize} 
	\item By keeping the quantum computer in the loop, the classical optimizer 
can directly account for the non-idealities and limitations of quantum operations via measurements of the output of the quantum computer.
\item If the PQC $U(\theta)$ is sufficiently flexible and the classical optimizer sufficiently effective, the approach may automatically design well-performing quantum algorithms that would have been hard to optimize by hand.
\end{itemize}

\begin{figure}
\begin{center}
	\includegraphics[clip,scale=0.25]{figqml1}
	\par\end{center}\vspace{-0.4cm}\caption{The high-level architecture of the quantum machine learning design methodology. A parametric quantum circuit (PQC) $U(\theta)$ is optimized via its vector of parameters, $\theta$, by a classical optimizer based on measurements of the output of the PQC. \label{fig:ch6:qmlintro}}
\end{figure}

Like classical machine learning, quantum machine learning follows an \textbf{inductive} methodology based on the following two-step approach: \begin{itemize}
	\item  \textbf{Selection of the PQC}: The designer first selects a  PQC defined by a specific sequence of parametric quantum gates (see Sec. \ref{sec:ch6:PQC}). This choice should be ideally dictated by knowledge available to the designer about quantum algorithmic architectures that are well suited for the problem at hand. This step mirrors the classical choice of a parametric model, e.g., a neural network, in classical machine learning.
	\item \textbf{Parametric optimization}: Based on measurements of the output of the quantum computer, typically in the form of estimated expectations of observables, the classical optimizer adapts the model parameter vector $\theta$ of the PQC. This is done with the goal of minimizing some loss function, which may depend also on training data. This step is also central to classical machine learning, in which the model parameters $\theta$ are typically optimized via gradient descent-based methods by targeting the minimization of the training loss.
\end{itemize}

\section{A Taxonomy of Quantum Machine Learning}

Unlike classical machine learning, in which data and processing are classical, in quantum machine learning
data and/or processing are of quantum nature. The possible scenarios are summarized in Table \ref{table:ch6:table1}, and are reviewed in this section.

\begin{table}
\begin{center}
	\begin{tabular}{cccc}
		&  & \textbf{data} & \textbf{processing}\tabularnewline
		&  & C & Q\tabularnewline
		\cmidrule{3-4} \cmidrule{4-4} 
		\textbf{data} & C & CC & CQ\tabularnewline
		\cmidrule{3-4} \cmidrule{4-4} 
		\textbf{generation} & Q & QC & QQ\tabularnewline
		\cmidrule{3-4} \cmidrule{4-4} 
	\end{tabular}
	\par\end{center}\vspace{-0.4cm}\caption{Taxonomy of machine learning settings as a function of the type of data and processing (C=classical, Q=quantum). \label{table:ch6:table1}}
\end{table}

The \textbf{classical data and classical processing (CC)} case prescribes the
optimization of a standard machine learning model, e.g., a neural
network, via a classical optimizer.
As illustrated in Fig. \ref{fig:ch6:cc}, a classical machine learning model implements
a parametrized function $f(x|\theta)$ mapping classical input data
$x$ to an output. The classical optimizer minimizes some cost function over $\theta$
based on classical data. A common example is given by classical supervised learning, in which the classical data consists of pairs of inputs and desired outputs, and the loss function measures how well the prediction of the output produced by function $f(x|\theta)$ matches the desired output. 

\begin{figure}
\begin{center}
	\includegraphics[clip,scale=0.3]{figqml2}
	\par\end{center}\vspace{-0.4cm} \caption{An illustration of classical machine learning, in which both data and processing are of classical nature. \label{fig:ch6:cc}}
\end{figure}

Currently, the most common quantum machine learning setting is characterized by \textbf{classical data and quantum processing (CQ)}. In this case, as illustrated in Fig. \ref{fig:ch6:cq}, 
a quantum model is defined by a PQC that implements a unitary transformation $U(x,\theta)$,
which generally depends on the classical input $x$ and on
the model parameter vector $\theta$. 
The input to the PQC is a set of qubits in the
ground state $|0\rangle$, and the output state produced by the PQC is hence given by  \begin{equation}|\psi(x,\theta)\rangle=U(x,\theta)|0\rangle.
\end{equation}
The classical optimizer minimizes some cost function over the model parameter vector $\theta$. The cost function depends on classical data, as well as of an estimate of an observable of the output quantum state
$|\psi(x,\theta)\rangle$. Estimating the expectation of the given observable requires running the PCQ multiple times in order to obtain an empirical average.

\begin{figure}
\begin{center}
	\includegraphics[clip,scale=0.25]{figqml3}
	\par\end{center}\vspace{-0.4cm}\caption{An illustration of the ``CQ'' setting of quantum machine learning, in which data is classical and processing is quantum.\label{fig:ch6:cq}}
\end{figure}


In the \textbf{quantum data and quantum processing (QQ)} case, the learner has access to quantum data defined by a collection of quantum systems, each in some
general density state. As illustrated in Fig. \ref{fig:ch6:qq}, such data can determine the input to the PQC, and/ or serve as a target to be
compared to the quantum state output by the PQC through a quantum
loss metric (e.g., the fidelity). An example of this case, which will not be further discussed in this monograph, is given by  quantum generative adversarial networks, in which the quantum
loss is computed via a detector that attempts to distinguish real
quantum data from quantum states generated by the PQC.

\begin{figure}
\begin{center}
	\includegraphics[clip,scale=0.25]{figvqe4}
	\par\end{center}\vspace{-0.4cm}\caption{An illustration of the ``QQ'' setting of quantum machine learning, in which data is quantum and processing is quantum.\label{fig:ch6:qq}}
\end{figure}

%
\section{Ansatz and Parametrized Quantum Circuit}\label{sec:ch6:PQC}

As discussed in the previous section, at the core of quantum machine learning methods are PQCs.
A PQC is a unitary $U(\theta)$ whose operation on $n$ qubits depends
on a tunable (classical) parameter vector $\theta$ consisting of $D$ real numbers. As also seen in the previous section, in the CQ case, the unitary may also depend on input data $x$, and we
will discuss this case in the context of supervised learning in Sec. \ref{sec:ch6:sl}.
The unitary $U(\theta)$ is typically defined as a sequence of one-
or two-qubit gates, with each gate possibly dependent on the parameter
$\theta.$
For feasibility, the number of gates should be polynomial in the number
of qubits and not in the size of the Hilbert space. This way the number
of gates does not grow exponentially with the number of qubits.


The choice of the architecture of the PQC as a sequence of specific
gates is akin to the choice of the model class in classical machine
learning (e.g., a neural architecture).
In quantum machine learning, we refer to the architecture of the unitary
$U(\theta)$ as the \textbf{ansatz}. An ansatz is an assumption about the form of an unknown function which
is made in order to facilitate solution of an equation or other problem. The term originates in the 1930s and comes from the German term used for ``approach'' or ``attempt''. As for the inductive bias in machine learning, one should choose the
ansatz, if possible, based on domain knowledge. 
For instance, in quantum chemistry there are special structures that
are known to reflect well the nature of certain phenomena.

In this section, we review parametric quantum gates and corresponding ansatzes by proceeding in order of complexity, and hence, generally, also of expressivity of the resulting PQC. Specifically, we first review parametrized single-qubit gates and the mean-field ansatz; then, we describe the more complex hardware-efficient ansatz; and finally we discuss parametrized multi-qubit gates.

\subsection{Parametrized Single-Qubit Gates}

The most typical type of parametrized single-qubit gates is given by \textbf{Pauli rotation matrices}. A Pauli rotation matrix $R_p(\theta)$, with $p\in\{x,y,z\}$ is a unitary gate whose generator (see Sec. \ref{sec:ch1:Paulibasis}) is given by $\theta/2\cdot P$, i.e., \begin{equation}\label{eq:ch6:Pauli}
	R_{p}(\theta)=\exp\left(\frac{\theta}{2} P\right)=\cos(\theta/2)I-i\sin(\theta/2)P,
	\end{equation} where  $P\in \{X,Y,Z\}$ is the corresponding Pauli operator and $\theta$ is a real parameter (see also Appendix A). Given the interpretation of Pauli rotations in terms of rotations on the Bloch sphere, the parameter $\theta$ is also known as the \textbf{rotation angle}. The three Pauli rotations are summarized in Table \ref{table:ch6:Pauli}. By (\ref{eq:ch6:Pauli}), we note that we have the equalities
\begin{equation}\label{eq:ch6:Rx}
R_{x}(-\pi)=iX,
\end{equation}
\begin{equation}
R_{y}(-\pi)=iY,
\end{equation}
and 
\begin{equation}\label{eq:ch6:Rz}
R_{z}(-\pi)=iZ.
\end{equation}
Therefore, apart from a global phase, the Pauli rotations recover as special
cases, i.e., for a specific choice of the rotation angle $\theta$, the Pauli gates.

\begin{table}

\begin{center}
	{\small{}}%
	\begin{tabular}{cc}
		\toprule 
		{\small{}Pauli rotation} & {\small{}definition}\tabularnewline
		\midrule
		\midrule 
		{\small{}$R_{x}(\theta)$} & {\small{}$\exp\left(-i\frac{\theta}{2}X\right)=\left[\begin{array}{cc}
				\cos\left(\frac{\theta}{2}\right) & -i\sin\left(\frac{\theta}{2}\right)\\
				-i\sin\left(\frac{\theta}{2}\right) & \cos\left(\frac{\theta}{2}\right)
			\end{array}\right]$}\tabularnewline
		\midrule 
		{\small{}$R_{y}(\theta)$} & {\small{}$\exp\left(-i\frac{\theta}{2}Y\right)=\left[\begin{array}{cc}
				\cos\left(\frac{\theta}{2}\right) & -\sin\left(\frac{\theta}{2}\right)\\
				\sin\left(\frac{\theta}{2}\right) & \cos\left(\frac{\theta}{2}\right)
			\end{array}\right]$}\tabularnewline
		\midrule 
		{\small{}$R_{z}(\theta)$} & {\small{}$\exp\left(-i\frac{\theta}{2}Z\right)=\left[\begin{array}{cc}
				\cos\left(\frac{\theta}{2}\right)-i\sin\left(\frac{\theta}{2}\right) & 0\\
				0 & \cos\left(\frac{\theta}{2}\right)+i\sin\left(\frac{\theta}{2}\right)
			\end{array}\right]$}\tabularnewline
		\bottomrule
	\end{tabular}{\small\par}
	\par\end{center}

\vspace{-0.4cm}\caption{Pauli rotations are the most commonly used parametrized single-qubit gates. \label{table:ch6:Pauli}}
\end{table}

A \textbf{general parametrized single-qubit gate} can be expressed, apart from a global
phase, as the following cascade of two types of rotations 
\begin{equation}
	R(\theta^{1},\theta^{2},\theta^{3})=R_{p}(\theta^{1})R_{p'}(\theta^{2})R_{p}(\theta^{3}),
\end{equation}where $p'\neq p \in \{x,y,z\}$. A typical choice is $p=z$ and $p'=y$. Note that this general gate is specified by three parameters, i.e., rotation angles, $\theta^{1}$, $\theta^{2}$, and $\theta^{3}$.


Single-qubit gates can be applied in parallel to the qubits of a quantum
system. 
For instance, if we have two qubits ($n=2$), applying a rotation
only to the second qubit amounts to using the unitary\textrm{ $I\otimes R(\theta^{1},\theta^{2},\theta^{3})$},
with a $2\times2$ identity matrix $I$, to the system of two qubits.  
To indicate the qubit to which a single-qubit gate is applied one
typically uses a subscript. 
As an example, the gate $Z_{k}$ denotes a Pauli string with $n-1$
$2\times2$ identity matrices $I$ except for position $k$, where
we have the Pauli operator $Z$, i.e., 
\begin{equation}\label{eq:ch6:Zk}
	Z_{k}=\underbrace{I\otimes\cdots\otimes I}_{k-1}\otimes Z\otimes\underbrace{I\otimes\cdots\otimes I}_{n-k}.
\end{equation}
Similarly, we can write 
\begin{equation}
	R_{k}(\theta_{k}^{1},\theta_{k}^{2},\theta_{k}^{3})=\underbrace{I\otimes\cdots\otimes I}_{k-1}\otimes R(\theta_{k}^{1},\theta_{k}^{2},\theta_{k}^{3})\otimes\underbrace{I\otimes\cdots\otimes I}_{n-k}
\end{equation}
for a rotation with parameters $\theta_{k}^{1},\theta_{k}^{2},\theta_{k}^{3}$
applied to the $k$th qubit.

\subsection{Mean-Field Ansatz}

An ansatz $U(\theta)$ that uses only single-qubit gates is known
as a \textbf{mean-field ansatz} and is illustrated in Fig. \ref{fig:ch6:mf}. 
The mean-field ansatz implements the PQC 
\begin{align}
	U(\theta) & =R(\theta_{0}^{1},\theta_{0}^{2},\theta_{0}^{3})\otimes\cdots\otimes R(\theta_{n-1}^{1},\theta_{n-1}^{2},\theta_{n-1}^{3})\nonumber\\
	& =\prod_{k=0}^{n-1}R_{k}(\theta_{k}^{1},\theta_{k}^{2},\theta_{k}^{3}),
\end{align}
with $\theta_{k}^{1},\theta_{k}^{2},\theta_{k}^{3}$ for $k=0,...,n-1$
being scalar parameters that belong to vector $\theta=[\theta_{0}^{1},\theta_{0}^{2},\theta_{0}^{3},...,\theta_{n-1}^{1},\theta_{n-1}^{2},\theta_{n-1}^{3}]^{T}.$
Note that we have $D=3n$ parameters in vector $\theta.$

\begin{figure}
\begin{center}
		\begin{quantikz} 
			\lstick[wires=4]{$\ket{0}$}\qw &\gate{R(\theta_{0}^{1},\theta_{0}^{2},\theta_{0}^{3})}& \qw\\
			\qw &\gate{R(\theta_{1}^{1},\theta_{1}^{2},\theta_{1}^{3})}& \qw \\	
			\qw &\gate{R(\theta_{2}^{1},\theta_{2}^{2},\theta_{2}^{3})}& \qw\\
			\qw &\gate{R(\theta_{3}^{1},\theta_{3}^{2},\theta_{3}^{3})}& \qw
			
		\end{quantikz}
\end{center}\vspace{-0.4cm}\caption{The mean-field ansatz consists of general single-qubit gates applied in parallel to the $n$ qubits, which are initially in the ground state $|0\rangle$. \label{fig:ch6:mf}}
\end{figure}


Given the input state $|0\rangle$, the mean-field ansatz outputs the separable state 
\begin{align}
	U(\theta) & |0\rangle=R(\theta_{0}^{1},\theta_{0}^{2},\theta_{0}^{3})|0\rangle\otimes\cdots\otimes R(\theta_{n-1}^{1},\theta_{n-1}^{2},\theta_{n-1}^{3})|0\rangle.
\end{align}Note that we have denoted as $|0\rangle$ both the multi-qubit ground state and the corresponding single-qubit states for simplicity of notation. 
The mean-field ansatz may be enough for some applications. 
Note, in fact, that even using only Pauli $Y$ rotations, i.e., by setting
$\theta_{k}^{1}=0$ and $\theta_{k}^{3}=0$, allows the mean-field
ansatz to produce all possible vectors in the computational basis.
This can be done by setting $\theta_{k}^{2}=0$ or $\theta_{k}^{2}=\pi$
to encode the two computational basis vectors. More generally, however, it is necessary to leverage entanglement among the qubits by introducing entangling, multi-qubit, gates.


\subsection{Hardware-Efficient Ansatz}

Moving one level up along the complexity axis for ansatzes, the \textbf{hardware-efficient ansatz} includes both parametrized single-qubit gates
and a \textbf{fixed entangling unitary} $U_{ent}$, which does not depend on the parameter vector $\theta$.  As detailed below, the entangling unitary $U_{ent}$ typically consist of CNOT or CZ
gates. 
The use of a fixed entangling unitary is for simplicity of implementation,
since two-qubit gates are generally hard to implement on quantum computers.
This motivation justifies the name ``hardware-efficient'' for this
ansatz.

Specifically, as illustrated in Fig. \ref{fig:ch6:he}, the hardware-efficient ansatz implements a PQC given by a cascade of $L$ layers
of unitaries as in
\begin{equation}
	U(\theta)=U_{L}(\theta)\cdot U_{L-1}(\theta)\cdots U_{1}(\theta),
\end{equation}
where each unitary matrix $U_{l}(\theta)$ at the $l$th layer can
be expressed as
\begin{equation}
	U_{l}(\theta)=U_{ent}\left(R(\theta_{l,0}^{1},\theta_{l,0}^{2},\theta_{l,0}^{3})\otimes\cdots\otimes R(\theta_{l,n-1}^{1},\theta_{l,n-1}^{2},\theta_{l,n-1}^{3})\right),
\end{equation}
with $\theta_{l,k}^{1},\theta_{l,k}^{2},\theta_{l,k}^{3}$ for $k=1,...,n$
being scalar parameters that belong to vector $\theta.$
Note that we have $D=3nL$ parameters in vector $\theta.$

\begin{figure}
\begin{center}
	\includegraphics[clip,scale=0.32]{figvqe1}
	\par\end{center}\vspace{-0.4cm}\caption{The hardware-efficient ansatz consists of $L$ layers, each encompassing general single-qubit gates applied in parallel to the $n$ qubits and a fixed entangling circuit $U_{ent}$. The qubits are initially in the ground state $|0\rangle$. \label{fig:ch6:he}}
\end{figure}


Accordingly, at each layer $l$, we apply separate single-qubit rotations
to all the $n$ qubits, as in the mean-field ansatz, and then we use
fixed entangling two-qubit gates defined by unitary $U_{ent}$.  The entangling unitary $U_{ent}$ is typically implemented using linear
or full entangling circuits. 
\textbf{Linear entangling circuits} implement entangling two-qubit gates between
successive qubits. The example in Fig. \ref{fig:ch6:linent} uses CZ gates, and it can be expressed as
\begin{equation}
	U_{ent}=\prod_{i=0}^{n-2}CZ_{i,i+1}.
\end{equation} \textbf{Full entangling circuits} implement entangling two-qubit gates between
all pairs of qubits as illustrated in Fig. \ref{fig:ch6:fullent} with CZ gates. 
In this regard, we observe that CZ gates have the advantage over CNOT gates that they can be applied in any order since they commute. 

\begin{figure}
\begin{center}
		\begin{quantikz} 
			\qw & \ctrl{1} & \qw & \qw & \qw & \\
			\qw &\ctrl{-1}& \ctrl{1} & \qw & \qw &\\	
			\qw &\qw& \ctrl{-1} & \ctrl{1} &\qw \\
			\qw &\qw& \qw & \ctrl{-1} & \qw 
			
		\end{quantikz}
\end{center}\vspace{-0.4cm} \caption{A linear entangling circuit $U_{ent}$ for $n=4$ qubits implemented via CZ gates.\label{fig:ch6:linent}}
\end{figure}

%


\begin{figure}
\begin{center}
		\begin{quantikz} 
			\qw & \ctrl{1} & \qw & \qw & \ctrl{2} & \qw & \ctrl{3} & \qw\\
			\qw &\ctrl{-1}& \ctrl{1} & \qw & \qw & \ctrl{2} & \qw & \qw\\	
			\qw &\qw& \ctrl{-1} & \ctrl{1} &\ctrl{-2} & \qw & \qw & \qw\\
			\qw &\qw& \qw & \ctrl{-1} & \qw & \ctrl{-2} & \ctrl{-3} & \qw
			
		\end{quantikz}
\end{center}\vspace{-0.4cm} \caption{A full entangling circuit $U_{ent}$ for $n=4$ qubits implemented via CZ gates.\label{fig:ch6:fullent}}
\end{figure}



The hardware-efficient ansatz is generic, and plays a similar role
to fully connected classical neural networks in the design of quantum
machine learning.
That said, it is important to stress that a hardware-efficient
ansatz does not have similar properties as fully connected classical
neural networks in terms of dependence on model parameters. 
Notably, in fully connected classical neural networks, one has significant
freedom in optimizing the connectivity between neurons by designing
the individual synaptic weights are biases.
In contrast, in the hardware-efficient ansatz, one can control only
the rotations applied to each individual qubit, and dependences among
qubits are dictated by fixed entangling circuits. 


\subsection{Parametrized Two-Qubit Gates}

At a higher level of complexity with respect to the hardware-efficient ansatz are PQCs that include also parametrized two-qubit gates. Most commonly, two-qubit gates include parametrized controlled gates and two-qubit Pauli rotations. We review them in turn in this subsection.

Using the notation introduced in Sec. \ref{sec:ch2:controlled}, \textbf{parametrized two-qubit controlled gates}  are of the form
$C_{jk}^{U(\theta)}$, where $j$ is the index of controlling qubit, 
 $k$ of the controlled qubit, and $U(\theta)$ is a parametrized single-qubit gate. 
Considering for simplicity of notation qubit $0$ as the controlling qubit and qubit $1$ as the controlled qubit, we have (cf. \ref{eq:ch2:cu})
\begin{equation}
	C_{01}^{U(\theta)}=|0\rangle\langle0|\otimes I+|1\rangle\langle1|\otimes U(\theta).
\end{equation} Therefore, on the ``branch'' of the computation in which the controlling qubit has state $|0\rangle$ no operation is applied to controlled qubit; while on the ``branch'' in which the controlling qubit has state $|1\rangle$ the parametrized single-qubit gate $U(\theta)$ is applied.

Typical examples of parametrized two-qubit gates include the \textbf{parametrized CNOT gate}
\begin{equation}
	\textrm{CNOT}_{jk}(\theta)=C_{jk}^{R_{x}(\theta)},
\end{equation}
where the controlled single-qubit gate is a Pauli $X$ rotation $R_{x}(\theta)$; and
the \textbf{parametrized CZ gate}
\begin{equation}
	\textrm{CZ}_{jk}(\theta)=C_{jk}^{R_{z}(\theta)},
\end{equation}
where the controlled single-qubit gate is a Pauli $Z$ rotation $R_{z}(\theta)$. Note that, by (\ref{eq:ch6:Rx})-(\ref{eq:ch6:Rz}),  we recover the standard CNOT and CZ gates by setting $\theta=-\pi$, apart from a phase term.


As a more complex solution than parametrized two-qubit gates, we have \textbf{two-qubit Pauli rotations}. For a system with two qubits, they are defined as 
\begin{equation}
	R_{pq}(\theta)=\exp\left(-i\frac{\theta}{2}(P\otimes Q)\right),
\end{equation}
where $P$ and $Q$ are selected as one of the four Pauli operators
$\{X,Y,Z\}$.
A common example is the \textbf{Pauli $ZZ$ rotation gate} defined
by the unitary
\begin{equation}
	R_{zz}(\theta)=\exp\left(-i\frac{\theta}{2}Z\otimes Z\right).
\end{equation}
Note that, despite the presence of the product $P\otimes Q$, two-qubit
Pauli rotations are generally not separable. In this regard, note that we have $R_{zz}(-\pi)=i(Z\otimes Z)$, so
that with the special choice of $\theta=-\pi$ the gate $R_{zz}(-\pi)$
is separable.
More generally, the Pauli $ZZ$ rotation can be implemented as the
cascade of CNOT, Pauli $Z$ rotation, and CNOT gate as in Fig. \ref{fig:ch6:Rzz}.

\begin{figure}
\begin{center}
		\begin{quantikz} 
			\qw & \ctrl{1} & \qw & \ctrl{1} & \qw & \\
			\qw &\gate{X}& \gate{R_z(\theta)} & \gate{X}& \qw 
			
		\end{quantikz}
\end{center}\vspace{-0.4cm} \caption{An implementation of the Pauli $ZZ$ rotation gate \label{fig:ch6:Rzz}}
\end{figure}



Recalling the notation $P_{j}$ for a single-qubit gate applied only
to the $j$th qubit, when applied to any two qubits $j$ and $k$, two-qubit rotation gates can be expressed as 
\begin{equation}
	R_{P_{j}Q_{k}}(\theta)=\exp\left(-i\frac{\theta}{2}(P_{j}Q_{k})\right),
\end{equation}
i.e., as the $2^{n}\times2^{n}$ unitary generated by the Pauli string with
all $2\times2$ identities except for $P_{j}\in\{X,Y,Z\}$ in the
$j$th position and $Q_{k}\in\{X,Y,Z\}$ in the $k$th position.
For example, we can write
\begin{equation}
	R_{z_{j}z_{k}}(\theta)=\exp\left(-i\frac{\theta}{2}Z_{j}Z_{k}\right)
\end{equation}
to denote a two-qubit Pauli $ZZ$ rotation acting on qubits $k$ and
$j$. 


%
\section{Variational Quantum Eigensolver}

In this section, we describe a first application of the methodology illustrated in Fig. \ref{fig:ch6:qmlintro}, whereby the parameter vector $\theta$ of a PQC is designed via a classical optimizer that receives as input measurements of the PQC's output state. Specifically, the  variational quantum eigensolver
(VQE) will be introduced as a means to address a class of binary combinatorial
optimization problems, namely quadratic unconstrained binary optimization
(QUBO) problems. Broader applications of VQEs will be also covered later in this section. While VQEs are not data-driven, and hence may not qualify as ``machine learning'', they serve as a useful stepping stone to describe quantum machine
learning applications. In fact, VQEs optimize the model parameter $\theta$ by minimizing the expectation of an observable under the quantum state produced by the PQC. As we will see in the next sections, this approach is common to most quantum machine learning methods.

\subsection{Quadratic Unconstrained Binary Optimization}

A QUBO can be formulated as the combinatorial optimization
\begin{align}\label{eq:ch6:qubo}
	\min_{\tilde{x}\in\{-1,1\}^{n}}\left\{ f(\tilde{x})=\sum_{k=0}^{n-1}\sum_{j=0}^{k-1}a_{k,j}\tilde{x}_{k}\tilde{x}_{j}+\sum_{k=0}^{n-1}b_{k}\tilde{x}_{k}\right\},
\end{align}
with coefficients $\{a_{k,j},b_{k}\}.$ QUBO has a wide range of applications from finance and economics to
machine learning. 
The exact solution of a QUBO generally requires a search over the exponentially
large space, in $n$, of the binary optimization vector $\tilde{x}$. We will assume for simplicity that the problem has a single optimum solution 
$\tilde{x}^{*}\in\{-1,1\}^{n}.$


Problem (\ref{eq:ch6:qubo}) can be equivalently expressed in terms of a binary vector $x\in\{0,1\}^{n}$. To this end, one assigns each binary string  $x\in\{0,1\}^{n}$ to the binary
string $\tilde{x}\in\{-1,1\}^{n}$, which has entries $\tilde{x}_{k}=-1$
for $x_{k}=1$ and $\tilde{x}_{k}=1$ for $x_{k}=0$ for $k\in\{0,1,...,n-1\}$. The mapping between the two vectors is hence given by the entry-wise equality
\begin{equation}
	\tilde{x}_{k}=1-2x_{k}
\end{equation}
for $k\in\{0,1,...,n-1\}.$
We will write this assignment for short as $\tilde{x}=1-2x$, in which
the operations are element-wise.



\subsection{QUBO Objective as a Quantum Observable}

In order to address the QUBO problem (\ref{eq:ch6:qubo}) with a PQC, we start by expressing
the objective function $f(\cdot)$ in terms of a quantum observable
$F$ on $n$ qubits.
As we will see in the next subsections, the main idea underlying VQEs is to design the PQC to output $n$ qubits in a state
that (approximately) minimizes the expectation of the observable $F$.

The objective function $f(\cdot)$ can be associated with the following
observable defined on $n$ qubits
\begin{equation}\label{eq:ch6:obsF}
	F=\sum_{k=0}^{n-1}\sum_{j=0}^{k-1}a_{k,j}Z_{k}Z_{j}+\sum_{k=0}^{n-1}b_{k}Z_{k},
\end{equation}
which is also known as the \textbf{Ising Hamiltonian}. We recall from the previous section that the matrix $Z_k$ is defined as in (\ref{eq:ch6:Zk}). 
This observable is the sum of $n(n-1)/2+n$ observables, each given
by a Pauli string consisting of Pauli operators $\{I,Z\}$. Each individual observable in (\ref{eq:ch6:obsF}) corresponds to the term in (\ref{eq:ch6:qubo}) obtained by replacing the Pauli string $Z_k$ with the binary variable $\tilde{x}_k$. 


The association between objective function $f(\cdot)$ in (\ref{eq:ch6:qubo}) and the observable
$F$ in (\ref{eq:ch6:obsF}) is in the following sense:\begin{itemize}
\item \textbf{Eigenvectors as solutions}: The observable $F$ has eigenvectors given by the vectors $\{|x\rangle\}_{x=0}^{2^{n}-1}$
of the computational basis. Hence, each eigenvector $|x\rangle$ corresponds to a possible solution $\tilde{x}=1-2x$ of the QUBO problem.
\item \textbf{Eigenvalues as objective function values}: Each eigenvector $|x\rangle$ has corresponding eigenvalue $f(\tilde{x})$,
with $\tilde{x}=1-2x.$
\end{itemize} The two conditions can be summarized mathematically as the equalities \begin{equation}\label{eq:ch6:eigVQE}
	F|x\rangle=f(\tilde{x})|x\rangle,
\end{equation} which hold for all $x\in\{0,1,...,2^{n}-1\}$. These equalities reveal that the value $f(\tilde{x})$ of the objective function at any candidate solution $\tilde{x}\in\{-1,1\}^{n}$ can be computed by evaluating the eigenvalue of the observable $F$ corresponding to the eigenvector $|x\rangle$ with $\tilde{x}=1-2x.$

To prove the key equality (\ref{eq:ch6:eigVQE}), recall that the eigendecomposition of the
Pauli $Z$ operator implies the equality 
\begin{equation}
	Z_{k}Z_{j}|x\rangle=\tilde{x}_{k}\tilde{x}_{j}|x\rangle\textrm{ and }Z_{k}|x\rangle=\tilde{x}_{k}|x\rangle,
\end{equation}where $\tilde{x}_k$ is the $k$th element of vector $\tilde{x}=1-2x.$ 
It follows that we have
\begin{align}
	F|x\rangle & =\sum_{k=0}^{n-1}\sum_{j=0}^{k-1}a_{k,j}\left(Z_{k}Z_{j}|x\rangle\right)+\sum_{k=0}^{n-1}b_{k}Z_{k}|x\rangle \nonumber\\
	& =\sum_{k=0}^{n-1}\sum_{j=0}^{k-1}a_{k,j}\tilde{x}_{k}\tilde{x}_{j}|x\rangle+\sum_{k=0}^{n-1}b_{k}\tilde{x}_{k}|x\rangle.
\end{align}

\subsection{QUBO Minimization as a Minimum-Eigenvalue Problem}\label{sec:ch6:mineig}

Given the equality (\ref{eq:ch6:eigVQE}), the minimum eigenvalue of the observable $F$ corresponds to the minimum value $f(\tilde{x}^{*})$ of the QUBO problem. It is a well-known result from linear algebra that the minimum eigenvalue of a Hermitian matrix can be obtained by solving the problem 	\begin{equation} \min_{|\psi\rangle}\langle\psi|F|\psi\rangle
	\end{equation} over all possible normalized $2^n$ vectors $|\psi\rangle$. Therefore, the QUBO problem can be equivalently solved by addressing the \textbf{minimum-eigenvalue problem}\begin{equation}\label{eq:ch6:QUBOeig}
	\min_{|\psi\rangle}\langle\psi|F|\psi\rangle=\min_{\tilde{x}\in\{-1,1\}^{n}}f(\tilde{x})=f(\tilde{x}^{*}).
\end{equation} Note that the optimal solution $|\psi^{*}\rangle$ of problem (\ref{eq:ch6:QUBOeig}) provides, by (\ref{eq:ch6:eigVQE}), the solution of the QUBO problem in the sense that we have the equality $|\psi^{*}\rangle=|x^*\rangle$ with $\tilde{x}^{*}=1-2x^{*}$.

\subsection{QUBO Minimization as a Minimization of the Expected Value of an Observable}

The discussion in the previous subsection does not provide direct insights into how the minimum eigenvalue problem (\ref{eq:ch6:QUBOeig}) could be practically addressed using a quantum computer. To discuss this important point, let us consider the measurement of the observable $F$ under the state $|\psi\rangle$ produced by a quantum algorithm. (In the next subsection, we will assume this state to be the output of the PQC.) Since an eigenbasis of $F$ is, by (\ref{eq:ch6:eigVQE}),  the computational basis, from Sec. \ref{sec:ch5:obs}, measuring $F$ amounts to performing a standard measurement. This measurement returns the eigenvalue $f(\tilde{x})$ with
probability $\langle x|F|x\rangle$, where $\tilde{x}=1-2x$. 


Suppose now that we perform multiple measurements of the observable $F$ by producing state $|\psi\rangle$ multiple times.  Given a state $|\psi\rangle=\sum_{x=0}^{2^{n}-1}\alpha_{x}|x\rangle$
of the $n$ qubits, the expectation of the observable $F$ is given
by \begin{equation}
	\langle F\rangle_{|\psi\rangle}=\langle\psi|F|\psi\rangle=\sum_{x=0}^{2^{n}-1}|\alpha_{x}|^{2} f(\tilde{x}=1-2x).
\end{equation}Therefore, the expectation is a weighted average of all the values $f(\tilde{x}=1-2x)$ of the objective function, with weight given by the corresponding amplitude $|\alpha_{x}|^{2}$ of the input state. 

The discussion in the previous paragraph implies that the minimum value of the expectation $\langle F\rangle_{|\psi\rangle}$ is attained when the amplitudes $\alpha_x$ of the input state $|\psi\rangle$ in the computational basis are all equal to $0$ except for the vector $|x^{*}\rangle$ corresponding to the optimal solution $\tilde{x}^{*}=1-2x^{*}$ of the QUBO problem. This follows directly from the fact that $f(\tilde{x}^{*})$ is the (unique) minimum value of the objective function.

The problem of minimizing the expectation $\langle F\rangle_{|\psi\rangle}=\langle\psi|F|\psi\rangle$ is equivalent to the minimum-eigenvalue problem (\ref{eq:ch6:QUBOeig}). Therefore, we have the equalities \begin{align}\label{eq:ch6:QUBOexp}
	\min_{|\psi\rangle} \langle F\rangle_{|\psi\rangle} & = \min_{|\psi\rangle}\langle\psi|F|\psi\rangle = \langle F\rangle_{|x^{*}\rangle}\nonumber\\ &=\min_{\tilde{x}\in\{-1,1\}^{n}}f(\tilde{x})=f(\tilde{x}^{*}), 
\end{align} 
 where $\tilde{x}^{*}=1-2x^{*}$. 

Overall, the discussion in the last two subsections has shown that the QUBO problem can be equivalently addressed by searching for the quantum state $|\psi^{*}\rangle=|x^{*}\rangle$, with $x\in\{0,1\}^{n}$, that minimizes the expectation $\langle F\rangle_{|\psi^{*}\rangle}$. 


\subsection{Variational Quantum Eigensolver}\label{sec:ch6:vqe}

The key idea underlying VQEs is to replace the optimization over state
$|\psi\rangle$ in (\ref{eq:ch6:QUBOexp}) with an optimization over the parameters $\theta$
of the PQC. 
Specifically, as illustrated in Fig. \ref{fig:ch6:vqe}, the VQE design methodology starts off by assuming a given ansatz for the PQC implementing a parametrized unitary $U(\theta).$ The PQC produces the parametrized quantum state
\begin{equation}
	|\psi(\theta)\rangle=U(\theta)|0\rangle.
\end{equation}
For any vector $\theta$, the expected value of the observable $F$ is
given by $\langle F\rangle_{|\psi(\theta)\rangle}=\langle\psi(\theta)|F|\psi(\theta)\rangle$. The goal of the classical optimizer in Fig. \ref{fig:ch6:vqe} is to use estimates of the expected value $\langle F\rangle_{|\psi(\theta)\rangle}$ to address the problem of minimizing
$\langle F\rangle_{|\psi(\theta)\rangle}$ over vector $\theta$, i.e.,
\begin{equation}\label{eq:ch6:vqeopt}
	\min_{\theta}\left\{ L(\theta)=\langle F\rangle_{|\psi(\theta)\rangle}=\langle\psi(\theta)|F|\psi(\theta)\rangle=\langle0|U(\theta)^{\dagger}FU(\theta)|0\rangle\right\} .
\end{equation}

\begin{figure}
	\begin{center}
		\includegraphics[clip,scale=0.32]{figqml4}
		\par\end{center}\vspace{-0.4cm}\caption{Illustration of the operation of a VQE. The classical optimizer aims at minimizing the expected value $\langle F \rangle_{F} =\rangle\langle \psi(\theta)|F| \psi(\theta)\rangle$ of the observable $F$.\label{fig:ch6:vqe}}
\end{figure}

The solution of the VQE problem (\ref{eq:ch6:vqeopt}) generally provides an upper bound on the minimum
value of the cost function, i.e., 
\begin{equation}
	\min_{\theta}L(\theta)\geq\min_{|\psi\rangle}\langle\psi|F|\psi\rangle=f(\tilde{x}^{*}),
\end{equation}
and tightness of the bound depends on the flexibility of the ansatz underlying the PQC $U(\theta)$. In fact, if there exists a model parameter $\theta^{*}$ such that the PQC produces the optimal state, i.e., such that we have 
$|\psi(\theta^{*})\rangle=|x^{*}\rangle$, the solution of the VQE
problem coincides with the optimal solution of the QUBO problem. 
As we discussed in the previous section, this is the case even with a simple mean-field ansatz
using only Pauli $Y$ rotations, since the latter can produce any vector in the computational basis. 
That said, in practice, exact optimization of problem (\ref{eq:ch6:vqeopt}) is not possible, and hence
one is not guaranteed to recover the optimal solution. We will discuss solutions methods in the next subsection.


Having (approximately) solved the problem (\ref{eq:ch6:vqeopt}), how can one extract a solution?
If the goal is merely to compute the minimum value $f(\tilde{x}^{*})$ of the objective
function, an estimate of the optimal objective $f(\tilde{x}^{*})$
can be obtained by estimating the expectation $\langle F \rangle_{|\psi(\theta^{*})\rangle}$
for the optimized parameters $\theta^{*}.$ As we recall in the next subsection, estimating this expectation requires making multiple measurements from a number of runs of the PQC. 
Estimating the solution $\tilde{x}^{*}$ is instead possible by making
a single measurement of the state $|\psi(\theta^{*})\rangle$. In fact, such a measurement returns a vector $|x\rangle$ in the computational basis, whose corresponding signed vector $\tilde{x}$ can bet taken to be an approximation of the optimal solution $\tilde{x}^{*}$. 
In this regard, it has been pointed out that, if the goal is estimating
the solution $\tilde{x}^{*}$, optimizing quantiles of the distribution
of the observable $F$ may be preferable to optimizing the mean as
done by the standard VQE.


\subsection{Addressing the VQE Optimization Problem}

In order to address the VQE problem (\ref{eq:ch6:vqeopt}), the classical optimizer should first be able to estimate the 
expected value $\langle F\rangle_{|\psi(\theta)\rangle}$ for given candidate solutions $\theta$. 
By the decomposition of the observable $F$ into Pauli strings, we can write the expectation as
have
	\begin{equation}\label{eq:ch6:mF}
		\langle F\rangle_{|\psi(\theta)\rangle}=\sum_{k=0}^{n-1}\sum_{j=0}^{k-1}a_{k,j}\langle Z_{k}Z_{j}\rangle_{|\psi(\theta)\rangle}+\sum_{k=0}^{n-1}b_{k}\langle Z_{k}\rangle_{|\psi(\theta)\rangle}.
	\end{equation}Following Sec. \ref{sec:ch5:projmeas}, all the  $n(n-1)/2+n$ expectations in (\ref{eq:ch6:mF}) can be approximated via empirical averages obtained
from multiple measurements in the computational basis of the $n$
qubits in state $|\psi(\theta)\rangle$. It is emphasized that, in practice, only a finite number $N_S$ of measurements can be made by the classical optimizer, with each measurement requiring to run the PQC anew. 
Randomness caused by the use of a finite number of measurements in the estimation of the expectation of an observable  is
known as \textbf{shot noise}. 


Optimization of problem (\ref{eq:ch6:vqeopt}) is typically carried out in an iterative way using local \textbf{gradient-based 
optimization}. Accordingly,  at the current iterate $\theta$ for the model parameter vectors, the classical optimizer obtains an estimate $\hat{\nabla}L(\theta)$
of the gradient 
\begin{equation}\label{eq:ch6:grad}
	\nabla L(\theta)=\left[\frac{\partial L(\theta)}{\partial\theta_{1}}\cdots\frac{\partial L(\theta)}{\partial\theta_{D}}\right]^{T}
\end{equation}
of the expected value $L(\theta)=\langle F \rangle_{|\psi(\theta)\rangle}$. Note that the classical optimizer can generally only evaluate an estimate subject to shot noise due to random measurements of the observable $F$. Having obtained estimate  $\hat{\nabla}L(\theta)$, the classical optimizer updates the parameter vector as \begin{equation}\theta\leftarrow\theta-\gamma\hat{\nabla}L(\theta) \end{equation} 
for some learning rate $\gamma>0$. The procedure is repeated for a number of iterations. We will discuss how to estimate the gradient of the expected value of an observable in the next section.

One of the important problems with using gradient descent on PQCs
is that, as the number of qubits grows, the loss
function $L(\theta)$ -- given by the expectation of an observable -- has been shown to tend exponentially
to zero in probability, i.e., $\Pr\left[\frac{\partial c(\theta)}{\partial\theta_{d}}>c\right]=O(a^{-n})$.
This is known as barren plateau problem, which applies under given assumptions on the ansatz.

In this regard, it should be noted that it is also possible to use global optimization strategies or other
forms of local optimization, e.g., based on second-order information.
One approach for global optimization is to leverage \textbf{surrogate objective
functions}, which extrapolate the value of the loss $L(\theta)$ across
different values of $\theta$.
The surrogate is typically updated sequentially based on previous
measurements.
One such method is Bayesian optimization.


\subsection{Other Applications of VQEs}

In this section, we have presented VQE as a means to address the QUBO problem. More generally, following the discussion in Sec. \ref{sec:ch6:mineig}, VQE can be adopted as a tool to tackle the problem of estimating
the minimum eigenvalue of an observable $F$. While the observable arising from the solution of a QUBO is given in terms of Pauli $Z$ operators, one may be more broadly interested in observables that can
be written as arbitrary linear combinations of Pauli strings. 
Therefore, the observable $F$ may include also the $X$ and $Y$
Pauli operators, as well as terms including more than two Pauli operators.
Most typically, one has terms of one- and two-qubit terms of the form
{$X_{k}X_{j}$, $X_{k}$, $Y_{k}Y_{j}$, $Y_{k}$, $Z_{k}Z_{j}$,
	$Z_{k}$. When implementing VQE for this more general class of observables, it should be kept in mind that it is only possible to measure simultaneously observables derived
from the same Pauli operator (see Sec. \ref{sec:ch5:compatible}), so the general observable of this form
requires three separable, i.e., qubit by qubit, measurements in the
$X$, $Y$, and $Z$ bases.



\section{Estimating the Gradient of the Expected Value of an Observable}\label{sec:ch6:estgrad}

In this section, we discuss the important problem of estimating the gradient of the expected value $\langle O \rangle_{|\psi(\theta)\rangle=U(\theta)|0\rangle}$ of an observable $O$ under the parametrized state $|\psi(\theta)\rangle$ produced by a PQC. Following the notation in the previous section, we will write this for short as the function of $\theta$ \begin{equation}\label{eq:ch6:obsdiff}
	L(\theta)=\langle O \rangle_{|\psi(\theta)\rangle=U(\theta)|0\rangle}.
\end{equation} As we have seen in the previous section, estimating the gradient $\nabla L(\theta)$ is a key step in the implementation of VQE solutions based on gradient descent (where the observable $O$ equals the Ising Hamiltonian $F$ in \ref{eq:ch6:obsF}). Furthermore, as we will discuss in the next sections, it is also a central subroutine for quantum machine learning. 

\subsection{Numerical Differentiation}
A natural idea is to estimate the gradient via numerical differentiation.
Accordingly, the $d$th partial derivative in the gradient (\ref{eq:ch6:grad}), for $d=1,...,D$,  is first approximated as 
\begin{equation}\label{eq:ch6:approxgrad}
	\frac{\partial L(\theta)}{\partial\theta_{d}}\simeq\frac{L(\theta+\epsilon e_{d})-L(\theta-\epsilon e_{d})}{2\epsilon},
\end{equation}
where $\epsilon>0$ is a small number and $e_{d}$ is a one-hot $D$-dimensional
vector with a 1 in position $d$. It can be readily checked that the error of the approximation (\ref{eq:ch6:approxgrad}) is of the order $\mathcal{O}(\epsilon^2)$, and hence it can be controlled by selecting a sufficiently small $\epsilon$. In words, the approximation (\ref{eq:ch6:approxgrad}) is obtained by perturbing each parameter $\theta_{d}$ by a small number $\epsilon$ in both positive and negative directions in order to evaluate
the corresponding partial derivative. 

The second step is to estimate both terms in the approximation (\ref{eq:ch6:approxgrad}) via empirical averages obtained from multiple measurements of the quantum state produced by the PQC. As illustrated in Fig. \ref{fig:ch6:numdiff},  for each $d$th parameter $\theta_d$, with $d=1,...,D$, we run the quantum circuit
$2N_{S}$ times, where $N_{S}$ is the number of runs, or shots, used to estimate
the expected value of the observable. In particular, $N_S$ measurements are used to estimate the expected value \begin{equation} L(\theta+\epsilon e_d)=\langle O \rangle_{|\psi(\theta+\epsilon e_d)\rangle=U(\theta+\epsilon e_d)|0\rangle},
\end{equation} and $N_S$ measurements are used to estimate the expected value\begin{equation} L(\theta-\epsilon e_d)=\langle O \rangle_{|\psi(\theta-\epsilon e_d)\rangle=U(\theta-\epsilon e_d)|0\rangle}.
\end{equation} It follows that a total number of $2DN_S$ measurements are needed to estimate the gradient vector at one model parameter vector $\theta$.

\begin{figure}
\begin{center}
	\includegraphics[clip,scale=0.32]{figvqe2}
	\par\end{center}\vspace{-0.4cm} \caption{Numerical differentiation method to estimate the gradient of the expectation of an observable (\ref{eq:ch6:obsdiff}). For each $d$th entry $\partial L(\theta)/ \partial \theta_d$ of the gradient, with $d=1,...,D$, one needs to carry out $2N_S$ separate measurements of the observable. $N_S$ measurements, or shots, are used to estimate the expected value $L(\theta+\epsilon e_d)$, and $N_S$ measurements are used to estimate the expected value $L(\theta-\epsilon e_d)$. \label{fig:ch6:numdiff} }
\end{figure}


\subsection{Parameter Shift Rule}


In classical machine learning, with neural networks used as models, the gradient of the loss function can be computed at once via backpropagation. Backpropagation consists of two runs through the model, once in the forward direction and once backwards. Backpropagation is hence significantly more efficient than numerical differentiation, since the latter requires a number of runs through the model that is proportional to $D$. No quantum counterpart of backpropagation exists, and hence the computation of the gradient is an inherently more complex, and less scalable, operation than in classical machine learning. 

That said, when only (possibly multi-qubit) Pauli rotations are used as parametric
gates in the PQC, a related approach, known as the \textbf{parameter shift rule}, can be proved to provide the exact gradient as the number of shots $N_S$ goes to infinity. As we elaborate in this subsection, the parameter shift rule does \emph{not} solve the scalability problem highlighted above, as it still requires a number of runs through the model proportional to $D$. The only advantage as compared to numerical differentiation is that the approximate equality in (\ref{eq:ch6:approxgrad}) can be turned into an equality without requiring the numerically problematic step of reducing the value of $\epsilon$. 

To elaborate, assume that each parameter $\theta_d$ contributes to the PQC through
a gate of the form
\begin{equation}\label{eq:ch6:UPauli}
	U_{d}(\theta)=\exp\left(-i\frac{\theta_d}{2}P_{d}\right),
\end{equation}
where the generator $P_{d}$ is a Pauli string. Note that the gate (\ref{eq:ch6:UPauli}) may apply to an arbitrary number of qubits, and that it encompasses as special case single- and two-qubit Pauli rotation gates discussed in Sec. \ref{sec:ch6:PQC}. Therefore, mean-field ansatz, hardware-efficient ansatz, as well as generalizations thereof involving parametrized two-qubit Pauli rotations  satisfy the assumption at hand.

Under this assumption, it can be proved that the partial derivative can be
exactly computed as (see Appendix B)
\begin{equation}\label{eq:ch6:psrule}
	\frac{\partial L(\theta)}{\partial\theta_{d}}=\frac{L\left(\theta+\frac{\pi}{2}e_{d}\right)-L\left(\theta-\frac{\pi}{2}e_{d}\right)}{2}.
\end{equation}
Therefore, the use of the ``numerical differentiation-like'' expression in (\ref{eq:ch6:psrule}) does not entail any approximation, unlike (\ref{eq:ch6:approxgrad}). Note that the shifts of the parameters in (\ref{eq:ch6:psrule}) take the specific value $\pi/2$ (and that the normalization term (\ref{eq:ch6:approxgrad}) is also modified in (\ref{eq:ch6:psrule})).  As anticipated, and as detailed in Fig. \ref{fig:ch6:psrule}, the parameter shift rule still entails the implementation of the same number $2DN_S$ of measurements. Furthermore, the procedure is equivalent to that depicted in Fig. \ref{fig:ch6:numdiff} for numerical differentiation, with the only caveat that the shift takes the specific value $pi/2$ and that the normalization constant is given by $1/2$.


\begin{figure}
\begin{center}
	\includegraphics[clip,scale=0.32]{figparshift}
	\par\end{center}\vspace{-0.4cm} \caption{Parameter shift rule to estimate the gradient of the expectation of an observable (\ref{eq:ch6:obsdiff}). For each $d$th entry $\partial L(\theta)/ \partial \theta_d$ of the gradient, with $d=1,...,D$, one needs to carry out $2N_S$ separate measurements of the observable. $N_S$ measurements, or shots, are used to estimate the expected value $L(\theta+\epsilon e_d)$, and $N_S$ measurements are used to estimate the expected value $L(\theta-\epsilon e_d)$. \label{fig:ch6:psrule} }
\end{figure}



\section{Unsupervised Learning for Generative Models}

As a first machine learning application of PQCs, this section studies the unsupervised
learning problem of training probabilistic models generating
random binary strings $x\in\{0,1\}^{n}$. 

\subsection{Using and Training Generative Models}\label{sec:ch6:genmod}

Given a training set $\text{\ensuremath{\mathcal{D}}=}\{x_{1},...,x_{|\mathcal{D}|}\}$ of $|\mathcal{D}|$ $n$-cbit strings, we would like to train a probabilistic model that is able to generate binary strings that are distributed in a manner that ``resembles'' the underlying, unknown, distribution of the data. 

As an example, one may think of $x$ as a black-and-white image, flattened into an $n$ dimensional vector, with black and white pixels identified by entries of the vector equal to $1$ and $0$, respectively. The goal of unsupervised learning in this context is that of training a model that can produce black-and-white images that are ``similar'' to those in the training set $\mathcal{D}$.

We are hence interested in probabilistic generative models that can produce random cbit strings $x$ from some parametric distribution $p(x|\theta)$, where $x\in\{0,1\}^n$ and $\theta$ is a vector of model parameters. Once trained, that is, once a vector $\theta$ is optimized, the model can be used by directly generating one, or more, random strings -- e.g., images -- $x\sim p(x|\theta)$.

Training relies on the definition of a loss function $\ell(x|\theta)$, which describes how suitable the generative model defined by distribution $p(x|\theta)$ is as a mechanism to generate the specific string $x$. Loss functions for probabilistic models are also known as \textbf{scoring functions}. A scoring function should be a non-increasing function of $p(x|\theta)$: A model $p(x|\theta)$ that assigns a low probability to a data point $x$ should be assigned a larger loss than a model $p(x|\theta)$ that assigns a high probability to a data point $x$. The most common scoring function is the \textbf{log-loss} \begin{equation}
	\ell(x|\theta)=-\log p(x|\theta),
\end{equation}also known as \textbf{cross-entropy loss} or \textbf{information theoretic suprise}, which is indeed a decreasing function of $p(x|\theta)$. Other scoring functions include the linear loss $\ell(x|\theta)=1-p(x|\theta)$.

Once a training loss is determined, the \textbf{training loss} is defined as \begin{equation}\label{eq:ch6:trloss}
	L_{\mathcal{D}}(\theta)=\frac{1}{|\mathcal{D}|}\sum_{x\in\mathcal{D}}\ell(x|\theta).
\end{equation} The goal of training is typically defined as the minimization of the training loss (\ref{eq:ch6:trloss}) -- a problem known as \textbf{empirical risk minimization}\begin{equation}\label{eq:ch6:erm}
\min_{\theta} L_{\mathcal{D}}(\theta).
\end{equation}

\subsection{Born Machines}

A PQC implementing a unitary $U(\theta)$, with some fixed model parameter vector $\theta$, on $n$ qubits can be readily used as a generative model. To this end, as illustrated in Fig. \ref{fig:ch6:Born}, one simply run the PQC \emph{once} and makes a measurement of the $n$ qubits in the computational basis. This produces a binary string $x \sim p(x|\theta)$, where the distribution $p(x|\theta)$ is dictated by the Born rule. As a result, generative models based on PQCs are also known as \textbf{Born machines}.

It is worth reiterating that a sample $x \sim p(x|\theta)$ is produced with a \emph{single} run of the PQC, hence not requiring multiple runs to average out the shot noise associated with quantum measurements. In this sense,  shot noise is actually useful for generative models, as it is leveraged to produce random
samples.
This is indeed a common feature of probabilistic models, as we will also
see in the next section for supervised learning. 



\begin{figure}
	\begin{center}
		\includegraphics[clip,scale=0.32]{figqml5}
		\par\end{center}\vspace{-0.4cm} \caption{For data generation, a Born machine implements a single run of the PQC $U(\theta)$ measuring a random cbit string $x\sim p(x|\theta)$. For training, a classical optimizer applies gradient descent based on estimates of the expectations of data-dependent observables. \label{fig:ch6:Born}}
\end{figure}

By Born's rule, a Born machine implementing a PQC $U(\theta)$ produces a bit string $x\in\{0,1\}^{n}$ with probability
\begin{equation}\label{eq:ch6:probgen}
	p(x|\theta)=|\langle x|\psi(\theta)\rangle|^{2},
\end{equation}where we recall that $\langle x|\psi(\theta)\rangle$ is the complex amplitude of the state $|\psi(\theta)\rangle$ associated with the computational basis vector $|x\rangle$.  


Having defined the probability (\ref{eq:ch6:probgen}), one can train a PQC by following the methodology described in Sec. \ref{sec:ch6:genmod}. Specifically, we first choose a scoring function $\ell(x|\theta)$ as a non-increasing function of the probability $p(x|\theta)$ in (\ref{eq:ch6:probgen}), such as the log-loss
\begin{equation}
	\ell(x|\theta)=-\log p(x|\theta)=-\log|\langle x|\psi(\theta)\rangle|^{2}.
\end{equation}


An interesting perspective on such loss functions stems from the interpretation of the quantity  $|\langle x|\psi(\theta)\rangle|^{2}$ in (\ref{eq:ch6:probgen})
as the \textbf{fidelity} between the two states $|x\rangle$
and $|\psi(\theta)\rangle$. 
The fidelity is an important metric in quantum theory that measures the degree to which one state can be ``confused''
for the other state based on a measurement of one of the two states. In this regard,  a loss function defined as a non-increasing function of the fidelity $|\langle x|\psi(\theta)\rangle|^{2}$ can be thought of as measuring how well the state $|\psi(\theta)\rangle$
represents the input data $x$ encoded in state $|x\rangle$.


As in the case of VQE reviewed in Sec. \ref{sec:ch6:vqe}, the loss function can be evaluated as a function of
the expectation of a particular observable, with the difference that here 
the observable depends on the data point $x$.
In fact, taking the log-loss as an example, the loss function for a data point $x$ can be written as
\begin{equation}\label{eq:ch6:logloss}
	\ell(x|\theta)=-\log\langle\psi(\theta)|F_{x}|\psi(\theta)\rangle=-\log\langle F_{x}\rangle_{|\psi(\theta)\rangle},
\end{equation}
where we have introduced the observable \begin{equation} F_{x}=|x\rangle\langle x|.
\end{equation} As anticipated, the observable $F_x$ depends on the data point $x$. Note that, unlike for sample generation, evaluating the loss 	$\ell(x|\theta)$ requires running the PQC multiple ($N_{S}$) times in order to estimate the observable. 

The ERM problem (\ref{eq:ch6:erm}) with loss function (\ref{eq:ch6:logloss}) -- or with a scoring function different from the log-loss -- is typically addressed via gradient descent or stochastic gradient descent. Obtaining the gradient of the training loss \begin{equation}\label{eq:ch6:gradgen}
	\nabla L_{\mathcal{D}}(\theta)=\frac{1}{|\mathcal{D}|}\sum_{x\in\mathcal{D}}\nabla \ell(x|\theta)
\end{equation} requires computing the individual gradients $\nabla \ell(x|\theta)$ for each training point. Since the loss function $\ell(x|\theta)$ is a function of the expected value of an observable, namely $F_x$, the procedures described in Sec. \ref{sec:ch6:estgrad} can be directly used for this purpose.  Stochastic gradient descent adds a further source of noise in the estimate of the gradient by sampling from the data set $\mathcal{D}$ and averaging the per-data point gradients $\nabla \ell(x|\theta)$ in (\ref{eq:ch6:gradgen}) only for the selected mini-batch of samples. 

 
%Given a training set $\text{\ensuremath{\mathcal{D}}=}\{x_{1},...,x_{|\mathcal{D}|}\},$
%we can define the training loss
%\begin{equation}
%	L_{\mathcal{D}}(\theta)=\frac{1}{|\mathcal{D}|}\sum_{x\in\mathcal{D}}\ell(x|\theta).
%\end{equation}
%This criterion can be again optimized using the tools described above
%including the parameter shift rule.
%In fact, the gradient $\nabla L_{\mathcal{D}}(\theta)$ of the loss
%$L_{\mathcal{D}}(\theta)$ is given by the average of the gradients
%$\nabla\ell(x|\theta)$, each of which can be evaluated in a manner
%similar to VQE.
%
\section{Supervised Learning}\label{sec:ch6:sl}

In this section, we study supervised learning, in which we have a classical
input $x$ in the form of a real-valued vector and a classical target variable $y$.
The target variable $y$ is a discrete variable for classification problems, while it is a real-valued vector in regression problems. We start by discussing the most common way to encode the input $x$ as an input to the PQC, and then cover separately probabilistic and deterministic models defined from the output of a PQC. 



\subsection{Angle Encoding}\label{sec:ch6:angleenc}
A common and efficient way to encode the input $x$ is via \textbf{angle encoding}. Angle encoding defines a unitary transformation $U(x,\theta)$ that depends on the input vector $x$ in a manner similar to the model parameters $\theta.$ 

Specifically, angle encoding adopts a PQC that alternates between unitaries dependent on input 
$x$ and unitaries dependent on the model parameter vector $\theta$ as 
\begin{equation}
	U(\theta)=W_{L}(\theta)V_{L}(x)\cdot W_{L-1}(\theta)V_{L-1}(x)\cdots W_{1}(\theta)V_{1}(x).
\end{equation} Note that, in this architecture, the data $x$ is potentially entered multiple times, i.e., at each layer $l$. The unitaries dependent on $x$ and $\theta$ -- i.e., $V_{l}(x)$
and $W_{l}(\theta)$ for $l=1,...,L$ -- in turn consist of a cascade of single-qubit rotations and, possibly parametrized, entangling gates as discussed in Sec. \ref{sec:ch6:PQC}. The name ``angle encoding'' reflects the standard choice of parameterized single- or two-qubit Pauli rotations for the unitaries  $V_{l}(x)$, so that the entries of vector $x$ play the role of angles defining such rotations. 
 
The two types of unitaries,  $V_{l}(x)$
and $W_{l}(\theta)$, may follow different ansatzes. For instance,
in some architectures, one uses single- and two-qubit rotations for
the unitaries $V_{l}(x)$, while fixed entangling gates are used for
the unitaries $W_{l}(\theta)$ as in the hardware-efficient ansatz. 

In order to enable the encoding of an input $x=[x_0,...,x_{M-1}]$ containing $M$ real numbers, angle encoding typically uses at least $M$ qubits.  For example, one could use a simple mean-field ansatz for the unitary $V_{l}(x)$, with \begin{equation}
	V_{l}(x)=R_p(x_0)\otimes \cdots \otimes R_p(x_{M-1}),
	\end{equation} where $R_p(\cdot)$ is some Pauli rotation. Accordingly, a separate rotation -- each determined by an entry of the vector -- is applied to a distinct qubit. As mentioned, the ansatz can be made more complex, and expressive, by adding also two-qubit gates.

The output state of the PQC $U(x,\theta)$, i.e., \begin{equation}
	|\psi(x,\theta)\rangle=U(x,\theta)|0\rangle,
\end{equation} is a function of the input $x$. Therefore, the quantum state $|\psi(x,\theta)\rangle$ is often the \textbf{quantum
embedding} of the classical input $x$ in that it ``lifts'' the classical input $x$ from the space of $M$-dimensional real vectors to a quantum state in the $2^n$ dimensional Hilbert space.
Note that the embedding can be controlled via the model parameter
$\theta.$

We refer to Sec. \ref{sec:ch6:beyondangle} for a discussion of alternative encoding methods that differ from angle encoding in terms of number of required qubits and information processing models.

\section{Inference and Training via Probabilistic Models for Supervised Learning}

In supervised learning, each data point consists of a pair $(x,y)$, with $x$ being a real-valued input and $y$ being the discrete or real-valued target variable. We are given a training set $\text{\ensuremath{\mathcal{D}}=}\{(x_{1},y_{1}),...,(x_{|\mathcal{D}|},y_{|\mathcal{D}|})\}$ of $|\mathcal{D}|$ such examples, and we would like to train a predictive model that maps an input $x$ to an output $y$ in such a way that the mapping reflects well the underlying, unknown, data distribution. We distinguish between probabilistic and deterministic models, and we consider first probabilistic models, whose behavior is similar to that of the generative models covered in the previous section.

We specifically focus on probabilistic models for classification, in which the
target variable is a binary string $y\in\{0,1\}^{m}$ with $m\leq n$. This accounts for settings in which the input $x$ belongs to one of  
$2^{m}$ classes, which are indexed by the binary string $y$. A probabilistic model outputs a random binary label $y$ given an input $x$ with a distribution defined by a parametrized conditional distribution $p(y|x,\theta)$. 

\textbf{Inference} in probabilistic models amounts to the random generation of a label $y\sim p(y|x,\theta)$ given the input $x$ to be classified. A single sample is sufficient to make a point prediction, and multiple samples can be used if one is also interested in quantifying uncertainty.

\textbf{Training} relies on the definition of a loss function $\ell(x,y|\theta)$ that measures the (lack of) accuracy of the model $p(y|x,\theta)$ when evaluated on an input-output pair $(x,y)$. As for generative models, the loss function is defined as a non-increasing (scoring) function of $p(y|x,\theta)$: A model $p(y|x,\theta)$ that assigns a low probability to the label $y$ of a data point $(x,y)$ is assigned a larger loss than a model $p(y|x,\theta)$ that assigns a high probability to $y$. The most common scoring function is the \textbf{log-loss} \begin{equation}
	\ell(x,y|\theta)=-\log p(y|x,\theta),
\end{equation}which is also known as \textbf{cross-entropy loss}. Other scoring functions include the linear loss $\ell(x,y|\theta)=1-p(y|x,\theta)$, which measures the probability of error when the true label is $y$ given input $x$.

 The goal of training is typically defined in terms of the \textbf{empirical risk minimization} problem (\ref{eq:ch6:erm}) with  \textbf{training loss}  \begin{equation}\label{eq:ch6:trloss1}
	L_{\mathcal{D}}(\theta)=\frac{1}{|\mathcal{D}|}\sum_{(x,y)\in\mathcal{D}}\ell(x,y|\theta).
\end{equation}
%
\subsection{Probabilistic Quantum Models for Classification}

As illustrated in Fig. \ref{fig:ch6:psup}, a probabilistic model for classification can be implemented via a PQC in a manner similar to a Born machine. In this subsection, we first discuss how to implement inference, i.e., prediction, via probabilistic quantum models and then we briefly describe the problem of training such models.

Consider first \textbf{inference} and hence assume that the model parameter vector $\theta$ is fixed. Given any input $x$ to be classified, the PQC $U(x,\theta)$ produces the quantum embedding $|\psi(x,\theta)\rangle$. We wish to extract a binary string $y$ of $m$ cbits -- the label assigned by the model to input $x$ -- from this state. This can be done by implementing a projective (partial) measurement with $2^m$ possible outputs (see Sec. \ref{sec:ch5:projmeas}). For instance,  for binary classification ($m=1$), one apply a parity measurement, whereby class $y=0$ is selected if the parity is even and $y=0$ if the parity is odd (see Sec. \ref{sec:ch5:paritymeas} for a description of the case $n=2$).  



\begin{figure}
\begin{center}
	\includegraphics[clip,scale=0.32]{figqml6}
	\par\end{center}\vspace{-0.4cm} \caption{For inference, a probabilistic quantum model implements a single run of the PQC $U(x,\theta)$, which produces via a projective measurement a discrete label $y$. For training, a classical optimizer applies gradient descent based on estimates of the expectations of data-dependent observables.  \label{fig:ch6:psup}}
\end{figure}


To formalize the outlined approach, each possible output $y\in\{0,1\}^{m}$ is assigned to  a projection matrix $\Pi_{y}$ to defined a projective measurement $\{\Pi_{y}\}_{y=0}^{2^{m}-1}.$ A random label $y$ is produced by the circuit at inference time by making a single measurement of the quantum embedding $|\psi(x,\theta)\rangle$.  Therefore, in order to carry out classification on any given input $x$,
one does not need to average the output of the measurement. Rather, the model leverages shot noise for sampling.


By the generalized Born rule  (\ref{eq:ch3:genBorn}), the outlined quantum probabilistic models implements a stochastic 
mapping between $x$ and $y$ defined by the probability
\begin{equation}\label{eq:ch6:probsl}
	p(y|x,\theta)=\langle\psi(x,\theta)|\Pi_{y}|\psi(x,\theta)\rangle=\langle\Pi_{y}\rangle_{|\psi(x,\theta)\rangle}.
\end{equation} As in the case of generative models, by (\ref{eq:ch6:probsl}), the probability $p(y|x,\theta)$ equals the expectation of a data-dependent observable.  Specifically, here the observable depends on the label $y$, and is given by the projector $\Pi_y$. (Recall that projection matrices are Hermitian and hence they also defined observables.) 


A loss functions may be directly defined via the log-loss 
\begin{equation}
	\ell(x,y|\theta)=-\log p(y|x,\theta)=-\log\langle\Pi_{y}\rangle_{|\psi(x,\theta)\rangle},
\end{equation}
or some other scoring rule.
The loss is hence expressed, once again, in terms of the expectation of an observable
dependent on $y$.
Estimating the vaue of the loss function hence requires repeating the measurement of
the observable multiple times. 
The ERM problem (\ref{eq:ch6:erm})  with training loss (\ref{eq:ch6:trloss1})  can be addressed by following similar
steps as described in the previous section for generative models.


%
\subsection{Inference and Training via Deterministic Models for Supervised Learning}

Deterministic models implement parametrized functions $h(x|\theta)$ of the input $x$. Function $h(x|\theta)$ typically returns a vector of real numbers. A typical implementation in classical machine learning adopts a neural network as the parametrized function $h(x|\theta)$. Deterministic models can be used for both regression and classification.

In the case of regression, at \textbf{inference time}, given an input $x$, the model may directly use the output  $h(x|\theta)$ as an estimate of the target variable $y$. In the case of classification, the function $h(x|\theta)$ is typically passed to a fixed function to produce either a hard decision or a probability distribution over the possible outcome values. For instance,  for binary classification, we can take the sign of the (scalar) function $h(x|\theta)$ to make a hard decision; or  ``squash'' the function
$h(x|\theta)$ using, e.g., the sigmoid function, to produce a
probability
\begin{equation}\label{eq:ch6:logreg}
	\Pr[y=1|x,\theta]=\sigma(h(x|\theta))=\frac{1}{1+\exp(-h(x|\theta))}.
\end{equation} Similarly, for multi-class classification, the (vector) function $h(x|\theta)$ can be used to define the logit vector to be fed to a softmax function in order to define a vector of probabilities on the class indices.

For \textbf{training}, the standard approach is again to tackle the ERM problem (\ref{eq:ch6:erm}) with training loss defined as in (\ref{eq:ch6:trloss1}). The loss function $\ell(x,y|\theta)$ is a function of the function $h(x|\theta)$. For example, for scalar regression, one can adopt the squared 
\begin{equation}
	\ell(x,y|\theta)=(y-h(x|\theta))^{2},
\end{equation}
whiled for binary classification with the logistic regression squashing function (\ref{eq:ch6:logreg}) one can choose the cross-entropy loss
\begin{equation}
	\ell(x,y|\theta)=-y\log\sigma(h(x|\theta))-(1-y)\sigma(-h(x|\theta)).
\end{equation}


\subsection{Deterministic Quantum Models for Classification and Regression} 

PQC can implement deterministic function $h(x|\theta)$ as illustrated in Fig. \ref{fig:ch6:dsup}. The main idea is to realize a deterministic function $h(x|\theta)$ by measuring the expected value of an observable $M$ under the quantum embedding $|\psi(x,\theta)\rangle$ produced by the PQC. 

Accordingly, for \textbf{inference}, given an input $x$, the PQC is run multiple times in order to estimate the expectation 
\begin{equation}\label{eq:ch6:expd}
	h_{M}(x|\theta)=\langle\psi(x,\theta)|M|\psi(x,\theta)\rangle=\langle M\rangle_{|\psi(x,\theta)\rangle},
\end{equation}where we have made explicit the dependence of the function $h_{M}(x|\theta)$ on the observable $M$. The function $h_{M}(x|\theta)$ can then be used as described in the previous subsection to carry out regression and classification decisions. Note that vector functions 	$h(x|\theta)$ can be implemented by measuring multiple observables, one for each entry of the vector $h(x|\theta)$. Importantly, unlike  probabilistic models, deterministic models require multiple runs of the PQC in order to mitigate the effect of shot noise in estimating the expectation (\ref{eq:ch6:expd}). 


\begin{figure}
	\begin{center}
		\includegraphics[clip,scale=0.32]{figqml6}
		\par\end{center}\vspace{-0.4cm} \caption{For inference, a deterministic quantum model implements multiple runs of the PQC $U(x,\theta)$ to estimate the expected value of an observable $M$ (or multiple observables). For training, a classical optimizer applies gradient descent based on estimates of the expectations of data-dependent observables.  \label{fig:ch6:dsup}}
\end{figure}
 


Function $h_{M}(x|\theta)$
is linear in the 
the observable $M$.
Therefore, deterministic quantum models effectively implement linear
discriminative functions in the space of quantum embeddings whose
weights are defined by the choice of the observable.
As such, deterministic quantum models are akin to classical kernel
methods in that they operate over a large feature space -- the Hilbert
space of dimension $2^{n}$ -- via linear operations.

Having defined the model output function as in (\ref{eq:ch6:expd}), loss functions can be directly defined as detailed in the previous subsection. In all cases, the loss function can be expressed in terms of the observable
$\langle M\rangle_{|\psi(x,\theta)\rangle}.$ Therefore, the ERM problem can be again addressed by using the optimization methods discussed in the context of generative models.


%
\section{Beyond Standard PQCs}

In some problems, it may be possible to choose specialized ansatzes
that follow a more principled approach than the generic 
ansatzes described in Sec. \ref{sec:ch6:PQC}. There are at least two ways to do this: \begin{itemize}
\item mimic the operation of classical neural networks, while retaining some of the unique advantages of quantum computation, such as superposition; and
\item relax and parametrize a handcrafted quantum algorithm.
\end{itemize}
In this section, we briefly review these two alternatives. 

\subsection{Mimicking Classical Neural Networks}

Consider first the class of ansatzes that tries to mimic the way in
which neurons operate in a classical neural network.
A classical neuron produces an output as a function of a linear combination
$\sum_{k}w_{k}x_{k}$ of the inputs $\{x_{k}\}$ to the neuron with
weights $\{w_{k}\}$. 

A standard deterministic neuron outputs $g\left(\sum_{k}w_{k}x_{k}\right)$
for some non-linear activation function $g(\cdot)$, such as a sigmoid
$\sigma(a)=(1+\exp(-a))$ or a threshold function.
A quantum neuron mimicking the operation of a classical deterministic
neuron would produce an output of the form $g\left(\sum_{k}w_{k}x_{k}\right)$
when the inputs are in the computational basis, i.e., classical, while
also being able to operate on superposition states.
Note that implementing such a neuron is not straightfoward due to
the linearity of quantum evolutions, and it typically requires the
introduction of mechanisms involving measurements.

As an alternative, a  classical probabilistic neuron produces outputs whose probabilities
depend on non-linear functions of $\sum_{k}w_{k}x_{k}$. 
A classical example is given by a binary classical neuron, which outputs
1 with probability $\sigma\left(\sum_{k}w_{k}x_{k}\right).$
Classical neurons of this type can be directly implemented using a quantum circuit via a measurement whose output probabilities are given by a function of the linear combination $\sum_{k}w_{k}x_{k}$ (see Sec. \ref{sec:ch3:spiking}). 

\subsection{Relaxing Handcrafted Quantum Algorithms}
An example of the second type of approaches that relax and parametrize
a handcrafted quantum algorithm is given by the Quantum Approximate
Optimization Algorithm (QAOA). QAOA provides a problem-dependent ansatz for the VQE applied to an Ising
Hamiltonian (see Sec. \ref{sec:ch6:vqe}).
QAOA uses knowledge of the loss function observable $F$ in (\ref{eq:ch6:obsF}) in order
to define the ansatz of the quantum circuit $U(\theta)$ producing
the state $|\psi(\theta)\rangle$.
QAOA consists of a first layer of Hadamard gates, producing the mixture
state $|+\rangle^{\otimes n},$ followed by multiple layers. 
Each layer alternates between unitary $U(F,\gamma)=\exp(-i\gamma F)$
dependent on the Ising Hamiltonian $F$ and unitary $U(B,\beta)=\exp(-i\beta B),$where
$B=\sum_{k=1}^{n}X_{k}$ and $X_{i}$ is the $X_{k}$ operator applied
to the $k$th qubit.
The circuit provides an asymptotic approximation of the so-called quantum adiabatic
algorithm as the number of layers goes to infinity.


%
\section{Beyond Angle Encoding}\label{sec:ch6:beyondangle}

In this chapter we have so far adopted angle encoding as a mechanism to classical information in the form of a real vector $x$, with $M$ entries, into a quantum state. As we have introduced in Sec. \ref{sec:ch6:angleenc}, angle encoding is an analog strategy in which the $M$ entries of vector $x$ are directly
mapped to continuous-valued angles of parametrized quantum gates. In this section, we briefly review two alternative ways to encode classical information in a quantum state, and we also give an example of the type of inference methods that may be enabled by such methods. 


\subsection{Amplitude Encoding}

Amplitude encoding is an analog strategy, like angle encoding, which is, however, exponentially more efficient in terms of the number of required qubits. Amplitude encoding maps each entry $x_{k}$ of vector $x$ into the $k$th amplitude of a quantum
state. Accordingly, the encoded state, or quantum embedding, for data $x$ is 
\begin{equation}\label{eq:ch6:aa}
	|\psi(x)\rangle=\sum_{k}x_{k}|k\rangle.
\end{equation}
Note that we have implicitly assumed the normalization condition $\sum_{k}|x_{k}|^{2}=1$, which may be guaranteed, e.g., by scaling appropriately the input data. 

Amplitude encoding requires a number of qubits equal to the logarithm
of the size of the input, i.e., $\log_2(M)$. This provides an exponential improvement in terms of efficiency
of the input representation. That said, 
the computational complexity of amplitude encoding -- that is, the number of quantum operations necessary to produce state (\ref{eq:ch6:aa}) -- is, however, generally linear in the size $M$ of the input 
 as for angle encoding. 


\subsection{Basis Encoding}

Unlike angle and amplitude encoding, basis encoding is a digital strategy, and
it enables the encoding of an entire data set $\mathcal{D}=\{x\}$
of $|\mathcal{D}|=D$ data points into a single quantum state. As we detail next, the number of qubits dictates the resolution of the representation of input $x$.

Basis encoding first converts each data point $x$ in the binary domain to produce a binary
string $x_{b}\in\{0,1\}^{n}$. Note that the number of bits $n$ determines the precision level of the binary representation. Then, the entire data set $\mathcal{D}$ is mapped to the quantum state
\begin{equation}\label{eq:ch6:npqs}
	|\psi(\mathcal{D})\rangle=\frac{1}{Z}\sum_{x\in\mathcal{D}}|x_{b}\rangle,
\end{equation}
where $Z$ is a suitable constant to ensure a unitary norm. 



\subsection{Non-Parametric Quantum Machine Learning}

How can quantum states such as (\ref{eq:ch6:npqs}) used in machine learning applications? In this section, we outline an approach for \textbf{density estimation} that is akin to \textbf{non-parametric} methods in classical machine learning. This is in the sense that the approach makes decisions by using the entire data set, in the form of state (\ref{eq:ch6:npqs}) without requiring a training stage. 

Given a data set $\text{\ensuremath{\mathcal{D}}=}\{x_{1},...,x_{|\mathcal{D}|}\}$ of $|\mathcal{D}|$ samples, density estimation aims at estimating the probability distribution $p(x)$ underlying the generation of the data. Consider a new point $x^*$ at which we would like to estimate the distribution $p(x^*)$. Intuitively, the probability  $p(x^*)$ should be larger the more ``similar'' $x^*$ to the data points in the training set $\mathcal{D}$. Therefore, one could conceive the use of the inner product 
\begin{equation}
\hat{p}(x^{*})	\propto |\langle\psi(x^{*})|\psi(\mathcal{D})\rangle|^{2}
\end{equation}
as a non-parametric (unnormalized) estimate of the probability. The estimate $\hat{p}(x^{*})$ can be evaluated as the expectation of the observable $|\psi(x^{*})\rangle\langle\psi(x^{*})|$ under the encoded state (\ref{eq:ch6:npqs}). 


%This implements a form of non-parametric density estimation somewhat
%akin to kernel density estimation.
%In fact, the estimate is proportional to 
%\begin{equation}
%	\left|\sum_{x\in\mathcal{D}}\langle\psi(x^{*})|\psi(x)\rangle\right|^{2}.
%\end{equation}
%Therefore, the estimated density at $x^{*}$ is larger when the embedding
%$|\psi(x^{*})\rangle$ is similar, in terms of inner products, to
%the available data.


%%
%{A Note of Caution}
%\begin{center}
%	\includegraphics[clip,scale=0.36]{table}
%	\par\end{center}
%
%
%%
%{From Quantum Supremacy to... {[}Schuld and Killoran '22{]}}
%
%What are good building blocks for quantum models?
%How can we bridge quantum computing and classical learning theory
%to gain a better understanding of quantum machine learning?
%How can we make quantum software ready for machine learning applications?
%
%
%
%%
%{Problems}

\section{Conclusions}
This chapter has provided an introduction to quantum machine learning, focusing on the most common setting in which data is classical and processing is quantum. For this ``CQ'' case, a parametrized quantum circuit (PQC) is optimized via a classical processor by minimizing estimates of the expected value of some observables, which generally depend on (classical) data. Gradient-based optimization for PQCs is significantly less efficient than its counterpart  for standard machine learning models. In fact, estimating the gradient entails a complexity that scales linearly with the number of model parameters, and it requires multiple runs through the model in order to mitigate measurement shot noise. 

This key distinction with respect to classical machine learning tools is one of the many differences between the two fields. While classical machine learning is typically applied to unstructured, large data sets with the goal of maximizing accuracy; ``CQ'' quantum machine learning is often applied to small, well-structured, data sets and ``quantum advantages'' are often measured in terms of efficiency. Efficiency is often evaluated in terms of the number of physical resources needed to implement a model: number of model parameters, number of bits/ qubits, training time, inference inference time, and so on. While it is possible to prove such advantages for very structured problems -- often lifted from problems such as factoring or search, for which quantum algorithms are known to be beneficial -- the current practice appears to be that of making limited comparisons via experiments, or sidestepping the question of ``quantum advantages'' altogether. 

Rather than focusing on establishing formal advantages, research in the field may focus on establishing effective building blocks for quantum machine learning models; understanding the relative merits of deterministic and probabilistic models; evaluating the impact of different data encoding techniques; developing effective software platforms; and investigating at a theoretical level the problem of generalization for given ansatzes.

\section{Recommended Resources}

Quantum machine learning is an emerging, very active, field of research. A useful starting point is the book \cite{schuld21}, which contains many pointers to papers published before 2021. For more recent work, the reader is referred to the online repository ArXiv (https://arxiv.org/), in which most up-to-date pre-prints can be found.


\section{Problems}
\begin{itemize}
\item Write the matrix representation (in the computational basis) of
the three unitaries $Z\otimes Z$, $CZ$, and $R_{zz}(\theta)=\exp\left(-i\frac{\theta}{2}Z\otimes Z\right)$.
Which one(s) are separable and why? Obtain eigenvalues and eigenvectors.
Which one(s) are also observables?
\item  Show that the Pauli $ZZ$ rotation can be implemented using two
CNOT gates and a Pauli $Z$ rotation.
\item  Prove that using only Pauli $Y$ rotations allows the mean-field
ansatz to produce all possible vectors in the computational basis.
\item  Describe the quantum adiabatic theorem and the quantum adiabatic
algorithm.
\item  Derive the parameter shift rule.
\item  Demonstrate some practical examples of applications of quantum
machine learning methods (from papers or using your own simulations).
\item  Describe an example of quantum-quantum machine learning problem.
\end{itemize}


\section*{Appendix A: On Unitaries with Pauli Strings as Generators}
%A unitary matrix $U$ can always be expressed in terms of a Hermitian
%matrix $G$ as
%\begin{equation}
%	U=\exp(-iG)
%\end{equation}
%The Hermitian matrix $G$ is known as the generator of the unitary
%$U$ (and is also known as the Hamiltonian).
%Note that this matrix is indeed unitary since Hermitian matrices satisfy
%the condition $G^{\dagger}=G$, which yields
%\begin{equation}
%	U^{\dagger}U=\exp(iG^{\dagger})\exp(-iG)=\exp(iG^{\dagger}-iG)=I=UU^{\dagger}.
%\end{equation}
%For the case of rotation gate, the Hermitian matrices are $\frac{\theta}{2}X,\frac{\theta}{2}Y,$and
%$\frac{\theta}{2}Z$. 
%More generally, the generators are often defined as strings of Pauli
%matrices.
%
%
%%
%{Unitaries and Generators}
In this appendix, we derive some useful properties of parametrized unitaries whose generators are given by Pauli strings. Examples include single-qubit and two-qubit Pauli rotation gates. Such unitaries can be written as 
\begin{equation}
	U(\theta)=\exp\left(-i\frac{\theta}{2}P\right),
\end{equation}
%for some Hermitian matrix $G$. 
%Recall that, given the eigendecomposition $G=\sum_{x=0}^{2^{n}-1}\lambda_{x}|v_{x}\rangle\langle v_{x}|=\sum_{x=0}^{2^{n}-1}\lambda_{x}v_{x}$,
%with $v_{x}=|v_{x}\rangle\langle v_{x}|$ and real eigenvalues $\lambda_{x}$,
%we can equivalently write 
%\begin{equation}
%	U(\theta)=\exp\left(-i\frac{\theta}{2}G\right)=\sum_{x=0}^{2^{n}-1}\exp\left(-i\frac{\theta}{2}\lambda_{x}\right)v_{x}.
%\end{equation}
where  $P$ is a Pauli string. 

A Pauli string $P$ has two 
distinct eigenvalues $+1$ and $-1$. Therefore, it can be expressed as  $P=\Pi_{0}-\Pi_{1},$ where $\Pi_{0}=\sum_{x:\textrm{ \ensuremath{\lambda_{x}=1}}}v_{x}$
is the projection matrix into the subspace spanned by the eigenvectors
associated with eigenvalue $+1$, and $\Pi_{1}=\sum_{x:\textrm{ \ensuremath{\lambda_{x}=-1}}}v_{x}$
is the projection matrix into the subspace spanned by the eigenvectors
associated with eigenvalue $-1$. 
Note that $\Pi_{0}+\Pi_{1}=I$, since the set of all eigenvectors
span the entire Hilbert space.

Given the above, we obtain the equality
\begin{align}
	U(\theta) & =\sum_{x=0}^{2^{n}-1}\exp\left(-i\frac{\theta}{2}\lambda_{x}\right)v_{x}\nonumber\\
	& =\Pi_{0}\exp\left(-i\frac{\theta}{2}\right)+\Pi_{1}\exp\left(i\frac{\theta}{2}\right)\nonumber\\
	& =\Pi_{0}\left(\cos\left(\frac{\theta}{2}\right)-i\sin\left(\frac{\theta}{2}\right)\right)+\Pi_{1}\left(\cos\left(\frac{\theta}{2}\right)+i\sin\left(\frac{\theta}{2}\right)\right)\nonumber\\
	& =\cos\left(\frac{\theta}{2}\right)\left(\Pi_{0}+\Pi_{1}\right)-i\sin\left(\frac{\theta}{2}\right)\left(\Pi_{0}-\Pi_{1}\right)\nonumber\\
	& =\cos\left(\frac{\theta}{2}\right)I-i\sin\left(\frac{\theta}{2}\right)G.
\end{align}
Note that if we set $\theta=\pm\pi/2$, we get 
\begin{equation}
	U\left(\pm\frac{\pi}{2}\right)=\frac{1}{\sqrt{2}}\left(I\mp iG\right).
\end{equation}


%
\section*{Appendix B: The Parameter Shift Rule}

Consider one of the scalar parameters of the parameter vector $\theta=[\theta_{1},...,\theta_{D}]^{T}$, say $\theta_d$.
We are interested in computing the partial derivative $\partial\langle O\rangle_{|\psi(\theta)\rangle}/\partial\theta_{d}$
for the expectation 
\begin{equation}\label{eq:ch6:app1}
	\langle O\rangle_{|\psi(\theta)\rangle}=\langle\psi(\theta)|O|\psi(\theta)\rangle=\langle0|U^{\dagger}(\theta)OU(\theta)|0\rangle
\end{equation}
of some observable $O$ under the output state $U(\theta)|0\rangle$
produced by a PQC. 
All the loss functions we have considered in the problems studied
above are functions of such expectations. 
Note that, in some cases, the unitary $U(\theta)$ may also depend
on input data $x$, and this can be easily accommodated in the analysis
by considering unitaries of the form $U(x,\theta)$. 
We also emphasize that loss functions of the form (\ref{eq:ch6:app1}) are also relevant
for QQ problems, in which the observable $O$ may depend on the target
quantum state.



As discussed, in many PQCs of interest, parameter $\theta_{d}$ enters
as part of the overall unitary in a single gate of the form 
\begin{equation}
	U_{d}(\theta_{d})=\exp\left(-i\frac{\theta_{d}}{2}G_{d}\right),
\end{equation}
where $G_{d}$ is the generator Hermitian matrix.
Examples include the Pauli rotation matrices used in the hardware-efficient
ansatz.
Accordingly, we can write the overall unitary transformation as
\begin{equation}
	U(\theta)=V(\theta_{-d})U_{d}(\theta_{d})W(\theta_{-d})
\end{equation}
for some unitaries $V(\theta_{-d})$ and $W(\theta_{-d})$ representing the gates applied before
and after the $d$th gate dependent on $\theta_{d}$. 
Unitaries $V(\theta_{-d})$ and $W(\theta_{-d})$ generally depend
on the parameters in vector $\theta$ other than the parameter $\theta_{d}.$
This is captured by the notation \textrm{$\theta_{-d}$. }


We write the expected observable as 
\begin{equation}
	\langle O\rangle_{|\psi(\theta)\rangle}=\langle\phi_{d}|U_{d}^{\dagger}(\theta_{d})R_{d}U_{d}(\theta_{d})|\phi_{d}\rangle,
\end{equation}
where $|\phi_{d}\rangle=W(\theta_{-d})|0\rangle$ and $R_{d}=V(\theta_{-d})^{\dagger}OV(\theta_{-d})$.
Note that $R_{d}$ is Hermitian.
This way, we have incorporated gates following and preceding the $d$th
gate in the quantum state $|\phi_{d}\rangle$ and in the observable
$R_{d}$, respectively.
The subscript in $|\phi_{d}\rangle$ and $R_{d}$ is used to emphasize
that both quantities depend on the index $d$. 


The partial derivative is computed as 
	\begin{align}
		\frac{\partial\langle O\rangle_{|\psi(\theta)\rangle}}{\partial\theta_{d}}= & \frac{\partial\langle\phi_{d}|U_{d}^{\dagger}(\theta_{d})R_{d}U_{d}(\theta_{d})|\phi_{d}\rangle}{\partial\theta_{d}}\nonumber \\
		= & \langle\phi_{d}|U_{d}^{\dagger}(\theta_{d})R_{d}\nabla_{\theta_{d}}U_{d}(\theta_{d})|\phi_{d}\rangle\\ & +\langle\phi_{d}|\nabla_{\theta_{d}}U_{d}^{\dagger}(\theta_{d})R_{d}U_{d}(\theta_{d})|\phi_{d}\rangle,
	\end{align}
where $\nabla_{\theta_{d}}U_{d}(\theta_{d})$ represents the matrix
of derivatives of the unitary $U_{d}(\theta_{d}),$ and a similar definition
applies to $\nabla_{\theta_{d}}U_{d}^{\dagger}(\theta_{d}).$
We have 
\begin{align}
	\nabla_{\theta_{d}}U_{d}(\theta_{d}) & =\nabla_{\theta_{d}}\exp\left(-i\frac{\theta_{d}}{2}G_{d}\right)\nonumber \\
	& =-\frac{1}{2}iG_{d}\exp\left(-i\frac{\theta_{d}}{2}G_{d}\right)=-\frac{1}{2}iG_{d}U_{d}(\theta_{d})
\end{align}
and 
\begin{equation}
	\nabla_{\theta_{d}}U_{d}^{\dagger}(\theta_{d})=\frac{i}{2}G_{d}U_{d}^{\dagger}(\theta_{d}).
\end{equation}

We conclude that the following equalities hold
\begin{align}
	U_{d}(\theta_{d})+2\nabla_{\theta_{d}}U_{d}(\theta_{d}) & =U_{d}(\theta_{d})-iG_{d}U_{d}(\theta_{d})\nonumber\\
	& =(I-iG_{d})U_{d}(\theta_{d})\nonumber\\
	& =\sqrt{2}U_{d}(\pi/2)U_{d}(\theta_{d})\nonumber\\
	& =\sqrt{2}U_{d}(\theta_{d}+\pi/2).
\end{align}
Similarly, we have \textrm{
	\begin{equation}
		U_{d}(\theta_{d})-2\nabla_{\theta_{d}}U_{d}(\theta_{d})=\sqrt{2}U_{d}(-\pi/2)U_{d}(\theta_{d})=\sqrt{2}U_{d}(\theta_{d}-\pi/2).
	\end{equation}
}


Finally, we write the partial derivative as 
	\begin{align}
		\frac{\partial\langle O\rangle_{|\psi(\theta)\rangle}}{\partial\theta_{d}}= & \frac{1}{4}\langle\phi_{d}|(U_{d}(\theta_{d})+2\nabla_{\theta_{d}}U_{d}(\theta_{d}))^{\dagger}R_{d}(U_{d}(\theta_{d})+2\nabla_{\theta_{d}}U_{d}(\theta_{d}))|\phi_{d}\rangle \nonumber\\
		& -\frac{1}{4}\langle\phi_{d}|(U_{d}(\theta_{d})-2\nabla_{\theta_{d}}U_{d}(\theta_{d}))^{\dagger}R_{d}(U_{d}(\theta_{d})-2\nabla_{\theta_{d}}U_{d}(\theta_{d}))|\phi_{d}\rangle,\nonumber\\
		= & \frac{1}{2}\langle\phi_{d}|U_{d}(\theta_{d}+\pi/2){}^{\dagger}R_{d}U_{d}(\theta_{d}+\pi/2)|\phi_{d}\rangle\nonumber\\
		& -\frac{1}{2}\langle\phi_{d}|U_{d}(\theta_{d}-\pi/2){}^{\dagger}R_{d}U_{d}(\theta_{d}-\pi/2)|\phi_{d}\rangle, 
	\end{align}concluding the derivation.






==> Chapter6/quantumch.tex <==
\section{Quantum Channels}

In the previous section we have introduced POVMs -- the most general form of quantum measurement -- by studying the setting in Fig. \ref{fig:ch5:povm}. In it, the quantum system of interest, encompassing $n$ qubits in some state $\rho$, interacts with $n'$ ancilla qubits through a general unitary transformation $U$, and then a selective measurement is made on the ancillas. Following the discussion in Sec. \ref{sec:ch3:decoh}, we can use the ancilla qubits also to model the environment in which the quantum computer of $n$ qubits operates. In this case, the unitary $U$ accounts for the unwanted interactions with the environment. Furthermore, the fact that the quantum computer does not have access to the environment can be modelled by assuming that the ancillas, rather than being measured selectively as in Fig. \ref{fig:ch5:povm}, are measured \emph{non-selectively} as shown in Fig. \ref{fig:ch5:qch}.

The setting in Fig. \ref{fig:ch5:qch} -- in which the system of interest interacts with ``environment'' qubits, initially in the ground state $|0\rangle$, through a unitary and then the environment qubits are measured non-selectively -- defines a \textbf{quantum channel}. Quantum channels are used to model the impact of noise due to decoherence in quantum computers. More broadly, as we will further discuss below, quantum channels represent general quantum operations on a quantum state $\rho$ that do not involve selective measurements.
		
	

\begin{figure}
\begin{center}
			\begin{quantikz} 
				\lstick{$\ket{0}$}& \gate[wires=2]{U}\qwbundle{} & \meter{} \qwbundle{}& \trash{\text{trash}} \qwbundle{}\\
				\lstick{$\rho$} & \qwbundle{} &  \qwbundle{} & \qw 
			\end{quantikz}
	\end{center}\vspace{-0.4cm} \caption{A quantum channel can be described as a setting in which the quantum system of interest, consisting of $n$ qubits, interacts with $n'$ ancilla, or ``environment'', qubits (via a unitary $U$), which are measurement non-selectively (i.e., the output of the measurement is discarded).\label{fig:ch5:qch}}
\end{figure}

From Sec. \ref{sec:ch5:povm}, we know that in the setting of Fig. \ref{fig:ch5:qch}, the state at the output of the unitary is given by (\ref{eq:ch5:povmfc}), which we rewrite here for convenience as \begin{equation}\label{eq:ch5:qc1} \sum_{y=0}^{N'-1}|y\rangle\otimes K_{y}|\psi\rangle,
 \end{equation} where we have $N'=2^{n'}$ and the $N\times N$ matrices $K_y$ satisfy condition (\ref{eq:ch5:povm1}), i.e., 	\begin{equation}\label{eq:ch5:povmfc}
 \sum_{y=0}^{N'-1}K_{y}^{\dagger}K_{y}=I.
\end{equation} Unlike Sec. \ref{sec:ch5:povm}, we now perform a non-selective measurement of the ancillas. The outcome of this operation on the $n$ qubits of interest can be formally described by the partial trace operation described in Sec. \ref{sec:ch3:partialtrace}.

Before applying the partial trace, let us follow an equivalent and more direct argument by assuming that the ancillas are measured in the computational basis ${|y\rangle}_{y=0}^{N'-1}$. Recall from Sec. \ref{sec:ch3:partialtrace} that the output of a non-selective measurement does not depend on the specific choice of orthonormal basis. By the generalized Born rule, from (\ref{eq:ch5:qc1}), we obtain the post-measurement state $K_{y}|\psi\rangle/\sqrt{p_y}$ with probability $p_y=K_{y}|\psi\rangle \langle \psi | K^\dagger_{y}$. It follows that, from the viewpoint of the system of interest, which does not have access to the measurement outcome $y$, the state of the system is described by the density matrix	\begin{align}
	\rho_{out} & = \sum_{y=0}^{2^{n'}-1} p_y \frac{K_{y}|\psi\rangle}{p_y}
	& =\sum_{y=0}^{2^{n'}-1}K_{y}\rho K_{y}^{\dagger}.
\end{align}

	
		 This result can also be obtained by tracing out the ancillas -- denoted as $A$ -- to account for a non-selective measurement
		of the ancillas. In fact, using the definition (\ref{eq:ch3:ptrace}) of partial trace, we evaluate the output state as
		\begin{align}
			\rho_{out} & =\textrm{tr}_{A}(U(|0\rangle\langle0|\otimes\rho_{in})U^{\dagger})\nonumber\\
			& =\sum_{y=0}^{2^{n'}-1}(I\otimes\langle y|)(U(|0\rangle\langle0|\otimes\rho)U^{\dagger})(I\otimes|y\rangle)\\
			& =\sum_{y=0}^{2^{n'}-1}K_{y}\rho K_{y}^{\dagger}.
		\end{align}
		 
		 	
		 To summarize, a \textbf{quantum channel} operating on $n$ qubits is defined by a set of  matrices $\{K_{y}\}_{y=0}^{r-1}$, for some integer $r$, 
		known as \textbf{Kraus matrices}, of dimension $2^{n}\times2^{n}$, which satisfy the property  satisfying
		the property (\ref{eq:ch5:povmfc}), restated here as
		\begin{equation}\label{eq:ch5:povmfc1}
		\sum_{y=0}^{r-1}K_{y}^{\dagger}K_{y}=I.
		\end{equation}
		Given an input state $\rho$, the output state produced by a quantum channel defined by Kraus matrices $\{K_{y}\}_{y=0}^{r-1}$ is given as 
		\begin{equation}\label{eq:ch5:qchinout}
		\rho_{out}=\sum_{y=0}^{r-1}K_{y}\rho K_{y}^{\dagger}=\mathcal{N}(\rho_{in}),
		\end{equation}where the notation $\mathcal{N}(\cdot)$ is often used to describe the operation of the channel.
	
	By (\ref{eq:ch5:qchinout}), one can intuitively think of a quantum channel as a quantum operation that modifies the input
	density $\rho$ to the (normalized version of the unnormalized)
	density $K_{y}\rho_{in}K_{y}^{\dagger}$ with probability $p_y$. Therefore, each Kraus matrix $K_{y}$ can be interpreted as a different type of error that the channel causes on the quantum state $\rho$.
	Unless $r=1,$ quantum channels are generally not reversible, as they
	describe situations in which the system gets entangled with  the ``environment'' causing information to be irretrievably lost.
		
%	
%	The first description of a quantum channel in terms of a partial trace
%	is known as the system-environment representation or as the Stinespring
%	representation.
%	
%		 Kraus matrices are equivalent up to a unitary transformation.
%		 Two Kraus representations are equivalent if we can write 
%		\[
%		K_{x}=\sum_{y}[U]_{xy}K_{y}^{'},
%		\]
%		where $U$ is a unitary matrix.
%		 Hence the Kraus representation of a quantum channel is not unique.
%		 A Kraus representation with the smallest number of terms in the sum
%		is known as a minimal representation.
	
 An equivalent way to define a quantum channels $\rho_{out}\mathcal{N}(\rho)$ is as follows. A quantum channel is a mapping $\rho_{out}\mathcal{N}(\rho)$ from a density matrix $\rho$ to a matrix $\rho_{out}$ that is \textbf{linear, completely positive (CP), and 			 trace preserving (TP)}. Therefore, quantum channels are also referred to as \textbf{CPTP operators}. Linearity is evident from the characterization (\ref{eq:ch5:qchinout}). The TP property says the output state has unitary trace, i.e., $\textrm{tr}(\rho_{out})$ -- a necessary condition since the output $\rho_{out}$ must be a density matrix. This property can be directly proved based on the condition (\ref{eq:ch5:povmfc1}).  Finally, the CP condition means that, when applied on a subset of a larger		system, the quantum channel yields a valid density for the whole system. This is a necessary condition to guarantee that, if the channel is applied to only to some qubits of a system, the resulting output matrix is still a valid density state.
 
%	
%
%%
%{Quantum Channels}
%	
%		 Linearity is evident (see also below for an equivalent representation
%		in terms of matrix-vector multiplication).
%		 Trace preservation can be checked as:
%		\begin{align*}
%			\mathrm{tr}(\rho_{out}) & =\sum_{x=0}^{r-1}\mathrm{tr}\left(K_{x}\rho_{in}K_{x}^{\dagger}\right)\\
%			& =\sum_{x=0}^{r-1}\mathrm{tr}\left(\rho_{in}K_{x}^{\dagger}K_{x}\right)=\mathrm{tr}\left(\rho_{in}\sum_{x=0}^{r-1}K_{x}^{\dagger}K_{x}\right)=1
%		\end{align*}
%		 Note that this explains the need for the condition \textrm{$\sum_{x=0}^{r-1}K_{x}^{\dagger}K_{x}=I$.}
%		 
	


	
%		 Quantum channels can be further generalized by allowing the number
%		of qubits being measured to be generally different (larger or smaller)
%		from the number of ancilla qubits.
%		 If the number of input qubits is $n_{in}$ and the number of output
%		qubits is $n_{out}$, a quantum channel, a quantum channel is defined
%		by a set of matrices $\{K_{x}\}_{x=0}^{r-1}$, known as Kraus matrices,
%		of dimension $2^{n_{out}}\times2^{n_{in}}$, satisfying the completeness
%		relationship
%		\[
%		\sum_{x=0}^{r-1}K_{x}^{\dagger}K_{x}=I_{2^{n_{in}}}.
%		\]
%		 The output state is given as 
%		\[
%		\rho_{out}=\sum_{x=0}^{r-1}K_{x}\rho_{in}K_{x}^{\dagger},
%		\]
%		 It can be proved that the number of Kraus operators $r$ can be bounded
%		without loss of generality by $2^{n_{in}+n_{out}}.$
	

		 Quantum channels, i.e., CPTP operators, include all quantum operations that do not involve
		a selective measurement, including trace and partial trace. In fact, CPTPs and POVMs -- with the latter used to describe selective measurements -- exhaust the set of all possible operations that can be applied to a quantum system. 	Examples of quantum channels include the following.
		
		
		 \noindent $\bullet$ \textbf{Quantum state preparation}: This is the process of preparing a quantum ensemble $\{p_{x},|v_{x}\rangle\},$
		i.e., a density matrix $\rho_{out}=\sum_{x}p_{x}|v_{x}\rangle\langle v_{x}|$. It can be described as a quatum channel with Kraus operators $K_{x}=\sqrt{p_{x}}|v_{x}\rangle$ ($\sum_{x}p_{x}\langle v_{x}|v_{x}\rangle=1$),
			yielding the output state \textrm{$\rho_{out}=\sum_{x=0}^{r-1}p_{x}|v_{x}\rangle\langle v_{x}|$}.
		
	\noindent \textbf{Pauli channels}: Pauli channels are single-qubit channels
		that have Kraus matrices
		\begin{equation}
		K_{0}=\sqrt{p_{0}}I,\textrm{}K_{1}=\sqrt{p_{1}}X,\textrm{}K_{2}=\sqrt{p_{2}}Y,\textrm{}K_{3}=\sqrt{p_{3}}Z,
		\end{equation}
		yielding the output state
		\begin{equation}
		\rho_{out}=p_{0}\rho+p_{1}X\rho_{in}X+p_{2}Y\rho Y+p_{3}Z\rho Z
	\end{equation}
		for $p_{k}\geq0$ with $\sum_{k=0}^{3}p_{k}=1$. Single-qubit channels are practically important since most error models
		in quantum computing assume independent errors across qubits.
		  Pauli channels make particularly clear the interpretation mentioned above of individual Kraus operators as
		describing the different types of errors that can occur on a qubit. 
		 In particular, in a Pauli channel, the different types of errors correspond to the application
		of $X,$$Y,$or $Z$ operators to the qubit. 
		
		Pauli channels specialize to some important subclasses of channels, such as the bit-flip channel and the dephasing channel.  The \textbf{bit-flip channel} applies $X$ errors with some probability $p$, i.e., 
		\begin{equation}
		\rho_{out}=(1-p)\rho_{in}+pX\rho_{in}X,
		\end{equation}
		where we can assume without loss of generality $p\leq0.5$.  (otherwise,
		we can apply an $X$ operator to $\rho_{in}$ to obtain the same channel.) In contrast, \textbf{dephasing channels} apply  $Z$ errors with probability $p\leq0.5$, i.e., 
		\begin{equation}
		\rho_{out}=(1-p)\rho +pZ\rho Z.
		\end{equation}
%		For a single qubit with density 
%		\[
%		\rho_{in}=\left[\begin{array}{cc}
%			\rho_{00} & \rho_{01}\\
%			\rho_{01}^{*} & \rho_{11}
%		\end{array}\right],
%		\]
%		where $\rho_{00},\rho_{11}\geq0$, $\rho_{00}+\rho_{11}=1$, and $\rho_{00}\rho_{11}\geq|\rho_{01}|^{2},$
%		we have 
%		\[
%		\rho_{out}=\left[\begin{array}{cc}
%			\rho_{00} & (1-2p)\rho_{01}\\
%			(1-2p)\rho_{01}^{*} & \rho_{11}
%		\end{array}\right].
%		\]
%		
%		
%		A dephasing channel does not modify classical distributions, but it
%		does affect more general density states.
%		In particular, with $p=0.5$, we obtain the completely dephasing channel,
%		in which $\rho_{out}$ has the same diagonal elements of $\rho_{in}$
%		but zero out-of-diagonal elements.
%%		 If $\rho_{in}$ describes a classical distribution $(p_{0},p_{1})$,
%%		then $\rho_{out}$ is given as
%%		\[
%%		\rho_{out}=\left[\begin{array}{cc}
%%			(1-p)p_{0}+pp_{1} & 0\\
%%			0 & (1-p)p_{1}+pp_{0}
%%		\end{array}\right],
%%		\]
%%		which describes the distribution of a classical bit flip channel with
%%		input distribution $(p_{0},p_{1})$.
	


	


==> Chapter7/Chapter7.tex <==
\chapter{Outlook}

A note of caution
From quantum supremacy to...

==> FnTarticle-nowbook.tex <==
\PassOptionsToClass {book,biber}{nowfnt}
\input {FnTarticle}


==> FnTarticle-nowchapter.tex <==
\PassOptionsToClass {chapter,biber}{nowfnt}
\input {FnTarticle}


==> FnTarticle-nowebook.tex <==
\PassOptionsToClass {ebook,biber}{nowfnt}
\input {FnTarticle}


==> FnTarticle-nowechapter.tex <==
\PassOptionsToClass {echapter,biber}{nowfnt}
\input {FnTarticle}


==> FnTarticle-nowplain.tex <==
\PassOptionsToClass {plain,biber}{nowfnt}
\input {FnTarticle}


==> FnTarticle-nowsample.tex <==
\PassOptionsToClass {sample,biber}{nowfnt}
\input {FnTarticle}


==> FnTmeta-nowbook.tex <==
\PassOptionsToClass {book,biber}{nowfnt}
\input {FnTmeta}


==> FnTmeta-nowchapter.tex <==
\PassOptionsToClass {chapter,biber}{nowfnt}
\input {FnTmeta}


==> FnTmeta-nowebook.tex <==
\PassOptionsToClass {ebook,biber}{nowfnt}
\input {FnTmeta}


==> FnTmeta-nowechapter.tex <==
\PassOptionsToClass {echapter,biber}{nowfnt}
\input {FnTmeta}


==> FnTmeta-nowplain.tex <==
\PassOptionsToClass {plain,biber}{nowfnt}
\input {FnTmeta}


==> FnTmeta-nowsample.tex <==
\PassOptionsToClass {sample,biber}{nowfnt}
\input {FnTmeta}


==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> QuantumFnT-nowbook.tex <==
\PassOptionsToClass {book,biber}{nowfnt}
\input {QuantumFnT}


==> QuantumFnT-nowchapter.tex <==
\PassOptionsToClass {chapter,biber}{nowfnt}
\input {QuantumFnT}


==> QuantumFnT-nowebook.tex <==
\PassOptionsToClass {ebook,biber}{nowfnt}
\input {QuantumFnT}


==> QuantumFnT-nowechapter.tex <==
\PassOptionsToClass {echapter,biber}{nowfnt}
\input {QuantumFnT}


==> QuantumFnT-nowplain.tex <==
\PassOptionsToClass {plain,biber}{nowfnt}
\input {QuantumFnT}


==> QuantumFnT-nowsample.tex <==
\PassOptionsToClass {sample,biber}{nowfnt}
\input {QuantumFnT}


==> SIG-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{SIGcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {SIGcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Signal Processing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SIG}
\journalurl        {http://www.nowpublishers.com/SIG}
\journalissnprint  {1932-8346}
\journalissnonline {1932-8354}
\journaldoi        {10.1561/20}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Adaptive signal processing}
\item{Audio signal processing}
\item{Biological and biomedical signal processing}
\item{Complexity in signal processing}
\item{Digital signal processing}
\item{Distributed and network signal processing}
\item{Image and video processing}
\item{Linear and nonlinear filtering}
\item{Multidimensional signal processing}
\item{Multimodal signal processing}
\item{Multirate signal processing}
\item{Multiresolution signal processing}
\item{Nonlinear signal processing}
\item{Randomized algorithms in signal processing}
\item{Sensor and multiple source signal processing, source separation}
\item{Signal decompositions, subband and transform methods, sparse representations}
\item{Signal processing for communications}
\item{Signal processing for security and forensic analysis, biometric signal processing}
\item{Signal quantization, sampling, analog-to-digital conversion, coding and compression}
\item{Signal reconstruction, digital-to-analog conversion, enhancement, decoding and inverse problems}
\item{Speech/audio/image/video compression}
\item{Speech and spoken language processing}
\item{Statistical/machine learning}
\item{Statistical signal processing}
	\begin{itemize}
	\item{Classification and detection}
	\item{Estimation and regression}
	\item{Tree-structured methods}
	\end{itemize}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ACC-editorialboard.tex <==
%ACC-Editorialboard.

\begin{editorialboard}

%\subsection{Editor-in-Chief}

%\journalchiefeditor{Stefan J. Reichelstein}{Stanford University\\United States}



\subsection{Executive Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Jonathan Glover, Editor-in-Chief}{Columbia University}
\journaleditor{Stephen Penman}{Columbia University}
\journaleditor{Stefan J. Reichelstein}{Stanford University and University of Mannheim}
\journaleditor{Dan Taylor}{University of Pennsylvania}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ACC-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{ACCcolor}{officegreen}   %new color names can be defined before use
\journalcolor      {ACCcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Accounting}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ACC}
\journalurl        {http://www.nowpublishers.com/ACC}
\journalissnprint  {1554-0642}
\journalissnonline {1554-0650}
\journaldoi        {10.1561/14}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Accounting publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Auditing}
\item{Corporate Governance}
\item{Cost Management}
\item{Disclosure}
\item{Event Studies/Market Efficiency Studies}
\item{Executive Compensation}
\item{Financial Reporting}
\item{Management Control}
\item{Performance Measurement}
\item{Taxation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Accounting, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ACC-seriespage.tex <==
\vspace{12pt}
\noindent \textit{IFRS: Markets, Practice, and Politics}\\
Kirstin Becker, Jannis Bischof and Holger Daske\\
ISBN: 978-1-68083-830-5
\\
\\
\noindent \textit{Using Python for Text Analysis in Accounting Research}\\
Vic Anand, Khrystyna Bochkay, Roman Chychyla and Andrew Leone\\
ISBN: 978-1-68083-760-5
\\
\\
\noindent \textit{Research on Corporate Sustainability: Review and Directions for Future Research}\\
Jody Grewal and George Serafeim\\
ISBN: 978-1-68083-718-6
\\
\\
\noindent \textit{Field Experiments in Managerial Accounting Research}\\
Sofia M. Lourenco\\
ISBN: 978-1-68083-628-8

==> journaldata/ACG-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Marc Goergen}{IE Business School\\Spain}
\journalchiefeditor{Geoffrey Wood}{Western University\\Canada}

\subsection{Founding Editor}

\editor{Douglas Cumming}{Florida Atlantic University, USA}

\subsection{Associate Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Renee Adams}{University of Oxford}
\journaleditor{Lucian Bebchuk}{Harvard University}
\journaleditor{William Judge}{Old Dominion University}
\journaleditor{Mark Roe}{Harvard University}
\journaleditor{Rene Stulz}{Ohio State University}
\journaleditor{James Westphal}{University of Michigan}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ACG-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ACGcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ACGcolor} %a color name. 
\journaltitle      {Annals of Corporate Governance}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ACG}
\journalurl        {http://www.nowpublishers.com/ACG}
\journalissnprint  {2381-6724}
\journalissnonline {2381-6732}
\journaldoi        {10.1561/109	}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
Annals of Corporate Governancepublishes
 articles in the following topics:
% \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Boards of Directors}
\item{Ownership}
\item{National Corporate Governance Mechanisms}
\item{Comparative Corporate Governance Systems}
\item{Self Governance}
\item{Teaching Corporate Governance}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
 Annals of Corporate Governance, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ACG-seriespage.tex <==
\vspace{12pt}
\noindent \textit{The Social Purpose of the Modern Business Corporation}\\
Peter J. Buckley
\\ISBN: 978-1-68083-874-9
\\
\noindent \textit{Decentralized Autonomous Organizations: Internal Governance and External Legal Design}\\
Wulf A. Kaal
\\ISBN: 978-1-68083-798-8
\\
\noindent \textit{Decentralized Corporate Governance via Blockchain Technology}\\
Wulf A. Kaal
\\ISBN: 978-1-68083-676-9
\\
\noindent \textit{Corporate Governance in IPO Firms}\\
Erik E. Lehmann and Silvio Vismara
\\ISBN: 978-1-68083-634-9
\\
\noindent \textit{The Political and Governance Risks of Sovereign Wealth}\\
Paul Rose 
\\ISBN: 978-1-68083-624-0



==> journaldata/ASTP-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Audretsch}{Indiana University}
\journaleditor{William Bonvillian}{MIT}
\journaleditor{Barry Bozeman}{Arizona State University}
\journaleditor{Kaye Husbands Fealing}{Georgia Institute of Technology}
\journaleditor{John Hardin}{North Carolina Board of Science and Technology}
\journaleditor{Mariagrazia Squicciarini}{OECD}
\journaleditor{Wolfgang Polt}{Joanneum Research Institute}
\journaleditor{Nicholas Vonortas}{The George Washington University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ASTP-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ASTPcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ASTPcolor} %a color name. 
\journaltitle      {Annals of Science and Technology Policy}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ASTP}
\journalurl        {http://www.nowpublishers.com/ASTP}
\journalissnprint  {2475-1820}
\journalissnonline {2475-1812}
\journaldoi        {10.1561/110}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Annals of Science and Technology Policy publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Literature reviews of technology and innovation policies}
\item{Historical case studies of technology development and implementation}
\item{Institutional histories of technology- and innovation-based organizations}
\item{Analyses of policies attendant to technology development and adoption and diffusion}
\item{Studies documenting the adoption and diffusion of technologies and subsequent consequences}
\item{Studies of public and private research partnerships (cross sectional, over time, or case based)}
\item{Assessments and evaluations of specific technology and innovation policies}
\item{Analyses of ecosystems associated with the technology and/or innovation development}
\item{Cross observational (e.g., cross-agency or cross-country) comparisons of technology and innovation policies}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Annals of Science and Technology Policy, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ASTP-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Case Studies of Successful Technology Transfer from Federal Laboratories}\\
Gretchen B. Jordan, Christopher S. Hayter, Michael Hogan, Manuel A. Gonzalez and Alan C. O’Connor\\
ISBN: 978-1-68083-808-4\\

\noindent \textit{Toward More Effective Science and Technology Advice for Congress: The Historical Roots and Pathways Forward}\\
Peter D. Blair\\
ISBN: 978-1-68083-802-2\\

\noindent \textit{The Globalization of the Bayh–Dole Act}\\
Thorsten Gores and Albert N. Link\\
ISBN: 978-1-68083-754-4\\

\noindent \textit{Globalization and the High-Tech Policy Response}\\
Gregory Tassey\\
ISBN: 978-1-68083-690-5\\
\\
\noindent \textit{Evolution of Ireland’s Industrial, Science and Technology Policy}\\
James A. Cunningham, Patrick Collins and Majella Giblin\\
ISBN: 978-1-68083-680-6\\
\\
\noindent \textit{Public Support of Private Innovation: An Initial Assessment of the North Carolina SBIR/STTR Phase I Matching Funds Program}\\
John W. Hardin, David J. Kaiser and Albert N. Link\\
ISBN: 978-1-68083-674-5

==> journaldata/CGV-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols*}{2}\raggedcolumns
\journalchiefeditor{Aaron Hertzmann }{Adobe Research, USA}
%\end{multicols*}


\subsection{Editors} \scriptsize
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Marc Alexa}{TU Berlin}
\journaleditor{Kavita Bala}{Cornel}
\journaleditor{Ronen Basri}{Weizmann Institute of Science}
\journaleditor{Peter Belhumeur}{Columbia University}
\journaleditor{Andrew Blake}{Microsoft Research}
\journaleditor{Chris Bregler}{Facebook-Oculus}
\journaleditor{Joachim Buhmann}{ETH Zurich}
\journaleditor{Michael Cohen}{Facebook}
\journaleditor{Brian Curless}{University of Washington}
\journaleditor{Paul Debevec}{USC Institute for Creative Technologies}
\journaleditor{Julie Dorsey}{Yale}
\journaleditor{Fredo Durand}{MIT}
\journaleditor{Olivier Faugeras}{INRIA}
\journaleditor{Rob Fergus}{NYU}
%\columnbreak
\journaleditor{William T. Freeman}{MIT}
\journaleditor{Mike Gleicher}{University of Wisconsin}
\journaleditor{Richard Hartley}{Australian National University}
\journaleditor{Hugues Hoppe}{Microsoft Research}
\journaleditor{C. Karen Liu}{Stanford}
\journaleditor{David Lowe}{University of British Columbia}
\journaleditor{Jitendra Malik}{ Berkeley}
\journaleditor{Steve Marschner}{Cornell}
\journaleditor{Shree Nayar}{Columbia}
\journaleditor{Tomas Pajdla}{Czech Technical University}
\journaleditor{Pietro Perona}{California Institute of Technology}
\journaleditor{Marc Pollefeys}{ETH Zurich}
%\columnbreak
\journaleditor{Jean Ponce}{Ecole Normale Superieure}
\journaleditor{Long Quan}{HKUST}
\journaleditor{Cordelia Schmid}{INRIA}
\journaleditor{Steve Seitz}{University of Washington}
\journaleditor{Amnon Shashua}{Hebrew University}
\journaleditor{Peter Shirley}{University of Utah}
\journaleditor{Noah Snavely}{Cornell}
\journaleditor{Stefano Soatto}{UCLA}
\journaleditor{Richard Szeliski}{Microsoft Research}
\journaleditor{Luc Van Gool}{KU Leuven and ETH Zurich}
\journaleditor{Joachim Weickert}{Saarland University}
\journaleditor{Song Chun Zhu}{UCLA}
\journaleditor{Andrew Zisserman}{Oxford}
\end{multicols*}
\end{editorialboard} 

==> journaldata/CGV-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{CGVcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {CGVcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Computer Graphics and Vision}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CGV}
\journalurl        {http://www.nowpublishers.com/CGV}
\journalissnprint  {1572-2740}
\journalissnonline {1572-2759}
\journaldoi        {10.1561/06}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Rendering}
\item{Shape}
\item{Mesh simplification}
\item{Animation}
\item{Sensors and sensing}
\item{Image restoration and enhancement}
\item{Segmentation and grouping}
\item{Feature detection and selection}
\item{Color processing}
\item{Texture analysis and synthesis}
\item{Illumination and reflectance modeling}
\item{Shape representation}
\item{Tracking}
\item{Calibration}
\item{Structure from motion}
\item{Motion estimation and registration}
\item{Stereo matching and reconstruction}
\item{3D reconstruction and image-based modeling}
\item{Learning and statistical methods}
\item{Appearance-based matching}
\item{Object and scene recognition}
\item{Face detection and recognition}
\item{Activity and gesture recognition}
\item{Image and video retrieval}
\item{Video analysis and event recognition}
\item{Medical image analysis}
\item{Robot localization and navigation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/CGV-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Computer Vision for Autonomous Vehicles: Problems, Datasets and State of the Art}\\
Joel Janai, Fatma Güney, Aseem Behl and Andreas Geiger\\
ISBN: 978-1-68083-688-2\\
\\
\noindent \textit{Discrete Graphical Models - An Optimization Perspective}\\
Bogdan Savchynskyy\\
ISBN: 978-1-68083-638-7\\
\\
\noindent \textit{Line Drawings from 3D Models: A Tutorial}\\
Pierre Bénard and Aaron Hertzmann\\
ISBN: 978-1-68083-590-8\\
\\
\noindent \textit{Publishing and Consuming 3D Content on the Web: A Survey}\\
Marco Potenziani, Marco Callieri, Matteo Dellepiane and Roberto Scopigno\\
ISBN: 978-1-68083-536-6\\
\\
\noindent \textit{Crowdsourcing in Computer Vision}\\
Adriana Kovashka, Olga Russakovsky, Li Fei-Fei and Kristen Grauman\\
ISBN: 978-1-68083-212-9\\
\\
\noindent \textit{The Path to Path-Traced Movies}\\
Per H. Christensen and Wojciech Jarosz\\
ISBN: 978-1-68083-210-5\\
\\
\noindent \textit{(Hyper)-Graphs Inference through Convex Relaxations and Move Making Algorithms}\\
Nikos Komodakis, M. Pawan Kumar and Nikos Paragios\\
ISBN: 978-1-68083-138-2\\


==> journaldata/CIT-editorialboard.tex <==
\begin{editorialboard}

%\subsection{Editor-in-Chief}

\journalchiefeditor{Alexander Barg}{University of Maryland\\USA}

\subsection{Area Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Emmanuel Abbe}{Princeton University}
\journaleditor{Arya Mazumdar}{UMass Amherst}
\journaleditor{Olgica Milenkovic}{University of Illinois, Urbana-Champaign}
\journaleditor{Anelia Somekh-Baruch}{Bar-Ilan University}
\journaleditor{Himanshu Tyagi}{Indian Institute of Science}

\subsection{Editors} %\scriptsize
%\begin{multicols*}{3}\raggedcolumns
\journaleditor{Venkat Anantharam}{UC Berkeley}
\journaleditor{Giuseppe Caire}{TU Berlin}
\journaleditor{Daniel Costello}{University of Notre Dame}
%\journaleditor{Anthony Ephremides}{University of Maryland}
%\journaleditor{Andrea Goldsmith}{Stanford University}
\journaleditor{Albert Guillen i Fabregas}{Pompeu Fabra University}
\journaleditor{Dongning Guo}{Northwestern University}
\journaleditor{Dave Forney}{MIT}
\journaleditor{Te Sun Han}{University of Tokyo}
\journaleditor{Babak Hassibi}{Caltech}
\journaleditor{Michael Honig}{Northwestern University}
%\journaleditor{Tara Javidi}{UC San Diego}

\journaleditor{Ioannis Kontoyiannis}{Cambridge University}
\journaleditor{Gerhard Kramer}{TU Munich}
\journaleditor{Amos Lapidoth}{ETH Zurich}
\journaleditor{Muriel Medard}{MIT}
\journaleditor{Neri Merhav}{Technion}
\journaleditor{David Neuhoff}{University of Michigan}
\journaleditor{Alon Orlitsky}{UC San Diego}
\journaleditor{Yury Polyanskiy}{MIT}
\journaleditor{Vincent Poor}{Princeton University}
%\journaleditor{Maxim Raginsky}{UIUC}
\journaleditor{Kannan Ramchandran}{UC Berkeley}
\journaleditor{Igal Sason}{Technion}
%\columnbreak
\journaleditor{Shlomo Shamai}{Technion}
\journaleditor{Amin Shokrollahi}{EPF Lausanne}
\journaleditor{Yossef Steinberg}{Technion}
\journaleditor{Wojciech Szpankowski}{Purdue University}
\journaleditor{David Tse}{Stanford University}
\journaleditor{Antonia Tulino}{Bell Labs}
\journaleditor{R\"{u}diger Urbanke}{EPF Lausanne}
\journaleditor{Emanuele Viterbo}{Monash University}
\journaleditor{Frans Willems}{TU Eindhoven}
\journaleditor{Raymond Yeung}{CUHK}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> journaldata/CIT-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{CITcolor}{officegreen}   %new color names can be defined before use
\journalcolor      {CITcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Communications and Information Theory}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CIT}
\journalurl        {http://www.nowpublishers.com/CIT}
\journalissnprint  {1567-2190}
\journalissnonline {1567-2328 }
\journaldoi        {10.1561/01}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Communications and Information Theory publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Coded modulation}
\item{Coding theory and practice}
\item{Communication complexity}
\item{Communication system design}
\item{Cryptology and data security}
\item{Data compression}
\item{Data networks}
\item{Demodulation and Equalization}
\item{Denoising}
\item{Detection and estimation}
\item{Information theory and statistics}
\item{Information theory and computer science}
\item{Joint source/channel coding}
\item{Modulation and signal design}
\item{Multiuser detection}
\item{Multiuser information theory}
\item{Optical communication channels}
\item{Pattern recognition and learning}
\item{Quantization}
\item{Quantum information processing}
\item{Rate-distortion theory}
\item{Shannon theory}
\item{Signal processing for communications}
\item{Source coding}
\item{Storage and recording codes}
\item{Speech and Image Compression}
\item{Wireless Communications}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Communications and Information Theory, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/CIT-seriespage.tex <==
\vspace{12pt}
\\
\noindent \textit{An Algebraic and Probabilistic Framework for Network Information Theory}\\
S. Sandeep Pradhan, Arun Padakandla and Farhad Shirani\\
ISBN: 978-1-68083-766-7\\
\\
\noindent \textit{Theoretical Foundations of Adversarial Binary Detection}\\
Mauro Barni and Benedetta Tondi\\
ISBN: 978-1-68083-764-3\\
\\
\noindent \textit{Polynomial Methods in Statistical Inference}\\
Yihong Wu and Pengkun Yang\\
ISBN: 978-1-68083-730-8\\
\\
\noindent \textit{Information-Theoretic Foundations of Mismatched Decoding}\\
Jonathan Scarlett, Albert Guillen i Fabregas, Anelia Somekh-Baruch and Alfonso Martinez\\
ISBN: 978-1-68083-712-4\\
\\
\noindent \textit{Coded Computing: Mitigating Fundamental Bottlenecks in Large-Scale Distributed Computing and Machine Learning}\\
Songze Li and Salman Avestimehr \\
ISBN: 978-1-68083-704-9



==> journaldata/DBS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Joseph M. Hellerstein}{University of California at Berkeley\\United States}
\journalchiefeditor{Surajit Chaudhuri}{Microsoft Research, Redmond\\United States}



\subsection{Editors} %\scriptsize
%\begin{multicols*}{3}\raggedcolumns
\journaleditor{Azza Abouzied}{NYU-Abu Dhabi}
\journaleditor{Gustavo Alonso}{ETH Zurich}
\journaleditor{Mike Cafarella}{University of Michigan}
\journaleditor{Alan Fekete}{University of Sydney}
\journaleditor{Ihab Ilyas}{University of Waterloo}
\journaleditor{Andy Pavlo}{Carnegie Mellon University}
\journaleditor{Sunita Sarawagi}{IIT Bombay}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/DBS-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{DBScolor}{officegreen}   %new color names can be defined before use
\journalcolor      {DBScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Databases}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {DBS}
\journalurl        {http://www.nowpublishers.com/DBS}
\journalissnprint  {1931-7883}
\journalissnonline {1931-7891}
\journaldoi        {10.1561/19}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Databases publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Data Models and Query Languages}
    \item{Query Processing and Optimization}
    \item{Storage, Access Methods, and Indexing}
    \item{Transaction Management, Concurrency Control and Recovery}
    \item{Deductive Databases}
    \item{Parallel and Distributed Database Systems}
    \item{Database Design and Tuning}
    \item{Metadata Management}
    \item{Object Management}
    \item{Trigger Processing and Active Databases}
    \item{Data Mining and OLAP}
    \item{Approximate and Interactive Query Processing}
    \item{Data Warehousing}
    \item{Adaptive Query Processing}
    \item{Data Stream Management}
    \item{Search and Query Integration}
    \item{XML and Semi-Structured Data}
    \item{Web Services and Middleware}
    \item{Data Integration and Exchange}
    \item{Private and Secure Data Management}
    \item{Peer-to-Peer, Sensornet and Mobile Data Management}
    \item{Scientific and Spatial Data Management}
    \item{Data Brokering and Publish/Subscribe}
    \item{Data Cleaning and Information Extraction}
    \item{Probabilistic Data Management}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Databases, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/DBS-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Differential Privacy for Databases}\\
Joseph P. Near and Xi He\\
ISBN: 978-1-68083-850-3\\
\\
\noindent \textit{Database Systems on GPUs}\\
Johns Paul, Shengliang Lu and Bingsheng He\\
ISBN: 978-1-68083-848-0\\
\\
\noindent \textit{Machine Knowledge: Creation and Curation of Comprehensive Knowledge Bases}\\
Gerhard Weikum, Xin Luna Dong, Simon Razniewski and Fabian Suchanek\\
ISBN: 978-1-68083-836-7\\
\\
\noindent \textit{Cloud Data Services: Workloads, Architectures and Multi-Tenancy}\\
Vivek Narasayya and Surajit Chaudhuri\\
ISBN: 978-1-68083-774-2\\
\\
\noindent \textit{Data Provenance}\\
Boris Glavic\\
ISBN: 978-1-68083-828-2\\
\\
\noindent \textit{FPGA-Accelerated Analytics: From Single Nodes to Clusters}\\
Zsolt Istv\'an, Kaan Kara and David Sidler\\
ISBN: 978-1-68083-734-6\\
\\
\noindent \textit{Distributed Learning Systems with First-Order Methods}\\
Ji Liu and Ce Zhango\\
ISBN: 978-1-68083-700-1\\

==> journaldata/ECO-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{William H. Greene}{New York University\\United States}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Manuel Arellano}{CEMFI Spain}
\journaleditor{Wiji Arulampalam}{University of Warwick}
\journaleditor{Orley Ashenfelter}{Princeton University}
\journaleditor{Jushan Bai}{Columbia University}
\journaleditor{Badi Baltagi}{Syracuse University}
\journaleditor{Anil Bera}{University of Illinois}
\journaleditor{Tim Bollerslev}{Duke University}
\journaleditor{David Brownstone}{UC Irvine}
\journaleditor{Xiaohong Chen}{Yale University}
\journaleditor{Steven Durlauf}{University of Chicago}
\journaleditor{Amos Golan}{American University}
\journaleditor{Bill Griffiths}{University of Melbourne}
\journaleditor{James Heckman}{University of Chicago}
\journaleditor{Jan Kiviet}{University of Amsterdam}
\journaleditor{Gary Koop}{The University of Strathclyde}
\journaleditor{Michael Lechner}{University of St. Gallen}
\journaleditor{Lung-Fei Lee}{Ohio State University}
\journaleditor{Larry Marsh}{Notre Dame University}
\journaleditor{James MacKinnon}{Queens University}
\journaleditor{Bruce McCullough}{Drexel University}
\journaleditor{Jeff Simonoff}{New York University}
\journaleditor{Joseph Terza}{Purdue University}
\journaleditor{Ken Train}{UC Berkeley}
\journaleditor{Pravin Trivedi}{Indiana University}
\journaleditor{Adonis Yatchew}{University of Toronto}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ECO-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{ECOcolor}{brickred}   %new color names can be defined before use
\journalcolor      {ECOcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Econometrics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ECO}
\journalurl        {http://www.nowpublishers.com/ECO}
\journalissnprint  {1551-3076}
\journalissnonline {1551-3084}
\journaldoi        {10.1561/08}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Econometrics publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Econometric Models}
    \item{Simultaneous Equation Models}
    \item{Estimation Frameworks}
    \item{Biased Estimation}
    \item{Computational Problems}
    \item{Microeconometrics}
    \item{Treatment Modeling}
    \item{Discrete Choice Modeling}
    \item{Models for Count Data}
    \item{Duration Models}
   \item{Limited Dependent Variables}
    \item{Panel Data}
    \item{Time Series Analysis}
    \item{Latent Variable Models}
    \item{Qualitative Response Models}
    \item{Hypothesis Testing}
    \item{Econometric Theory}
    \item{Financial Econometrics}
    \item{Measurement Error in Survey Data}
    \item{Productivity Measurement and Analysis}
    \item{Semiparametric and Nonparametric Estimation}
    \item{Bootstrap Methods}
    \item{Nonstationary Time Series}
    \item{Robust Estimation}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Econometrics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ECO-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Climate Econometrics: An Overview}\\
Jennifer L. Castle and David F. Hendry\\
ISBN: 978-1-68083-708-7\\
\\
\noindent \textit{Foundations of Stated Preference Elicitation: Consumer Behavior\\ and Choice-based Conjoint Analysis}\\
Moshe Ben-Akiva, Daniel McFadden and Kenneth Train\\
ISBN: 978-1-68083-526-7\\
\\
\noindent \textit{Structural Econometrics of Auctions: A Review}\\
Matthew L. Gentry, Timothy P. Hubbard, Denis Nekipelov and\\ Harry J. Paarsch\\
ISBN: 978-1-68083-446-8\\
\\
\noindent \textit{Data Visualization and Health Econometrics}\\
Andrew M. Jones\\
ISBN: 978-1-68083-318-8\\


==> journaldata/EDA-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Radu Marculescu}{Carnegie Mellon University}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Robert K. Brayton}{University of California, Berkeley}
\journaleditor{Raul Camposano}{Sage Design Atomation}
\journaleditor{K.T. Tim Cheng}{HKUST}
\journaleditor{Jason Cong}{University of California, Los Angeles}
\journaleditor{Masahiro Fujita}{University of Tokyo}
\journaleditor{Georges Gielen}{KU Leuven}
\journaleditor{Tom Henzinger}{IST Austria}
\journaleditor{Andrew Kahng}{University of California, San Diego}
\columnbreak
\journaleditor{Andreas Kuehlmann}{Synopsys}
\journaleditor{Sharad Malik}{Princeton University}
\journaleditor{Joel Phillips}{Cadence Berkeley Labs}
\journaleditor{Jonathan Rose}{University of Toronto}
\journaleditor{Rob Rutenbar}{University of Pittsburgh}
\journaleditor{Alberto Sangiovanni-Vincentelli}{University of California, Berkeley}
\journaleditor{Leon Stok}{IBM Research}
\end{multicols*}
\end{editorialboard} 

==> journaldata/EDA-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{EDAcolor}{brickred}   %new color names can be defined before use
\journalcolor      {EDAcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Electronic Design Automation}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {EDA}
\journalurl        {http://www.nowpublishers.com/EDA}
\journalissnprint  {1551-3939}
\journalissnonline {1551-3947}
\journaldoi        {10.1561/10}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Electronic Design Automation publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{System Level Design}
    \item{Behavioral Synthesis}
    \item{Logic Design}
    \item{Verification}
    \item{Test}
    \item{Physical Design}
    \item{Circuit Level Design}
    \item{Reconfigurable Systems}
    \item{Analog Design}
    \item{Embedded software and parallel programming}
   \item{Multicore, GPU, FPGA, and heterogeneous systems}
    \item{Distributed, networked embedded systems}
    \item{Real-time and cyberphysical systems}
\end{itemize}
% \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Electronic Design Automation, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/EDA-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Smart Healthcare}\\
Hongxu Yin, Ayten Ozge Akmandor, Arsalan Mosenia and Niraj K. Jha\\
ISBN: 978-1-68083-440-6\\
\\
\noindent \textit{Contracts for System Design}\\
Albert Benveniste, Benoit Caillaud, Dejan Nickovic, Roberto Passerone, Jean-Baptiste Raclet, Philipp Reinkemeier, Alberto Sangiovanni-Vincentelli, Werner Damm, Thomas A. Henzinger and Kim G. Larsen\\
ISBN: 978-1-68083-402-4\\
\\
\noindent \textit{Non-Boolean Computing with Spintronic Devices}\\
Kawsher A. Roxy and Sanjukta Bhanja\\
ISBN: 978-1-68083-362-1

==> journaldata/EES-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Marija D. Ili\'c}{MIT and Carnegie Mellon University\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Hill}{University of Hong Kong and University of Sydney}
\journaleditor{Daniel Kirschen}{University of Washington}
\journaleditor{J. Zico Kolter}{Carnegie Mellon University}
\journaleditor{Chao Lu}{Tsinghua University}
\journaleditor{Steven Low}{California Institute of Technology}
\journaleditor{Ram Rajagopa}{Stanford University}
\journaleditor{Lou van der Sluis}{TU Delft}
\journaleditor{Goran Strbac}{Imperial College London}
\journaleditor{Robert J. Thomas}{Cornell University}
\journaleditor{David Tse}{University of California, Berkeley}
\journaleditor{Le Xie}{Texas A\&M University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/EES-journaldata.tex <==
\definecolor{cinnabar}{rgb}{0.89, 0.26, 0.2}
\colorlet{EEScolor}{cinnabar}   %new color names can be defined before use
\journalcolor      {EEScolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Electric Energy Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {EES}
\journalurl        {http://www.nowpublishers.com/EES}
\journalissnprint  {2332-6557}
\journalissnonline {2332-6565}
\journaldoi        {10.1561/31}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Electric Energy Systems publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Advances in power dispatch}
\item{Demand-side and grid scale data analytics}
\item{Design and optimization of electric services}
\item{Distributed control and optimization of distribution networks}
\item{Distributed sensing for the grid}
\item{Distribution systems}
\item{Fault location and service restoration}
\item{Integration of physics-based and data-driven modeling of future electric energy systems}
\item{Integration of Power electronics, Networked FACTS}
\item{Integration of renewable energy sources}
\item{Interdependence of power system operations and planning and the electricity markets}
\item{Microgrids}
\item{Modern grid architecture}
\item{Power system analysis and computing}
\item{Power system dynamics}
\item{Power system operation}
\item{Power system planning}
\item{Power system reliability}
\item{Power system transients}
\item{Security and privacy}
\item{Stability and control for the whole multi-layer (granulated) network with new load models (to include storage, DR, EVs) and new generation}
\item{System protection and control}
\item{The new stability guidelines and control structures for supporting high penetration of renewables (>50\%)}
\item{Uncertainty quantification for the grid}
\item{System impacts of HVDC}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Electric Energy Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/EES-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Network-Based Analysis of Rotor Angle Stability of Power Systems}\\
Yue Song, David J. Hill and Tao Liu\\
ISBN: 978-1-68083-778-0\\
\\
\noindent \textit{A Survey of Relaxations and Approximations of the Power Flow Equations}\\
Daniel K. Molzahn and Ian A. Hiskens\\
ISBN: 978-1-68083-540-3\\
\\
\noindent \textit{HELM: The Holomorphic Embedding Load-Flow Method. Foundations and Implementations}\\
Antonio Trias\\
ISBN: 978-1-68083-516-8\\
\\
\noindent \textit{Combinatorial Optimization of Alternating Current Electric Power Systems}\\
Sid Chi-Kin Chau\\
ISBN: 978-1-68083-514-4

==> journaldata/ENT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{1}
\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}
\journalchiefeditor{David B. Audretsch}{Indiana University\\United States}\\
\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Howard Aldrich}{University of North Carolina}
\journaleditor{Sharon Alvarez}{University of Denver}
\journaleditor{Per Davidsson}{Queensland University of Technology}
\journaleditor{Michael Frese}{National University of Singapore}
\journaleditor{William B. Gartner}{Copenhagen Business School}
\journaleditor{Magnus Henrekson}{IFN Stockholm}
\journaleditor{Michael A. Hitt}{Texas A\&M University}
\journaleditor{Joshua Lerner}{Harvard University}
\columnbreak
\journaleditor{Jeff McMullen}{Indiana University}
\journaleditor{P.R. Kumar}{Texas A\&M University}
\journaleditor{Maria Minniti}{Syracuse University}
\journaleditor{Simon Parker}{University of Western Ontario}
\journaleditor{Holger Patzelt}{TU Munich}
\journaleditor{Saras Sarasvathy}{University of Virginia}
\journaleditor{Roy Thurik}{Erasmus University}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ENT-journaldata.tex <==
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\colorlet{ENTcolor}{Cerulean}   %new color names can be defined before use
\journalcolor      {ENTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Entrepreneurship}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ENT}
\journalurl        {http://www.nowpublishers.com/ENT}
\journalissnprint  {1551-3114}
\journalissnonline {1551-3122}
\journaldoi        {10.1561/03}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Entrepreneurship publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Nascent and start-up entrepreneurs}
\item{Opportunity recognition}
\item{New venture creation process}
\item{Business formation}
\item{Firm ownership}
\item{Market value and firm growth}
\item{Franchising}
\item{Managerial characteristics and behavior of entrepreneurs}
\item{Strategic alliances and networks}
\item{Government programs and public policy}
\item{Gender and ethnicity}
\columnbreak
\item{New business financing:}
	\begin{itemize}
\item{Business angels}
\item{Bank financing, debt, and trade credit}
\item{Venture capital and private equity capital}
\item{Public equity and IPOs} 
\end{itemize}
\item{Family-owned firms}
\item{Management structure, governance and performance}
\item{Corporate entrepreneurship}
\item{High technology:}
	\begin{itemize}
        \item{Technology-based new firms}
        \item{High-tech clusters}
        \end{itemize}
\item{Small business and economic growth}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Entrepreneurship, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ENT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Ambidexterity and Entrepreneurship Studies: A Literature Review and Research Agenda}\\
Maribel Guerrero\\
ISBN: 978-1-68083-818-3\\
\\
\noindent \textit{Innovative Entrepreneurship as a Collaborative Effort: An Institutional Framework}\\
Niklas Elert and Magnus Henrekson\\
ISBN: 978-1-68083-810-7\\
\\
\noindent \textit{Entrepreneurial Finance: Emerging Approaches Using Machine Learning and Big Data}\\
Francesco Ferrati and Moreno Muffatto\\
ISBN: 978-1-68083-804-6\\
\\
\noindent \textit{Advice to Entrepreneurs and Small Business}\\
Kevin Mole\\
ISBN: 978-1-68083-758-2
\\
\noindent \textit{From Ethnic Enclaves to Transnational Landscapes: A Review of Immigrant Entrepreneurship Research}\\
Anuradha Basu and Sarika Pruthi\\
ISBN: 978-1-68083-756-8


==> journaldata/FIN-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\begin{multicols}{1}
\journalchiefeditor{Sheridan Titman}{University of Texas at Austin\\United States}
\end{multicols}

\subsection{Associate Editors}
\begin{multicols}{1}
\journaleditor{Josef Zechner}{WU Vienna University of Economics and Finance}
\journaleditor{Chester Spatt}{Carnegie Mellon University}
\end{multicols}
\end{editorialboard} 

==> journaldata/FIN-journaldata.tex <==
\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
\colorlet{FINcolor}{ceruleanblue}   %new color names can be defined before use
\journalcolor      {FINcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Finance}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {FIN}
\journalurl        {http://www.nowpublishers.com/FIN}
\journalissnprint  {1567-2395}
\journalissnonline {1567-2409}
\journaldoi        {10.1561/05}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Finance publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Corporate Finance}
\begin{itemize}
\item{Corporate Governance}
\item{Corporate Financing}
\item{Dividend Policy and Capital Structure}
\item{Corporate Control}
\item{Investment Policy}
\item{Agency Theory and Information}
\end{itemize}
\end{itemize}
\columnbreak
\begin{itemize}
\item{Financial Markets}
\begin{itemize}
\item{Market Microstructure}
\item{Portfolio Theory}
\item{Financial Intermediation}
\item{Investment Banking}
\item{Market Efficiency}
\item{Security Issuance}
\item{Anomalies and Behavioral Finance}
\end{itemize}
\end{itemize}
\end{multicols}
%}
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
%\columnbreak
%\begin{itemize}
\item{Asset Pricing}
\begin{itemize}
\item{Asset-Pricing Theory}
\item{Asset-Pricing Models}
\item{Tax Effects}
\item{Liquidity} 
\item{Equity Risk Premium} 
\item{Pricing Models and Volatility} 
\item{Fixed Income Securities} 
\end{itemize}
\end{itemize}
\columnbreak
\begin{itemize}
\item{Derivatives}
\begin{itemize}
\item{Computational Finance}
\item{Futures Markets and Hedging}
\item{Financial Engineering}
\item{Interest Rate Derivatives}
\item{Credit Derivatives}
\item{Financial Econometrics}
\item{Estimating Volatilities and Correlations}
\end{itemize}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Finance, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/FIN-seriespage.tex <==
\vspace{12pt}

\noindent \textit{The Implications of Heterogeneity and Inequality for Asset Pricing}\\
Stavros Panageas\\
ISBN: 978-1-68083-750-6\\
\\
\noindent \textit{Risk Sharing Within the Firm: A Primer}\\
Marco Pagano\\
ISBN: 978-1-68083-740-7\\
\\
\noindent \textit{The Economics of Credit Rating Agencies}\\
Francesco Sangiorgi and Chester Spatt\\
ISBN: 978-1-68083-380-5\\
\\
\noindent \textit{Initial Public Offerings: A Synthesis of the Literature and Directions for Future Research}\\
Michelle Lowry, Roni Michaely and Ekaterina Volkova\\
ISBN: 978-1-68083-340-9\\
\\
\noindent \textit{Privatization, State Capitalism, and State Ownership of Business in the 21st Century}\\
William L. Megginson\\
ISBN: 978-1-68083-338-6\\

==> journaldata/HCI-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Youn-Kyung Lim}{Korea Advanced Institute of Science and Technology}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Ben Bederson}{University of Maryland}
\journaleditor{Madeline Balaam}{KTH Royal Institute of Technology}
\journaleditor{Eun Kyoung Choe}{University of Maryland, College Park}
\journaleditor{Andy Cockburn}{University of Canterbury}
\journaleditor{Karrie Karahalios}{University of Illinois at Urbana-Champaign}
\journaleditor{Rohit Ashok Khot}{HAFP Research Lab, RMIT University}
\journaleditor{Uichin Lee}{Korea Advanced Institute of Science and Technology}
\journaleditor{Florian Mueller}{Exertion Games Lab, RMIT University}
\journaleditor{Bilge Mutlu}{University of Wisconsin-Madison}
\journaleditor{Marianna Obrist}{University of Sussex}
\journaleditor{Nuria Oliver}{Telefonica}
\journaleditor{Sameer Patil}{University of Utah}
\journaleditor{Orit Shaer}{Wellesley College}
\journaleditor{Desney S. Tan}{Microsoft Research}
\journaleditor{Koji Yatani}{University of Tokyo}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/HCI-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{HCIcolor}{pinegreen}   %new color names can be defined before use
\journalcolor      {HCIcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Human-Computer Interaction}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {HCI}
\journalurl        {http://www.nowpublishers.com/HCI}
\journalissnprint  {1551-3955}
\journalissnonline {1551-3963}
\journaldoi        {10.1561/11}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Human-Computer Interaction publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{History of the research community}
\item{Theory}
\item{Technology}
\item{Computer Supported Cooperative Work}
\item{Interdisciplinary influence}
\item{Advanced topics and trends}
\end{itemize}
%\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Human-Computer Interaction, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/HCI-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Improving HCI with Brain Input: Review, Trends, and Outlook}\\
Erin T. Solovey and Felix Putzer\\
ISBN: 978-1-68083-814-5\\
\\
\noindent \textit{Patient-Generated Health Data: Dimensions, Challenges, and Open Questions}\\
Mayara Costa Figueiredo and Yunan Cheng\\
ISBN: 978-1-68083-668-4\\
\\
\noindent \textit{Patterns and Themes in Designing with Children}\\
Jessica Korte\\
ISBN: 978-1-68083-660-8\\
\\
\noindent \textit{Gender-Inclusive HCI Research and Design: A Conceptual Review}\\
Simone Stumpf, Anicia Peters, Shaowen Bardzell, Margaret Burnett, Daniela Busse, Jessica Cauchard, Elizabeth Churchill\\
ISBN: 978-1-68083-656-1\\


==> journaldata/ICS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols*}{2}\raggedcolumns
\journalchiefeditor{Georges Gielen}{KU Leuven, Belgium}
%\end{multicols*}

\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Alison Burdett}{Sensium Healthcare, UK}
\journaleditor{Malgorzata Chrzanowska-Jeske}{Portland State University, USA}
\journaleditor{Paulo Diniz}{UFRJ, Brazil}
\journaleditor{Peter Kennedy}{University College Dublin, Ireland}
\journaleditor{Maciej Ogorzalek}{Jagiellonian University, Poland}
\journaleditor{Jan van der Spiegel}{University of Pennsylvania, USA}
\journaleditor{Ljiljana Trajkovic}{Simon Fraser University, USA}
%\end{multicols*}

\end{editorialboard} 

==> journaldata/ICS-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{ICScolor}{brickred}   %new color names can be defined before use
\journalcolor      {ICScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Integrated Circuits and Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ICS}
\journalurl        {http://www.nowpublishers.com/ICS}
\journalissnprint  {2693-9347}
\journalissnonline {2693-9355}
\journaldoi        {10.1561/35}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
 Integrated Circuits and Systems
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Analog, digital and mixed-signal circuits and systems}
\item{RF and mm-wave integrated circuits and systems}
\item{Wireless and wireline communication circuits and systems}
\item{Data converters and frequency generation}
\item{Power electronics and power management circuits}
\item{Biomedical circuits and systems}
\item{Sensor and imager circuits and cyber physical systems}
\item{Security and resilient circuits and systems}
\item{Circuits and systems in emerging non-CMOS technologies}
\item{Circuit theory, modeling, analysis and design methods}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Integrated Circuits and Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ICS-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Welcome to the World of Single-Slope Column-Level Analog-to-Digital Converters for CMOS Image Sensors}\\
Albert Theuwissen and Guy Meynants\\
ISBN: 978-1-68083-812-1\\





==> journaldata/INR-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Maarten de Rijke}{University of Amsterdam \\ and Ahold Delhaize\\The Netherlands}
\journalchiefeditor{Yiqun Liu}{Tsinghua University\\China}
\journalchiefeditor{Diane Kelly}{University of Tennessee\\USA}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Barbara Poblete}{University of Chile}
\journaleditor{Claudia Hauff}{Delft University of Technology}
\journaleditor{Doug Oard}{University of Maryland}
\journaleditor{Ellen M. Voorhees}{National Institute of Standards and Technology}
\journaleditor{Fabrizio Sebastiani}{Consiglio Nazionale delle Ricerche, Italy}
\journaleditor{Hang Li}{Bytedance Technology}
\journaleditor{Isabelle Moulinier}{Capital One}
\journaleditor{Jaap Kamps}{University of Amsterdam}
\journaleditor{Jimmy Lin}{University of Waterloo}
\journaleditor{Leif Azzopardi}{University of Glasgow}
\columnbreak
\journaleditor{Lynda Tamine}{University of Toulouse}
\journaleditor{Mark Sanderson}{RMIT University}
\journaleditor{Rodrygo Luis Teodoro Santos}{Universidade Federal de Minas Gerais}
\journaleditor{Ruihua Song}{Renmin University of China}
\journaleditor{Ryen White}{Microsoft Research}
\journaleditor{Shane Culpepper}{RMIT}
\journaleditor{Soumen Chakrabarti}{Indian Institute of Technology}
\journaleditor{Xuanjing Huang}{Fudan University}
\journaleditor{Zi Helen Huang}{University of Queensland}
\end{multicols*}
\end{editorialboard} 

==> journaldata/INR-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{INRcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {INRcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Information Retrieval}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {INR}
\journalurl        {http://www.nowpublishers.com/INR}
\journalissnprint  {1554-0669}
\journalissnonline {1554-0677}
\journaldoi        {10.1561/15}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Information Retrieval publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Applications of IR}
\item{Architectures for IR}
\item{Collaborative filtering and recommender systems}
\item{Cross-lingual and multilingual IR}
\item{Distributed IR and federated search}
\item{Evaluation issues and test collections for IR}
\item{Formal models and language models for IR}
\item{IR on mobile platforms}
\item{Indexing and retrieval of structured documents}
\item{Information categorization and clustering}
\item{Information extraction}
\item{Information filtering and routing}
\item{Metasearch, rank aggregation and data fusion}
\item{Natural language processing for IR}
\item{Performance issues for IR systems, including algorithms, data structures, optimization techniques, and scalability}
\item{Question answering}
\item{Summarization of single documents, multiple documents, and corpora}
\item{Text mining}
\item{Topic detection and tracking}
\item{Usability, interactivity, and visualization issues in IR}
\item{User modelling and user studies for IR}
\item{Web search}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Information Retrieval, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 5 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/INR-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Search and Discovery in Personal Email Collections}\\
Michael Bendersky, Xuanhui Wang, Marc Najork and Donald Metzler\\
ISBN: 978-1-68083-838-1\\

\noindent \textit{Extracting, Mining and Predicting Users’ Interests from Social Media}\\
Fattane Zarrinkalam, Stefano Faralli, Guangyuan Piao and Ebrahim Bagheri\\
ISBN: 978-1-68083-738-4\\

\noindent \textit{Knowledge Graphs: An Information Retrieval Perspective}\\
Ridho Reinanda, Edgar Meij and Maarten de Rijke\\
ISBN: 978-1-68083-728-5\\

\noindent \textit{Deep Learning for Matching in Search and Recommendation}\\
Jun Xu, Xiangnan He and Hang Li \\
ISBN: 978-1-68083-706-3\\

\noindent \textit{Explainable Recommendation: A Survey and New Perspectives}\\
Yongfeng Zhang and Xu Chen\\
ISBN: 978-1-68083-658-5\\



==> journaldata/ISY-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols}{1}
\journalchiefeditor{David Paradice}{Auburn University\\United States}
%\end{multicols}

\subsection{Honorary Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Izak Benbasat}{University of British Columbia}
\journaleditor{Alan R. Dennis}{Kelley School of Business, Indiana University}
\journaleditor{Jacqueline Rees Ulmer}{Iowa State University}
\journaleditor{Veda Storey}{Georgia State University}
\journaleditor{Detmar Straub}{Georgia State University}
\journaleditor{Hugh Watson}{University of Georgia}
%\end{multicols*}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Joey George}{Iowa State University}
\journaleditor{Alan Hevner}{University of South Florida}
\journaleditor{Carol Saunders}{University of Central Florida}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ISY-journaldata.tex <==
\definecolor{regalia}{rgb}{0.32, 0.18, 0.5}
\colorlet{ISYcolor}{regalia}   %new color names can be defined before use
\journalcolor      {ISYcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Information Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ISY}
\journalurl        {http://www.nowpublishers.com/ISY}
\journalissnprint  {2331-1231}
\journalissnonline {2331-124X}
\journaldoi        {10.1561/29}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Information Systems publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{IS and Individuals}
\item{IS and Groups}
\item{IS and Organizations}
\item{IS and Industries}
\item{IS and Society}
\item{IS Development}
\item{IS Economics}
\item{IS Management}
\item{IS Research Methods}
\end{itemize}
% \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Information Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ISY-seriespage.tex <==
\vspace{12pt}
\noindent \textit{IT Project Management: Lessons Learned from Project Retrospectives 1999–2020}\\
R. Ryan Nelson\\
ISBN: 978-1-68083-776-6\\
\\
\noindent \textit{Speech Analytics for Actionable Insights: Current Status, Recommendation, and Guidance}\\
J. P. Shim, Aaron M. French and Bikesh Upreti\\
ISBN: 978-1-68083-696-7\\
\\
\noindent \textit{A Review of Personality in Human–Robot Interactions}\\
Lionel P. Robert Jr., Rasha Alahmad, Connor Esterwood, Sangmi Kim, Sangseok You and Qiaoning Zhang\\
ISBN: 978-1-68083-662-2\\
\\
\noindent \textit{Information Technology and Entrepreneurship: Factors that Shape Investment Support for Innovation}\\
Veda C. Storey and Linda Wallace\\
ISBN: 978-1-68083-602-8


==> journaldata/MAL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Michael Jordan}{University of California, Berkeley\\United States}



\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Peter Bartlett}{UC Berkeley}
\journaleditor{Yoshua Bengio}{Universit{\'e} de Montr{\'e}al}
\journaleditor{Avrim Blum}{Toyota Technological Institute}
\journaleditor{Craig Boutilier}{University of Toronto}
\journaleditor{Stephen Boyd}{Stanford University}
\journaleditor{Carla Brodley}{Northeastern University}
\journaleditor{Inderjit Dhillon}{Texas at Austin}
\journaleditor{Jerome Friedman}{Stanford University}
\journaleditor{Kenji Fukumizu}{ISM}
\journaleditor{Zoubin Ghahramani}{Cambridge University}
\journaleditor{David Heckerman}{Amazon}
\journaleditor{Tom Heskes}{Radboud University}
\journaleditor{Geoffrey Hinton}{University of Toronto}
\journaleditor{Aapo Hyvarinen}{Helsinki IIT}
\journaleditor{Leslie Pack Kaelbling}{MIT}
\journaleditor{Michael Kearns}{UPenn}
\journaleditor{Daphne Koller}{Stanford University}
\journaleditor{John Lafferty}{Yale}
\journaleditor{Michael Littman}{Brown University}
\journaleditor{Gabor Lugosi}{Pompeu Fabra}
\journaleditor{David Madigan}{Columbia University}
\journaleditor{Pascal Massart}{Universit{\'e} de Paris-Sud}
\journaleditor{Andrew McCallum}{University of Massachusetts Amherst}
\journaleditor{Marina Meila}{University of Washington}
\journaleditor{Andrew Moore}{CMU}
\journaleditor{John Platt}{Microsoft Research}
\journaleditor{Luc de Raedt}{KU Leuven}
\journaleditor{Christian Robert}{Paris-Dauphine}
\journaleditor{Sunita Sarawagi}{IIT Bombay}
\journaleditor{Robert Schapire}{Microsoft Research}
\journaleditor{Bernhard Schoelkopf}{Max Planck Institute}
\journaleditor{Richard Sutton}{University of Alberta}
\journaleditor{Larry Wasserman}{CMU}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> journaldata/MAL-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MALcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MALcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Machine Learning}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MAL}
\journalurl        {http://www.nowpublishers.com/MAL}
\journalissnprint  {1935-8237}
\journalissnonline {1935-8245}
\journaldoi        {10.1561/22}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Machine Learning publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Adaptive control and signal processing}
\item{Applications and case studies}
\item{Behavioral, cognitive and neural learning}
\item{Bayesian learning}
\item{Classification and prediction}
\item{Clustering}
\item{Data mining}
\item{Dimensionality reduction}
\item{Evaluation}
\item{Game theoretic learning}
\item{Graphical models}
\item{Independent component analysis}
\item{Inductive logic programming}
\item{Kernel methods}
\item{Markov chain Monte Carlo}
\item{Model choice}
\item{Nonparametric methods}
\item{Online learning}
\item{Optimization}
\item{Reinforcement learning}
\item{Relational learning}
\item{Robustness}
\item{Spectral methods}
\item{Statistical learning theory}
\item{Variational inference}
\item{Visualization}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Machine Learning, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 6 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MAL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Tensor Regression}\\
Jiani Liu, Ce Zhu, Zhen Long and Yipeng Liu\\
ISBN: 978-1-68083-886-2\\
\\
\noindent \textit{Minimum-Distortion Embedding}\\
Akshay Agrawal, Alnur Ali and Stephen Boyd\\
ISBN: 978-1-68083-888-6\\
\\
\noindent \textit{Graph Kernels: State-of-the-Art and Future Challenges}\\
Karsten Borgwardt, Elisabetta Ghisu, Felipe Llinares-López, Leslie O’Bray and Bastian Rieck\\
ISBN: 978-1-68083-770-4\\
\\
\noindent \textit{Data Analytics on Graphs Part III: Machine Learning on Graphs, from Graph Topology to Applications}\\
Ljubiša Stanković, Danilo Mandic, Miloš Daković, Miloš Brajović, Bruno Scalzo, Shengxi Li and Anthony G. Constantinides\\
ISBN: 978-1-68083-982-16\\
\\
\noindent \textit{Data Analytics on Graphs Part II: Signals on Graphso}\\
Ljubiša Stanković, Danilo Mandic, Miloš Daković, Miloš Brajović, Bruno Scalzo, Shengxi Li and Anthony G. Constantinides\\
ISBN: 978-1-68083-982-1\\
\\
\noindent \textit{Data Analytics on Graphs Part I: Graphs and Spectra on Graphs}\\
Ljubiša Stanković, Danilo Mandic, Miloš Daković, Miloš Brajović, Bruno Scalzo, Shengxi Li and Anthony G. Constantinides\\
ISBN: 978-1-68083-982-1\\

==> journaldata/MGT-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{2}\raggedright
\journalchiefeditor{Nicholas S. Argyres}{Olin Business School, Washington University\\United States}
\journalchiefeditor{Timothy M. Devinney}{Leeds University Business School\\United Kingdom}
\journalchiefeditor{James Campbell Quick}{The University of Texas at Arlington\\United States}
\end{multicols}

\subsection{Editors}
\begin{multicols}{3}\raggedright \raggedcolumns
\renewcommand\journaleditor[2]{\par\textbf{#1}\\#2}%
\subsubsection{\footnotesize International Business}

\journaleditor{Gabriel R.G. Benito}{BI Norwegian School of Management}
\journaleditor{Allan Bird}{Northeastern University}
\journaleditor{Julian Birkinshaw}{London Business School}
\journaleditor{Peter Buckley}{University of Leeds}
\journaleditor{Saul Estrin}{London School of Economics}
\journaleditor{Sarianna Lundin}{University of Bremen}
\journaleditor{Xavier Martin}{Tilburg University} 
\journaleditor{Ram Mudambi}{Temple University}

\columnbreak

\subsubsection{\footnotesize Organizational Behavior}

\journaleditor{Myrtle Bell}{University of Texas at Arlington}
\journaleditor{Cary Cooper}{Lancaster University}
\journaleditor{Richard Griffin}{Texas A\&M University}
\journaleditor{Sean Hannah}{Wake Forest University}
\journaleditor{Debra Nelson}{Oklahoma State University}
\journaleditor{Pamela Perrewe}{Florida State University}

\columnbreak

\subsubsection{\footnotesize Strategy}

\journaleditor{Rajshree Agarwal}{University of Maryland}
\journaleditor{Marvin Lieberman}{UCLA}) 
\journaleditor{Michael Lenox}{University of Virginia}
\journaleditor{Joseph Mahoney}{University of Illinois at Urbana-Champaign}
\journaleditor{Jesper Sørensen}{Stanford University}
\journaleditor{Olav Sorenson}{Yale University}
\end{multicols}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MGT-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{MGTcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {MGTcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Management}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MGT}
\journalurl        {http://www.nowpublishers.com/MGT}
\journalissnprint  {2475-6946}
\journalissnonline {2475-6954}
\journaldoi        {10.1561/34}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Management publishes
 survey and tutorial articles in the following topics:
% \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{International Business}
\item{Organizational Behavior}
\item{Strategic Management}
\end{itemize}
 %\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Management, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MIC-editorialboard.tex <==
%MIC-Editorialboard.

\begin{editorialboard}

%\subsection{Editor-in-Chief}

\journalchiefeditor{W. Kip Viscusi}{Vanderbilt University Law School\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Richard Carson}{University of California, San Diego}
\journaleditor{William Gentry}{Williams College}
\journaleditor{Tom Kniesner}{Syracuse University}
\journaleditor{Mark V. Pauly}{University of Pennsylvania}
\journaleditor{Yossi Spiegel}{Tel Aviv University}
\journaleditor{William Zame}{University of California, Los Angeles}
\journaleditor{James Ziliak}{University of Kentucky}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MIC-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{MICcolor}{pinegreen}   %new color names can be defined before use   %new color names can be defined before use
\journalcolor      {MICcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Microeconomics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MIC}
\journalurl        {http://www.nowpublishers.com/MIC}
\journalissnprint  {1547-9846}
\journalissnonline {1547-9854}
\journaldoi        {10.1561/07}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Microeconomics publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Environmental economics}
\item{Health economics}
\item{Industrial organization}
\item{Labor economics}
\item{Law and economics}
\item{Public economics}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Microeconomics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MIC-seriespage.tex <==
\vspace{12pt}
\vspace{12pt}
\noindent \textit{Behavioral Economics of Multiperiod Insurance Purchasing Behavior: The Role of Emotions}\\
Howard Kunreuther and Mark Pauly
\\ISBN: 978-1-68083-524-3
\\
\\
\noindent \textit{Trade and Climate Change: Focus on Carbon Leakage, Border Carbon Adjustments and WTO Consistency}\\
ZhongXiang Zhang
\\ISBN: 978-1-68083-482-6
\\
\\
\noindent \textit{Natural Gas Pipeline Regulation in the United States: Past, Present, and Future}\\
Matthew E. Oliver
\\ISBN: 978-1-68083-452-9
\\
\\
\noindent \textit{The U.S. Market for Uranium: 70 Years of History}\\
Charles F. Mason
\\ISBN: 978-1-68083-382-9
\\
\\
\noindent \textit{Game Theory and Water Resources: Critical Review of its Contributions, Progress and Remaining Challenges}\\
Ariel Dinar and Margaret Hogarth
\\ISBN: 978-1-68083-016-3


==> journaldata/MKT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Jehoshua Eliashberg}{University of Pennsylvania}

\subsection{Associate Editor}

\journaleditor{Bernd Schmitt}{Columbia University}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Dawn Iacobucci}{Vanderbilt University}
\journaleditor{Ganesh Iyeri}{University of California, Berkeley}
\journaleditor{Anirban Mukhopadhyayi}{HKUST}
\journaleditor{Sharon Ngi}{Nanyang Technological University}
\journaleditor{Gerrit van Bruggeni}{Erasmus University}
\journaleditor{Miguel Villas Boasi}{University of California, Berkeley}
\journaleditor{Hema Yoganarasimhani}{University of Washington}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MKT-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MKTcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MKTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Marketing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MKT}
\journalurl        {http://www.nowpublishers.com/MKT}
\journalissnprint  {1555-0753}
\journalissnonline {1555-0761}
\journaldoi        {10.1561/17}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Marketing publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{B2B Marketing}
\item{Bayesian Models}
\item{Behavioral Decision Making}
\item{Branding and Brand Equity}
\item{Channel Management}
\item{Choice Modeling}
\item{Comparative Market Structure}
\item{Competitive Marketing Strategy}
\item{Conjoint Analysis}
\item{Customer Equity}
\item{Customer Relationship Management}
\item{Game Theoretic Models}
\item{Group Choice and Negotiation}
\item{Discrete Choice Models}
\item{Individual Decision Making}
\item{Marketing Decisions Models}
\item{Market Forecasting}
\item{Marketing Information Systems}
\item{Market Response Models}
\item{Market Segmentation}
\item{Market Share Analysis}
\item{Multi-channel Marketing}
\item{New Product Diffusion}
\item{Pricing Models}
\item{Product Development}
\item{Product Innovation}
\item{Sales Forecasting}
\item{Sales Force Management}
\item{Sales Promotion}
\item{Services Marketing}
\item{Stochastic Model}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Marketing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MKT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Brands: An Integrated Marketing, Finance, and Societal Perspective}\\
Bobby J. Calder\\
ISBN: 978-1-68083-746-9\\
\\
\noindent \textit{Machine Learning in Marketing: Overview, Learning Strategies, Applications, and Future Developments}\\
Vinicius Andrade Brei\\
ISBN: 978-1-68083-720-9\\
\\
\noindent \textit{Crowdfunding Platforms: Ecosystem and Evolution}\\
Yee Heng Tan and Srinivas K. Reddy\\
ISBN: 978-1-68083-698-1\\
\\
\noindent \textit{A Practical Approach to Sales Compensation: What Do We Know Now? What Should We Know in the Future?}\\
Doug J. Chung, Byungyeon Kim and Niladri B. Syam\\
ISBN: 978-1-68083-684-4\\


==> journaldata/NET-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Anthony Ephremides}{University of Maryland\\United States}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Fran\c{c}ois Baccelli}{University of Texas, Austin}
\journaleditor{Victor Bahl}{Microsoft Research}
\journaleditor{Helmut B\"{o}lcskei}{ETH Zurich}
\journaleditor{J.J. Garcia-Luna Aceves}{UC Santa Cruz}
\journaleditor{Andrea Goldsmith}{Stanford University}
\journaleditor{Roch Guerin}{Washington University in Saint Louis}
\journaleditor{Bruce Hajek}{UIUC}
\journaleditor{Jean-Pierre Hubaux}{EPFL}
\journaleditor{Frank Kelly}{University of Cambridge}
\journaleditor{P.R. Kumar}{Texas A\&M University}
\journaleditor{Steven Low}{Caltech}
\journaleditor{Eytan Modiano}{MIT}
\columnbreak
\journaleditor{Keith Ross}{Polytechnic Institute of NYU}
\journaleditor{Henning Schulzrinne}{Columbia University}
\journaleditor{Mani Srivastava}{UCLA}
\journaleditor{Leandros Tassiulas}{Yale University}
\journaleditor{Lang Tong}{Cornell University}
\journaleditor{Ozan Tonguz}{Carnegie Mellon University}
\journaleditor{Don Towsley}{University of Massachusetts, Amherst}
\journaleditor{Nitin Vaidya}{UIUC}
\journaleditor{Pravin Varaiya}{UC Berkeley}
\journaleditor{Roy Yates}{Rutgers University}
\journaleditor{Raymond Yeung}{Chinese University of Hong Kong}
\end{multicols*}
\end{editorialboard} 

==> journaldata/NET-journaldata.tex <==
\definecolor{cerise}{rgb}{0.87, 0.19, 0.39}
\colorlet{NETcolor}{cerise}   %new color names can be defined before use
\journalcolor      {NETcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Networking}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {NET}
\journalurl        {http://www.nowpublishers.com/NET}
\journalissnprint  {1554-057X}
\journalissnonline {1554-0588}
\journaldoi        {10.1561/13}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Networking publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Modeling and Analysis of:}
	\begin{itemize}
	\item{Ad Hoc Wireless Networks}
	\item{Sensor Networks}
	\item{Optical Networks}
	\item{Local Area Networks}
	\item{Satellite and Hybrid Networks}
	\item{Cellular Networks}
	\item{Internet and Web Services}
	\end{itemize}
\item{Protocols and Cross-Layer Design}
\item{Network Coding}
\item{Energy-Efficiency Incentives/Pricing/Utility-based}
\item{Games (co-operative or not)}
\item{Security}
\item{Scalability}
\item{Topology}
\item{Control/Graph-theoretic models}
\item{Dynamics and Asymptotic Behavior of Networks}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Networking, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/NET-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Age of Information: A New Concept, Metric, and Tool}\\
Antzela Kosta, Nikolaos Pappas and Vangelis Angelakis\\
ISBN: 978-1-68083-360-7\\
\\
\noindent \textit{Network and Protocol Architectures for Future Satellite Systems}\\
Tomaso de Cola, Alberto Ginesi, Giovanni Giambene,\\ George C. Polyzos, Vasilios A. Siris, Nikos Fotiou and Yiannis Thomas\\
ISBN: 978-1-68083-334-8\\
\\
\noindent \textit{Duality of the Max-Plus and Min-Plus Network Calculus}\\
Jorg Liebeherr\\
ISBN: 978-1-68083-294-5\\
\\
\noindent \textit{Opportunistic Routing in Wireless Networks}\\
Tara Javidi and Eric Van Buhler\\
ISBN: 978-1-68083-150-4

==> journaldata/NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> journaldata/OPT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

%\begin{multicols}{1}
\journalchiefeditor{Garud Iyengar}{Columbia University, USA}
%\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Dimitris Bertsimas}{Massachusetts Institute of Technology}
\journaleditor{John R. Birge}{The University of Chicago}
\journaleditor{Robert E. Bixby}{Rice University}
\journaleditor{Emmanuel Candes}{Stanford University}
\journaleditor{David Donoho}{Stanford University}
\journaleditor{Laurent El Ghaoui}{University of California, Berkeley}
\journaleditor{Donald Goldfarb}{Columbia University}
\journaleditor{Michael I. Jordan}{University of California, Berkeley}
\journaleditor{Zhi-Quan (Tom) Luo}{University of Minnesota, Twin Cites}
\journaleditor{George L. Nemhauser}{Georgia Institute of Technology}
\journaleditor{Arkadi Nemirovski}{Georgia Institute of Technology}
\columnbreak
\journaleditor{Yurii Nesterov}{HSE University}
\journaleditor{Jorge Nocedal}{Northwestern University}
\journaleditor{Pablo A. Parrilo}{Massachusetts Institute of Technology}
\journaleditor{Boris T. Polyak}{Institute for Control Science, Moscow}
\journaleditor{Tam\'as Terlaky}{Lehigh University}
\journaleditor{Michael J. Todd}{Cornell University}
\journaleditor{Kim-Chuan Toh}{National University of Singapore}
\journaleditor{John N. Tsitsiklis}{Massachusetts Institute of Technology}
\journaleditor{Lieven Vandenberghe}{University of California, Los Angeles}
\journaleditor{Robert J. Vanderbei}{Princeton University}
\journaleditor{Stephen J. Wright}{University of Wisconsin}
\end{multicols*}
\end{editorialboard} 

==> journaldata/OPT-journaldata.tex <==
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\colorlet{OPTcolor}{Cerulean}   %new color names can be defined before use
\journalcolor      {OPTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Optimization}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {OPT}
\journalurl        {http://www.nowpublishers.com/OPT}
\journalissnprint  {2167-3888}
\journalissnonline {2167-3918}
\journaldoi        {10.1561/24}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Optimization publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{algorithm design, analysis, and implementation (especially, on modern computing platforms}
\item{models and modeling systems, new optimization formulations for practical problems}
\item{applications of optimization in machine learning, statistics, and data analysis, signal and image processing, computational economics and finance, engineering design, scheduling and resource allocation, and other areas}
\end{itemize}
 %\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Optimization, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/OPT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Atomic Decomposition via Polar Alignment: The Geometry of Structured Optimization}\\
Zhenan Fan, Halyun Jeong, Yifan Sun and Michael P. Friedlander\\
ISBN: 978-1-68083-742-1\\
\\
\noindent \textit{Optimization Methods for Financial Index Tracking: From Theory to Practice}\\
Konstantinos Benidis, Yiyong Feng and Daniel P. Palomar\\
ISBN: 978-1-68083-464-2\\
\\
\noindent \textit{The Many Faces of Degeneracy in Conic Optimization}\\
Dmitriy Drusvyatskiy and Henry Wolkowicz\\
ISBN: 978-1-68083-390-4\\

==> journaldata/PGL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Rupak Majumdari}{Max Planck Institute for Software Systems}


\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Mart\'in Abadi}{Google and UC Santa Cruz}
\journaleditor{Anindya Banerjee}{IMDEA Software Instituet}
\journaleditor{Patrick Cousot}{ENS, Paris and NYU}
\journaleditor{Oege De Moor}{University of Oxford}
\journaleditor{Matthias Felleisen}{Northeastern University}
\journaleditor{John Field}{Google}
\journaleditor{Cormac Flanagan}{UC Santa Cruz}
\journaleditor{Philippa Gardner}{Imperial College}
\journaleditor{Andrew Gordon}{Microsoft Research and University of Edinburgh}
\journaleditor{Dan Grossman}{University of Washington}
\journaleditor{Robert Harper}{CMU}
\journaleditor{Tim Harris}{Amazon}
\journaleditor{Fritz Henglein}{University of Copenhagen}
\journaleditor{Rupak Majumdar}{MPI and UCLA}
\journaleditor{Kenneth McMillan}{Microsoft Research}
\journaleditor{J. Eliot B. Moss}{University of Massachusetts, Amherst}
\journaleditor{Andrew C. Myers}{Cornell University}
\journaleditor{Hanne Riis Nielson}{Technical University of Denmark}
\journaleditor{Peter O'Hearni}{University College London}
\journaleditor{Benjamin C. Pierce}{University of Pennsylvania}
\journaleditor{Andrew Pittsi}{University of Cambridge}
\journaleditor{Ganesan Ramalingami}{Microsoft Research}
\journaleditor{Mooly Sagiv}{Tel Aviv University}
\journaleditor{Davide Sangiorgi}{University of Bologna}
\journaleditor{David Schmidt}{Kansas State University}
\journaleditor{Peter Sewell}{University of Cambridge}
\journaleditor{Scott Stoller}{Stony Brook University}
\journaleditor{Peter Stuckey}{University of Melbourne}
\journaleditor{Jan Vitek}{Northeastern University}
\journaleditor{Philip Wadler}{University of Edinburgh}
\journaleditor{David Walker}{Princeton University}
\journaleditor{Stephanie Weiric}{University of Pennsylvania}
\end{multicols*}
\end{editorialboard} 

==> journaldata/PGL-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{PGLcolor}{brickred}   %new color names can be defined before use
\journalcolor      {PGLcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Programming Languages}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {PGL}
\journalurl        {http://www.nowpublishers.com/PGL}
\journalissnprint  {2325-1107}
\journalissnonline {2325-1131}
\journaldoi        {10.1561/25}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Programming Languages publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Abstract Interpretation}
\item{Compilation and Interpretation Techniques}
\item{Domain Specific Languages}
\item{Formal Semantics, including Lambda Calculi, Process Calculi, and Process Algebra}
\item{Language Paradigms}
    \item{Mechanical Proof Checking}
    \item{Memory Management}
    \item{Partial Evaluation}
    \item{Program Logic}
    \item{Programming Language Implementation}
    \item{Programming Language Security}
    \item{Programming Languages for Concurrency}
    \item{Programming Languages for Parallelism}
    \item{Program Synthesis}
    \item{Program Transformations and Optimizations}
    \item{Program Verification}
    \item{Runtime Techniques for Programming Languages}
    \item{Software Model Checking}
    \item{Static and Dynamic Program Analysis}
    \item{Type Theory and Type Systems}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Programming Languages, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/PGL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Shape Analysis}\\
Bor-Yuh Evan Chang, Cezara Drăgoi, Roman Manevich, Noam Rinetzky and Xavier Rival\\
ISBN: 978-1-68083-732-2\\
\\
\noindent \textit{Progress of Concurrent Objects}\\
Hongjin Liang and Xinyu Feng\\
ISBN: 978-1-68083-672-1\\
\\
\noindent \textit{QED at Large: A Survey of Engineering of Formally Verified \\Software}\\
Talia Ringer, Karl Palmskog, Ilya Sergey, Milos Gligoric and \\Zachary Tatlock\\
ISBN: 978-1-68083-594-6\\
\\
\noindent \textit{Reconciling Abstraction with High Performance: A MetaOCaml \\approach}\\
Oleg Kiselyov\\
ISBN: 978-1-68083-436-9

==> journaldata/ROB-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}
\journalchiefeditor{Julie Shah}{Massachusetts Institute of Technology}

\subsection{Honorary Editors}
\journaleditor{Henrik Christensen}{University of California, San Diego}
\journaleditor{Roland Siegwart}{ETH Zurich}


\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Minoru Asada}{Osaka University}
\journaleditor{Antonio Bicchi}{University of Pisa}
\journaleditor{Aude Billard}{EPFL}
\journaleditor{Cynthia Breazeal}{Massachusetts Institute of Technology}
\journaleditor{Oliver Brock}{TU Berlin}
\journaleditor{Wolfram Burgard}{University of Freiburg}
\journaleditor{Udo Frese}{University of Bremen}
\journaleditor{Ken Goldberg}{University of California, Berkeley}
\journaleditor{Hiroshi Ishiguro}{Osaka University}
\journaleditor{Makoto Kaneko}{Osaka University}
\journaleditor{Danica Kragic}{KTH Stockholm}
\journaleditor{Vijay Kumar}{University of Pennsylvania}
\journaleditor{Simon Lacroix}{LAAS}
\journaleditor{Christian Laugier}{INRIA}
\journaleditor{Steve LaValle}{University of Illinois at Urbana-Champaign}
\journaleditor{Yoshihiko Nakamura}{The University of Tokyo}
\journaleditor{Brad Nelson}{ETH Zurich}
\journaleditor{Paul Newman}{University of Oxford}
\journaleditor{Daniela Rus}{Massachusetts Institute of Technology}
\journaleditor{Giulio Sandini}{University of Genova}
\journaleditor{Sebastian Thrun}{Stanford University}
\journaleditor{Manuela Veloso}{Carnegie Mellon University}
\journaleditor{Markus Vincze}{Vienna University}
\journaleditor{Alex Zelinsky}{DSTG}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ROB-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{ROBcolor}{pinegreen}   %new color names can be defined before use
\journalcolor      {ROBcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Robotics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ROB}
\journalurl        {http://www.nowpublishers.com/ROB}
\journalissnprint  {1935-8253}
\journalissnonline {1935-8261}
\journaldoi        {10.1561/23}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Robotics publishes
 survey and tutorial articles in the following topics:
\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Mathematical modelling}
\item{Kinematics}
\item{Dynamics}
\item{Estimation Methods}
\item{Robot Control}
\item{Planning}
\item{Artificial Intelligence in Robotics}
\item{Software Systems and Architectures}
\item{Mechanisms and Actuators}
\item{Sensors and Estimation}
\item{Planning and Control}
\item{Human-Robot Interaction}
\item{Industrial Robotics}
\item{Service Robotics }
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Robotics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ROB-seriespage.tex <==
\vspace{12pt}
\noindent \textit{A Roadmap for US Robotics – From Internet to Robotics 2020 Edition}\\
Henrik Christensen, Nancy Amato, Holly Yanco, Maja Mataric, Howie Choset, Ann Drobnis, Ken Goldberg, Jessy Grizzle, Gregory Hager, John Hollerbach, Seth Hutchinson, Venkat Krovi, Daniel Lee, Bill Smart, Jeff Trinkle and Gaurav Sukhatme\\
ISBN: 978-1-68083-858-9\\
\\
\noindent \textit{The State of Industrial Robotics: Emerging Technologies, Challenges, and Key Research Directions}\\
Lindsay Sanneman, Christopher Fourie and Julie A. Shah\\
ISBN: 978-1-68083-800-8\\
\\
\noindent \textit{Semantics for Robotic Mapping, Perception and Interaction: A Survey}\\
Sourav Garg, Niko Sünderhauf, Feras Dayoub, Douglas Morrison, Akansel Cosgun, Gustavo Carneiro, Qi Wu, Tat-Jun Chin, Ian Reid, Stephen Gould, Peter Corke and Michael Milford\\
ISBN: 978-1-68083-768-1\\


==> journaldata/SEC-editorialboard.tex <==
%SEC-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Anupam Datta}{Carnegie Mellon University, USA}
\journalchiefeditor{Jeannette Wing}{Columbia University, USA}


\subsection{Editors}
\begin{multicols}{2}\raggedcolumns
\journaleditor{Mart\'in Abadi}{Google and University of California, Santa Cruz}
\journaleditor{Michael Backes}{Saarland University}
\journaleditor{Dan Boneh}{Stanford University, USA}
\journaleditor{V\'eronique Cortier}{LORIA, CNRS, France}
\journaleditor{Lorrie Cranor}{Carnegie Mellon University}
\journaleditor{C\'edric Fournet}{Microsoft Research}
\journaleditor{Virgil Gligor}{Carnegie Mellon University}
\journaleditor{Jean-Pierre Hubaux}{EPFL}
\journaleditor{Deirdre Mulligan}{University of California, Berkeley}
\journaleditor{Andrew Myers}{Cornell University}
\journaleditor{Helen Nissenbaum}{New York University}
\journaleditor{Michael Reiter}{University of North Carolina}
\journaleditor{Shankar Sastry}{University of California, Berkeley}
\journaleditor{Dawn Song}{University of California, Berkeley}
\journaleditor{Daniel Weitzner}{Massachusetts Institute of Technology}
\end{multicols}
\end{editorialboard} 


==> journaldata/SEC-journaldata.tex <==
\definecolor{bananayellow}{rgb}{1.0, 0.88, 0.21}
\colorlet{SECcolor}{bananayellow}   %new color names can be defined before use
\journalcolor      {SECcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Privacy and Security}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SEC}
\journalurl        {http://nowpublishers.com/SEC}
\journalissnprint  {2474-1558}
\journalissnonline {2474-1566}
\journaldoi        {10.1561/33}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Privacy and Security publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Access control}
\item{Accountability}
\item{Anonymity}
\item{Application security}
\item{Artifical intelligence methods in security and privacy}
\item{Authentication}
\item{Big data analytics and privacy}
\item{Cloud security}
\item{Cyber-physical systems security and privacy}
\item{Distributed systems security and privacy}
\item{Embedded systems security and privacy}
\item{Forensics}
\item{Hardware security}
\item{Human factors in security and privacy}
\item{Information flow}
\item{Intrusion detection}
\item{Malware}
\item{Metrics}
\item{Mobile security and privacy}
\item{Language-based security and privacy}
\item{Network security}
\item{Privacy-preserving systems}
\item{Protocol security}
\item{Security and privacy policies}
\item{Security architectures}
\item{System security}
\item{Web security and privacy}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Privacy and Security, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SEC-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Contextual Integrity through the Lens of Computer Science}\\
Sebastian Benthall, Seda Gurses and Helen Nissenbaum\\
ISBN: 978-1-68083-384-3\\
\\
\noindent \textit{Methods for Location Privacy: A comparative overview}\\
Kostantinos Chatzikokolakis, Ehab ElSalamouny, Catuscia Palamidessi and Pazii Anna\\
ISBN: 978-1-68083-366-9\\
\\
\noindent \textit{Principles and Implementation Techniques of Software-Based Fault Isolation}\\
Gang Tan\\
ISBN: 978-1-68083-344-7\\
\\
\noindent \textit{Modeling and Verifying Security Protocols with the Applied Pi\\ Calculus and ProVerif}\\
Bruno Blanchet\\
ISBN: 978-1-68083-206-8

==> journaldata/SIG-editorialboard.tex <==
%SIG-Editorialboard.

\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Yonina Eldar}{Weizmann Institute\\Israel}



\subsection{Editors}
\begin{multicols}{3}\raggedcolumns
\journaleditor{Pao-Chi Chang}{National Central University}
\journaleditor{Pamela Cosman}{University of California, San Diego}
\journaleditor{Michelle Effros}{California Institute of Technology}
\journaleditor{Yariv Ephraim}{George Mason University}
\journaleditor{Alfonso Farina}{Selex ES}
\journaleditor{Sadaoki Furui}{Tokyo Institute of Technology}
\journaleditor{Georgios Giannakis}{University of Minnesota}
\journaleditor{Vivek Goyal}{Boston University}
\journaleditor{Sinan Gunturk}{Courant Institute}
\journaleditor{Christine Guillemot}{INRIA}
\journaleditor{Robert W. Heath, Jr.}{The University of Texas at Austin}
\journaleditor{Sheila Hemami}{Northeastern University}
\journaleditor{Lina Karam}{Arizona State University}
\journaleditor{Nick Kingsbury}{University of Cambridge}
\journaleditor{Alex Kot}{Nanyang Technical University}
\journaleditor{Jelena Kovacevic}{New York University}
\journaleditor{Geert Leus}{TU Delft}
\journaleditor{Jia Li}{Pennsylvania State University}
\journaleditor{Henrique Malvar}{Microsoft Research}
\journaleditor{B.S. Manjunath}{University of California, Santa Barbara}
\journaleditor{Urbashi Mitra}{University of Southern California}
\journaleditor{Bj\"{o}rn Ottersten}{KTH Stockholm}
\journaleditor{Vincent Poor}{Princeton University}
\journaleditor{Anna Scaglione}{University of California, Davis}
\journaleditor{Mihaela van der Shaar}{University of California, Los Angeles}
\journaleditor{Nicholas D. Sidiropoulos}{Technical University of Crete}
\journaleditor{Michael Unser}{EPFL}
\journaleditor{P.P. Vaidyanathan}{California Institute of Technology}
\journaleditor{Ami Wiesel}{The Hebrew University of Jerusalem}
\journaleditor{Min Wu}{University of Maryland}
\journaleditor{Josiane Zerubia}{INRIA}
\end{multicols}
\end{editorialboard} 


==> journaldata/SIG-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{SIGcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {SIGcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Signal Processing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SIG}
\journalurl        {http://www.nowpublishers.com/SIG}
\journalissnprint  {1932-8346}
\journalissnonline {1932-8354}
\journaldoi        {10.1561/20}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Adaptive signal processing}
\item{Audio signal processing}
\item{Biological and biomedical signal processing}
\item{Complexity in signal processing}
\item{Digital signal processing}
\item{Distributed and network signal processing}
\item{Image and video processing}
\item{Linear and nonlinear filtering}
\item{Multidimensional signal processing}
\item{Multimodal signal processing}
\item{Multirate signal processing}
\item{Multiresolution signal processing}
\item{Nonlinear signal processing}
\item{Randomized algorithms in signal processing}
\item{Sensor and multiple source signal processing, source separation}
\item{Signal decompositions, subband and transform methods, sparse representations}
\item{Signal processing for communications}
\item{Signal processing for security and forensic analysis, biometric signal processing}
\item{Signal quantization, sampling, analog-to-digital conversion, coding and compression}
\item{Signal reconstruction, digital-to-analog conversion, enhancement, decoding and inverse problems}
\item{Speech/audio/image/video compression}
\item{Speech and spoken language processing}
\item{Statistical/machine learning}
\item{Statistical signal processing}
	\begin{itemize}
	\item{Classification and detection}
	\item{Estimation and regression}
	\item{Tree-structured methods}
	\end{itemize}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SIG-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Recent Advances in Clock Synchronization for Packet-Switched Networks}\\
Anantha K. Karthik and Rick S. Blum\\
ISBN: 978-1-68083-726-1\\
\\
\noindent \textit{Biomedical Image Reconstruction: From the Foundations to Deep Neural Networks}\\
Michael T. McCann and Michael Unser\\
ISBN: 978-1-68083-650-9\\
\\
\noindent \textit{Compressed Sensing with Applications in Wireless Networks}\\
Markus Leinonen, Marian Codreanu and Georgios B. Giannakis\\
ISBN: 978-1-68083-646-2\\

==> journaldata/STP-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Audretsch}{Indiana University}
\journaleditor{William Bonvillian}{MIT}
\journaleditor{Barry Bozeman}{Arizona State University}
\journaleditor{Kaye Husbands Fealing}{Georgia Institute of Technology}
\journaleditor{John Hardin}{North Carolina Board of Science and Technology}
\journaleditor{Mariagrazia Squicciarini}{OECD}
\journaleditor{Wolfgang Polt}{Joanneum Research Institute}
\journaleditor{Nicholas Vonortas}{The George Washington University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/STP-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ASTPcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ASTPcolor} %a color name. 
\journaltitle      {Annals of Science and Technology Policy}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ASTP}
\journalurl        {http://www.nowpublishers.com/ASTP}
\journalissnprint  {2475-1820}
\journalissnonline {2475-1812}
\journaldoi        {10.1561/110}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Annals of Science and Technology Policy publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Literature reviews of technology and innovation policies}
\item{Historical case studies of technology development and implementation}
\item{Institutional histories of technology- and innovation-based organizations}
\item{Analyses of policies attendant to technology development and adoption and diffusion}
\item{Studies documenting the adoption and diffusion of technologies and subsequent consequences}
\item{Studies of public and private research partnerships (cross sectional, over time, or case based)}
\item{Assessments and evaluations of specific technology and innovation policies}
\item{Analyses of ecosystems associated with the technology and/or innovation development}
\item{Cross observational (e.g., cross-agency or cross-country) comparisons of technology and innovation policies}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Annals of Science and Technology Policy, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SYS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Panos J. Antsaklis}{University of Notre Dame\\United States}
\journalchiefeditor{Alessandro Astolfi}{Imperial College London, United Kingdom\\ University of Rome ''Tor Vergata'', Italy}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{John Baillieul}{Boston University}
\journaleditor{Peter Caines}{McGill University}
\journaleditor{Christos Cassandras}{Boston University}
\journaleditor{Denis Dochain}{UC Louvain}
\journaleditor{Magnus Egerstedt}{Georgia Institute of Technology}
\journaleditor{Karl Henrik Johansson}{KTH Stockholm}
\journaleditor{Miroslav Krstic}{University of California, San Diego}
\journaleditor{Jan Maciejowski}{University of Cambridge}
\columnbreak
\journaleditor{Dragan Nesic}{The University of Melbourne}
\journaleditor{Marios Polycarpou}{University of Cyprus}
\journaleditor{J\"{o}rg Raisch}{Technical University Berlin}
\journaleditor{Arjan van der Schaft}{University of Groningen}
\journaleditor{M. Elena Valcher}{University of Padova}
\journaleditor{Richard Vinter}{Imperial College London}
\journaleditor{George Weiss}{Tel Aviv University}
\end{multicols*}
\end{editorialboard} 

==> journaldata/SYS-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet {SYScolor}{cobalt} %new color names can be defined before use
\journalcolor      {SYScolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Systems and Control}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SYS}
\journalurl        {http://www.nowpublishers.com/SYS}
\journalissnprint  {2325-6818}
\journalissnonline {2325-6826}
\journaldoi        {10.1561/26}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Systems and Control publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Control of:}
	\begin{itemize}
	\item{Hybrid and Discrete Event Systems}
	\item{Nonlinear Systems}
	\item{Network Systems}
	\item{Stochastic Systems}
	\item{Multi-agent Systems}
	\item{Distributed Parameter Systems}
	\item{Delay Systems}
	\end{itemize}
	\columnbreak
\item{Filtering, Estimation, Identification}
\item{Optimal Control}
\item{Systems Theory}
\item{Control Applications}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Systems and Control, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SYS-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Learning-Based Control: A Tutorial and Some Recent Results}\\
Zhong-Ping Jiang, Tao Bian and Weinan Gao\\
ISBN: 978-1-68083-752-0\\
\\
\noindent \textit{Synchronous Reinforcement Learning-Based Control for Cognitive Autonomy}\\
Kyriakos G. Vamvoudakis and Nick-Marios T. Kokolakis\\
ISBN: 978-1-68083-744-5\\
\\
\noindent \textit{Achieving Ecological Resilience Through Regime Shift Management}\\
M. D. Lemmon\\
ISBN: 978-1-68083-716-2\\
\\
\noindent \textit{Distributed Optimization for Smart Cyber-Physical Networks}\\
Giuseppe Notarstefano, Ivano Notarnicola and Andrea Camisa\\
ISBN: 978-1-68083-618-9\\
\\
\noindent \textit{Resilient Control in Cyber-Physical Systems: Countering Uncertainty, Constraints, and Adversarial Behavior}\\
Sean Weerakkody, Omur Ozel, Yilin Mo and Bruno Sinopoli\\
ISBN: 978-1-68083-586-1


==> journaldata/TCS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Salil Vadhan}{Harvard University\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Bernard Chazelle}{Princeton University}
\journaleditor{Oded Goldreich}{Weizmann Institute}
\journaleditor{Shafi Goldwasser}{Massachusetts Institute of Technology and Weizmann Institute}
\journaleditor{Sanjeev Khanna}{University of Pennsylvania}
\journaleditor{Jon Kleinberg}{Cornell University}
\journaleditor{L\'aszl\'o Lov\'asz}{Eötvös Lor\'and University}
\journaleditor{Christos Papadimitriou}{University of California, Berkeley}
\journaleditor{Peter Shor}{Massachusetts Institute of Technology}
\journaleditor{Eva Tardos}{Cornell University}
\journaleditor{Salil Vadhan}{Cornell University}
\journaleditor{Avi Wigderson}{AIS, Princeton University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/TCS-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{TCScolor}{cobalt}   %new color names can be defined before use
\journalcolor      {TCScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {TCS}
\journalurl        {http://www.nowpublishers.com/TCS}
\journalissnprint  {1551-305X}
\journalissnonline {1551-3068}
\journaldoi        {10.1561/04}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Algorithmic game theory}
    \item{Computational algebra}
    \item{Computational aspects of combinatorics and graph theory}
    \item{Computational aspects of communication}
    \item{Computational biology}
    \item{Computational complexity}
    \item{Computational geometry}
    \item{Computational learning}
    \item{Computational Models and Complexity}
    \item{Computational Number Theory}
    \item{Cryptography and information security}
    \item{Data structures}
    \item{Database theory}
    \item{Design and analysis of algorithms}
    \item{Distributed computing}
    \item{Information retrieval}
    \item{Operations Research}
    \item{Parallel algorithms}
    \item{Quantum Computation}
    \item{Randomness in Computation}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/TCS-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Higher-order Fourier Analysis and Applications}\\
Hamed Hatami, Pooya Hatami and Shachar Lovett\\
ISBN: 978-1-68083-592-2\\
\\
\noindent \textit{On Doubly-Efficient Interactive Proof Systems}\\
Oded Goldreich \\
ISBN: 978-1-68083-424-6\\
\\
\noindent \textit{Coding for Interactive Communication: A Survey}\\
Ran Gelles\\
ISBN: 978-1-68083-346-1\\

==> journaldata/TOM-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Panos Kouvelis}{Washington University St. Louis\\USA}

\subsection{Editors}
\journaleditor{Charles Corbett}{UCLA, USA}
\journaleditor{Uday Karmarkar}{UCLA, USA}

\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Onur Bayabatli}{Singapore Management University, Singapore}
\journaleditor{Jan Fransoo}{Tilburg University, The Netherlands} 
\journaleditor{Chuck Munson}{Washington State University, USA} 
\journaleditor{Nicholas Petruzzi}{Pennsylvania State University, USA}
\journaleditor{Guillaume Roels}{INSEAD, France}
\journaleditor{Nicola Secomandi}{Carnegie-Mellon University, USA} 
\journaleditor{Zuo-Jun Max Shen}{University of California, Berkeley, USA} 
\journaleditor{Sherri Xiaole Wu}{Fudan University, China} 
\journaleditor{Y. Karen Zheng}{MIT, USA} 
%\end{multicols*}
\end{editorialboard} 

==> journaldata/TOM-journaldata.tex <==
\definecolor{cerise}{rgb}{0.87, 0.19, 0.39}
\colorlet{TOMcolor}{cerise}   %new color names can be defined before use
\journalcolor      {TOMcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Technology, Information and Operations Management}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {TOM}
\journalurl        {http://www.nowpublishers.com/TOM}
\journalissnprint  {1571-9545}
\journalissnonline {1571-9553}
\journaldoi        {10.1561/02}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Technology, Information and Operations Management publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{B2B Commerce}
\item{Business Process Engineering and Design}
\item{Business Process Outsourcing}
\item{Capacity Planning}
\item{Competitive Operations}
\item{Contracting in Supply Chains}
\item{E-Commerce and E-Business Models}
\item{Electronic markets, auctions and exchanges}
\item{Enterprise Management Systems}
\item{Facility Location}
\item{Information Chain Structure and Competition}
\item{International Operations}
\item{Marketing/Manufacturing Interfaces}
\item{Multi-location inventory theory}
\item{New Product \& Service Design}
\item{Queuing Networks}
\item{Reverse Logistics}
\item{Service Logistics and Product Support}
\item{Supply Chain Management}
\item{Technology Management and Strategy}
\item{Technology, Information and Operations in:}
	\begin{itemize}
	\item{Automotive Industries}
	\item{Electronics manufacturing}
	\item{Financial Services}
	\item{Health Care}
	\item{Media and Entertainment}
	\item{Process Industries}
	\item{Retailing}
	\item{Telecommunications}
	\end{itemize}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Technology, Information and Operations Management, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/TOM-seriespage.tex <==
\vspace{12pt}
\noindent \textit{AI and Business Models: The Good, The Bad and The Ugly}\\
Vania Sena and Manuela Nocker
\\ISBN: 978-1-68083-794-0
\\
\\
\noindent \textit{The Business of Electric Vehicles: A Platform Perspective}\\
Jonas Boehm, Hemant K. Bhargava and Geoffrey G. Parker
\\ISBN: 978-1-68083-762-9
\\
\\
\noindent \textit{Advances in Supply Chain Finance and FinTech Innovations Overview}\\
Panos Kouvelis, Ling Dong and Danko Turcic
\\ISBN: 978-1-68083-722-3

==> journaldata/WEB-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{1}%\raggedcolumns
\journalchiefeditor{Wendy Hall}{University of Southampton, UK}
\journalchiefeditor{Noshir R. Contractor}{Northwestern University, USA}
\journalchiefeditor{Kieron O'Hara}{University of Southampton, UK}
\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Tim Berners-Lee}{Massachusetts Institute of Technology}
\journaleditor{Noshir Contractor}{Northwestern University}
\journaleditor{Lorrie Crano}{Carnegie Mellon University}
\journaleditor{Dieter Fensel}{University of Innsbruck}
\journaleditor{Carole Goble}{University of Manchester}
\journaleditor{Pat Hayes}{IHMC}
\journaleditor{James Hendler}{Rensselaer Polytechnic Institute}
\journaleditor{Arun Iyengar}{IBM Research}
%\columnbreak
\journaleditor{Craig Knoblock}{University of Southern California}
\journaleditor{Ora Lassila}{Pegasystems}
\journaleditor{Sun Maosong}{Tsinghua University}
\journaleditor{Cathy Marshall}{Microsoft}
\journaleditor{Peter Monge}{University of Southern California}
\journaleditor{Ben Shneiderman}{University of Maryland}
\journaleditor{Danny Weitzner}{Massachusetts Institute of Technology}
\journaleditor{Yorick Wilks}{University of Sheffield}
\end{multicols*}
\end{editorialboard} 

==> journaldata/WEB-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{WEBcolor}{brickred}   %new color names can be defined before use
\journalcolor      {WEBcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Web Science}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {WEB}
\journalurl        {http://www.nowpublishers.com/WEB}
\journalissnprint  {1551-3939}
\journalissnonline {1551-3947}
\journaldoi        {10.1561/10}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Web Science publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Agents and the Semantic Web}
    \item{Collective Intelligence}
    \item{Content Management}
    \item{Databases on the Web}
    \item{Data Mining}
    \item{Democracy and the Web}
    \item{Dependability}
    \item{Economics of information and the Web}
    \item{E-Crime}
    \item{E-Government}
    \item{Emergent behaviour}
    \item{Ethics}
    \item{Hypertext/Hypermedia}
    \item{Identity}
    \item{Languages on the Web}
    \item{Memories for Life}
    \item{Mobile/Pervasive}
    \item{Network Infrastructures}
    \item{Performance}
    \item{Privacy}
    \item{Scalability}
    \item{Security}
    \item{Semantic Web}
    \item{Social Networking}
    \item{Standards}
    \item{The Law and the Web}
    \item{The Web as an Educational Tool}
    \item{The Web in the Developing World}
    \item{Trust and Provenance}
    \item{Universal Usability}
    \item{User Interfaces}
    \item{Virtual Reality}
    \item{Web Art}
    \item{Web Governance}
    \item{Search}
    \item{Web Services}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Web Science, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/WEB-seriespage.tex <==
\vspace{12pt}
\noindent \textit{An Introduction to Hybrid Human-Machine Information Systems}\\
Gianluca Demartini, Djellel Eddine Difallah, Ujwal Gadiraju and\\ Michele Catasta\\
ISBN: 978-1-68083-374-4\\
\\
\noindent \textit{Minds Online: The Interface between Web Science, Cognitive Science and the Philosophy of Mind}\\
Paul Smart, Robert Clowes and Richard Heersmink\\
ISBN: 978-1-68083-322-5\\
\\
\noindent \textit{Collective Attention on the Web}\\
Christian Bauckhage and Kristian Kersting\\
ISBN: 978-1-68083-204-4
